Certified Robustness to Programmable Transformations in LSTMs

Deep neural networks for natural language processing are fragile in the face of adversarial examples -- small input perturbations, like synonym substitution or word duplication, which cause a neural network to change its prediction. We present an approach to certifying the robustness of LSTMs (and extensions of LSTMs) and training models that can be efficiently certified. Our approach can certify robustness to intractably large perturbation spaces defined programmatically in a language of string transformations. Our evaluation shows that (1) our approach can train models that are more robust to combinations of string transformations than those produced using existing techniques; (2) our approach can show high certification accuracy of the resulting models.

==> LSTM%20robust%20training%20(EMNLP)/macros.tex <==
%%%%%%%%%%%%%%%%%% Notes %%%%%%%%%%%%%%%%%%
\newcommand{\mytodoblue}[1]{\textcolor{blue}{\ding{46}~{\sf}~#1}}
\newcommand{\mytodoviolet}[1]{\textcolor{violet}{\ding{46}~{\sf}~#1}}
\newcommand{\mytodopink}[1]{\textcolor{Maroon}{\ding{46}~{\sf}~#1}}

\newcommand{\yh}[1]{\mytodopink{[yuhao: #1]}}
\newcommand{\loris}[1]{\mytodoviolet{[loris: #1]}}
\newcommand{\aws}[1]{\mytodoblue{aws---#1}}

\newcommand{\newadded}[1]{
\textcolor{red}{==========new BEGIN==========}

#1

\textcolor{red}{==========new END==========}
}

% \newcommand{\yh}[1]{}
% \newcommand{\loris}[1]{}
% \newcommand{\aws}[1]{}

\newcommand{\todo}[1]{{\color{red} \bf \{TODO: {#1}\}}}
\newcommand{\etal}{et al.}
\newcommand{\code}[1]{{\tt {#1}}}
\newcommand{\smalltitle}[1]{{\smallskip \noindent \bf  {#1}.\ }}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


\def\modify#1#2#3{{\small\underline{\sf{#1}}:} {\color{red}{\small #2}}
{{\color{red}\mbox{$\Rightarrow$}}} {\color{blue}{#3}}}

\newcommand{\yhmodify}[2]{\modify{Yuhao}{#1}{#2}}

\expandafter\def\expandafter\UrlBreaks\expandafter{\UrlBreaks%  save the current one
  \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j%
  \do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t%
  \do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D%
  \do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N%
  \do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X%
  \do\Y\do\Z}

%%%%%%%%%%%%%%%%%% Code %%%%%%%%%%%%%%%%%%
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{1,1,1}
 
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,           
    tabsize=2,
    xleftmargin=1.5em
}

\lstset{style=mystyle}


%%%%%%%%%%%%%%%%%% Math & Symbols %%%%%%%%%%%%%%%%%%
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{proposition}{Proposition}[section]

\newcommand{\hstate}[0]{h}
\newcommand{\cstate}[0]{c}
\newcommand{\rnnfun}[0]{g}
\newcommand{\relation}[0]{R}
\newcommand{\spec}[0]{S}
\newcommand{\specspace}[0]{\mathbb{S}}
\newcommand{\perturb}[0]{P}
\newcommand{\alphabet}[0]{\Sigma}
\newcommand{\bfx}[0]{\mathbf{x}}
\newcommand{\bfz}[0]{\mathbf{z}}
\newcommand{\bft}[0]{\mathbf{t}}
\def\perturbs#1{\perturb_{#1}}
\def\substring#1#2#3{#1_{#2:#3}}
\newcommand{\treespace}[0]{\mathbb{T}}
\newcommand{\labelspace}[0]{\mathbb{L}}
\def\subtree#1#2{#1_{#2}}
\newcommand{\constree}[0]{\emph{TrCons}}
\newcommand{\embed}[0]{\phi}
\newcommand{\dinput}[0]{{d_i}}
\newcommand{\dhidden}[0]{{d_h}}
\newcommand{\chidden}[0]{{d_c}}
\newcommand{\out}[0]{\mathbf{o}}
\newcommand{\mapping}[0]{\emph{P2O}}
\newcommand{\offset}{\textsc{off}}
\def\term#1{\emph{term}[#1]}
\newcommand{\variables}[0]{X}
\def\termspace#1#2{\gT_{#1}#2}
\def\lb#1{{#1}^\emph{(lb)}}
\def\ub#1{{#1}^\emph{(ub)}}
\newcommand{\mt}[0]{m}
\newcommand{\vars}[0]{\emph{vars}}
\newcommand{\pos}[0]{\emph{pos}}
\newcommand{\toolname}[0]{ARC}
\newcommand{\reviewperturb}[0]{S_\emph{review}}
\newcommand{\jiaapproach}[0]{CertSub}
% PROMPT	PROvable dynaMic Programming Training

\def\interval#1#2{l^{(#1)}_{#2}, u^{(#1)}_{#2}}
\def\simitvl#1#2{\alpha^{(#1)}_{#2}}


\newcommand{\Tinsword}{T_{\emph{Dup}}}
\newcommand{\Tdelword}{T_{\emph{DelStop}}}
\newcommand{\Tsubword}{T_{\emph{SubSyn}}}
\newcommand{\SDS}{\{(\Tdelword{}, 2), (\Tsubword{}, 2)\}}%{S_\emph{DS}}
\newcommand{\SIS}{\{(\Tinsword{}, 2), (\Tsubword{}, 2)\}}%{S_\emph{IS}}
\newcommand{\SDI}{\{(\Tdelword{}, 2), (\Tinsword{}, 2)\}}%{S_\emph{DI}}

\newcommand{\lengththreecell}{4.3cm}
\newcommand{\lengthcell}{0.82cm}
\newcommand{\lengthcellshorter}{0.6cm}
\newcommand{\lengthcelllonger}{0.84cm}
\newcommand{\Exhaustiveshort}{EX Acc.}
\newcommand{\Verifiedshort}{CF Acc.}

\newcommand{\lstm}{\textsc{lstm}}
\newcommand{\treelstm}{\textsc{trlstm}}
\newcommand{\ibp}[1]{\widehat{#1}}
\newcommand{\concreteset}[1]{\bar{#1}}
\newcommand{\tightperturb}{S^=}
\newcommand{\tightperturbset}[1]{\textsc{dec}_{#1}}
\newcommand{\groundtruthset}{Q}

\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\newcommand{\perturbed}[1]{{\color{red}{#1}}}
\newcommand{\len}[1]{\textsc{len}_{#1}}
\newcommand{\maxlen}[1]{\textsc{maxlen}_{#1}}
\newcommand{\size}[1]{\textsc{size}_{#1}}
\newcommand{\reverse}{\emph{R}}


\newcommand{\TReviewFirst}[0]{T_{\emph{review}1}}
\newcommand{\TReviewSecond}[0]{T_{\emph{review}2}}
\newcommand{\TReviewThird}[0]{T_{\emph{review}3}}
\newcommand{\TReviewFourth}[0]{T_{\emph{review}4}}

==> LSTM%20robust%20training%20(EMNLP)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{fig~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Fig~\ref{#1}}
\def\Twofigref#1#2{Figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an table, lower-case.
\def\tblref#1{table~\ref{#1}}
% Reference to an table, upper case
\def\Tblref#1{Table~\ref{#1}}
% Reference to two Tables.
\def\twoTblrefs#1#2{Tables~\ref{#1} and~\ref{#2}}
% Reference to three Tables.
\def\threeTblrefs#1#2#3{Tables~\ref{#1},~\ref{#2} and~\ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{eq~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Eq~\ref{#1}}
% Reference to an example, lower-case.
\def\expref#1{ex.~\ref{#1}}
% Reference to an example, upper case
\def\Expref#1{Ex.~\ref{#1}}
% Reference to an lemma, lower-case.
\def\lemmaref#1{lemma~\ref{#1}}
% Reference to an lemma, upper case
\def\Lemmaref#1{Lemma~\ref{#1}}
% Reference to an theorem, lower-case.
\def\theref#1{theorem~\ref{#1}}
% Reference to an theorem, upper case
\def\Theref#1{Theorem~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> LSTM%20robust%20training%20(EMNLP)/pkgs.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage[group-separator={,}]{siunitx}
\usepackage{booktabs} % For formal tables
\usepackage{color}
\usepackage{listings}
\usepackage{enumitem}
\usepackage{threeparttable}
\usepackage{multirow}% http://ctan.org/pkg/multirow
\usepackage{hhline}% http://ctan.org/pkg/hhline
\usepackage{subfigure}
\usepackage{array}
\usepackage{pifont}
\usepackage{booktabs}
\usepackage{dsfont}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{stmaryrd}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{url}
\usepackage{bbm}
\usepackage{xspace}
\usepackage[normalem]{ulem}
\usepackage{booktabs, siunitx}
\usepackage[svgnames,table]{xcolor}
\usepackage[tableposition=above]{caption}
\usepackage{xcolor}
\usepackage{tkz-euclide}
\usepackage[framemethod=tikz]{mdframed}
\usepackage{empheq}
\usepackage[most]{tcolorbox}
\usepackage{adjustbox}
\usepackage{wrapfig}
\usepackage{hyperref}
\usepackage[capitalize]{cleveref}


\usepackage{balance}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\expandafter\def\expandafter\UrlBreaks\expandafter{\UrlBreaks%  save the current one
  \do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j%
  \do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t%
  \do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D%
  \do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N%
  \do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X%
  \do\Y\do\Z}


==> LSTM%20robust%20training%20(EMNLP)/sections/ablation.tex <==
\newpage
\subsection{Discussion}

\subsubsection{Ablation Study}
Alternatively, we can change the definition of $H_i^S$ to $C_i^S$:
\begin{align*}
    C_i^S = \bigcup_{j=0}^{L_{\bfx}}  \{\lstm(\bfz, \hstate_0)\mid \bfz \in S(\substring{\bfx}{1}{j}) \wedge L_{\bfz}=i\}
\end{align*}
%
By definition, the base case $C_0^\varnothing = \{0^d\}$. Notice that we do not require a tight perturbation space in the definition.

There are several disadvantages of defining $C_i^S$ in the above way:
\begin{itemize}
    \item $C_i^S$ overlap with each other, e.g., $C_i^{S_{-j}} \subseteq C_i^S$. While $H_i^S$ are disjoint unless different transformations lead to the same prefix.
    \item We have to enumerate all possible offsets for each state in $C_i^S$ because the original prefix lengths transformed by $S$ are unknown and different among the LSTM states in $C_i^S$. While the original prefix lengths transformed by $S^=$ are determined and the same among the LSTM states in $H_i^S$.
    \item The memoization of $C_i^S$ can be imprecise, i.e., containing infeasible states. While $H_i^S$ is precise.
\end{itemize}

For example, there are two states in the set $C^{\{(T_\emph{del}, 1)\}}_1$: $\lstm(\text{``to''}, \hstate_0)$ and $\lstm(\text{``the''}, \hstate_0)$. 

\textbf{Different offsets:}
For state $\lstm(\text{``to''}, \hstate_0)$, there are two possible original prefix: ``to'' (with offset 0) and ``to the'' (with offset -1). 
In other words, we can get transformed prefix ``to'' from the original prefix ``to'' by applying no transformations or from ``to the'' by applying deletion to word ``the''.

\textbf{Imprecision:}
Notice that we cannot tell what prefix has been proceeded by LSTM for each state in $C^{\{(T_\emph{del}, 1)\}}_1$. 
Because we cannot distinguish $\lstm(\text{``to''}, \hstate_0)$ with $\lstm(\text{``the''}, \hstate_0)$, we will generate states of ``to the'' (feasible), ``the the'' (infeasible) for $C^{\{(T_\emph{del}, 1)\}}_2$, resulting in imprecision. 

As we will show in the evaluation, this ablation version runs slower and certifies less test examples. 

\subsection{\textcolor{red}{new write up for memoization}}

\paragraph{Tight Perturbation Space} 

Think of the set of all strings
in a perturbation space as a tree, like in \cref{fig:approachfig}(b),
where strings that share prefixes
share LSTM states.
We want to characterize the set of LSTM
states at the $i$th layer of the tree
for prefixes that have had \emph{all} transformations in a space $S$ applied on the original prefix $\substring{\bfx}{1}{j}$.

We formally define  $H_{i,j}^S$ as follows:
\begin{align}
    H_{i,j}^S = \{\lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{j}) \wedge L_{\bfz}=i\} \label{eq: newcomplexstate}
\end{align}
By definition, the base case $H_{0,0}^\varnothing = \{0^d\}$.

\paragraph{Memoizing equation}
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.8\columnwidth]{imgs/illu_state_new.png}
    \caption{Illustration of two causes of \Eqref{eq:newcontransition1}}
    \label{fig:illu_state_new}
\end{figure*}


We now demonstrate how to rewrite \Eqref{eq: newcomplexstate}
by explicitly applying the transformations defining the perturbation space $S$, thus deriving our final equation:
\begin{align}
   H_{i,j}^S = & \bigcup_{\substack{1\leq k \leq |S|\\ \varphi_k(\substring{\bfx}{a}{b})=1}} \{\lstm(\bfz, h) \mid  \bfz \in f_k(\substring{\bfx}{a}{b}), h \in H_{i-t_k,j-s_k}^{S_{-k}}\}\nonumber \\
  &~~~~~~ \cup\ \{\lstm(x_{j}, h) \mid h \in H_{i-1,j-1}^S\} \label{eq:newcontransition1}
\end{align}
where 
$a {=} j {-} s_k + 1$ and
$b {=} j$.
Notation $S_{-k}$ denotes $S$
after reducing $\delta_k$ by 1;
therefore $S_{-k} \in \tightperturbset{S}$.

As illustrated in \Figref{fig:illu_state_new},
$H_{i,j}^S$ contains strings whose suffix is perturbed by $T_k = (\varphi_k,f_k)$ (the first line of \Eqref{eq:newcontransition1}), and strings whose suffixes are not perturbed by any transformations (the second line of \Eqref{eq:newcontransition1}). 
We compute \Eqref{eq:newcontransition1} in a bottom-up fashion, starting from $H_{0,0}^\varnothing=\{0^d\}$ and increasing $i,j$ and considering every possible perturbation space in the decomposition of $S$, $\tightperturbset{S}$.

\paragraph{Defining final states using prefixes}
Finally, we compute the set of final states, $F$, by considering all perturbation space in $\tightperturbset{S}$.
\begin{equation}
F = \bigcup_{S' \in \tightperturbset{S}} \bigcup_{i \ge 0} H_{i, L_{\bfx}}^{S'} \label{eq:newhfinal}
\end{equation}

\paragraph{Abstract memozing equations}
\begin{align*}
  \ibp{H}_{i,j}^S = & \bigsqcup_{\substack{1\leq k \leq |S|\\ \varphi_k(\substring{\bfx}{a}{b})=1}} \widehat{\lstm}(\alpha(f_k(\substring{\bfx}{a}{b})), \widehat{H}_{i-t_k,j-s_k}^{S_{-k}}) \\
  &~~~~~~\sqcup \ \widehat{\lstm}(\alpha(\{x_{j}\}), \widehat{H}_{i-1,j-1}^S)\\
%   \label{eq:abstract}~\\
\ \\
 \ibp{F} = & \bigsqcup_{S' \in \tightperturbset{S}} \bigsqcup_{i \ge 0}  \ibp{H}_{i, L_{\bfx}}^{S'} \nonumber
\end{align*}
where $a$ and $b$ are the same in \Eqref{eq:newcontransition1}.

The above abstract equations give us a compact overapproximation of $F$ that can be computed with a number of steps that is quadratic in the length of the input because we can have $O(\len{\bfx}^2)$ number of $H_{i,j}^S$ for a given $S$. 

\paragraph{Optimize the number of $H$'s} We now show that we can compute $\ibp{F}$ with a number of steps that is linear in the length of the input.

\begin{lemma}
\label{lemma: optimize_h}
For a given $i$ and $S$, define $j$ as 
\[j = \sum_{(T_k, \delta_k) \in S} (s_k - t_k)\delta_k + i \]
where $f_k: \alphabet^{s_k} \to 2^{\alphabet^{t_k}} $.
Then $H_{i,j'}^S = \varnothing$ for all $j' \neq j$.
\end{lemma}
\Lemmaref{lemma: optimize_h} tells us there is at most one non-empty $H_{i,j}^S$ for a given $i$ and $S$, which implies that there are only $O(L_x)$ number of non-empty $H_{i,j}^S$ for a given $S$.
We can prove a similar lemma for $\ibp{H}_{i,j}^S$ as well.

\begin{theorem}(Soundness \& Complexity)
\label{theorem: theorem4.2}
$F \subseteq \widehat{F}$ and the
number of LSTM cell evaluations needed is $O(L_{\bfx} n\prod_{i=1}^n \delta_i)$.
\end{theorem}

\newpage

==> LSTM%20robust%20training%20(EMNLP)/sections/approach.tex <==
\section{\toolname{}: Abstract Recursive Certification}
\label{sec:approach}
In this section, we present our technique for proving $S$-robustness of an LSTM
on $(\bfx,y)$.
Formally, we do this by computing the adversarial loss,
$\max_{\bfz \in S(\bfx)} L_\theta(\bfz,y)$.
Recall that
if the solution is $< 0$, then we have proven $S$-robustness.
%
To solve adversarial loss optimally, we effectively need to evaluate the LSTM on all of $S(\bfx)$ and collect all final states:
\begin{align}
F = \{\lstm(\bfz,h_0) \mid \bfz \in S(\bfx)\} \label{eq: theF}
\end{align}
Computing $F$  precisely is challenging,
as $S(\bfx)$ may be prohibitively large.
Therefore, we propose to compute a superset
of $F$, which we will call $\ibp{F}$.
%
This superset will therefore yield an upper bound on the adversarial loss. 
%
We prove $S$-robustness if the upper bound is $<0$.


To compute $\ibp{F}$, we present two key ideas
that go hand-in-hand:
 In \Secref{sec:concrete}, we observe that strings in the perturbation space share common prefixes,
and therefore we can \emph{memoize} hidden states to reduce the number of evaluations of LSTM cells---a form of dynamic programming.
We carefully derive the set of final states $F$
as a system of memoizing equations.
The challenge of this derivation is characterizing which strings share common prefixes without explicitly exploring the perturbation space.
In \Secref{sec:abstract},
we apply abstract interpretation
to efficiently and soundly solve the system of memoizing equations,
thus computing an overapproximation 
$\ibp{F} \supseteq F$.

% These  ideas result in an efficient approach 
% for computing $\ibp{F}$.
% that is linear\yh{polynomial?} in the length of the input string
% and the radius of the perturbation space (defined by $\delta_i$s).


% \input{sections/ablation}
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.8\columnwidth]{imgs/illu_state_new.png}
%     \caption{Illustration of two cases of \Eqref{eq:contransition1}}
% \end{figure*}

\begin{figure}[t]
    \centering
    \input{imgs/illu_state}
    \caption{Illustration of two cases of \Eqref{eq:contransition1}.}
    \label{fig:illu_state_new}
\end{figure}


\subsection{Memoizing Equations of Final States}
\label{sec:concrete}
% We now derive a set of
% memoizing equations defining $F$.
% We begin by showing how to characterize sets of
% intermediate states of an LSTM with respect to a perturbation space.


% \subsubsection{Defining prefix states}
\paragraph{Tight Perturbation Space} 
Given a perturbation space $S$, we shall use $\tightperturb{}$ 
to denote the \emph{tight} perturbation space where each transformation $T_j$ in $S$ is be applied \textbf{exactly} $\delta_j$ times. 

Think of the set of all strings
in a perturbation space as a tree, like in \cref{fig:approachfig}(b),
where strings that share prefixes
share LSTM states.
We want to characterize a subset $H_{i,j}^S$ of LSTM
states at the $i$th layer where the perturbed prefixes have had \emph{all} transformations in a space $S$ applied on the original prefix $\substring{\bfx}{1}{j}$.

We formally define  $H_{i,j}^S$ as follows:
\vskip -0.1in
\begin{small}
\begin{align}
    H_{i,j}^S = \{\lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{j}) \wedge \len{\bfz}=i\} \label{eq: complexstate}
\end{align}
\end{small}%
By definition, the base case $H_{0,0}^\varnothing = \{0^d\}$.



% \yh{only the following example uses the $T_\emph{del}$ by deleting `the` and `to`.}
\begin{example}
\label{ex: state}
Let $\bfx =$ ``\emph{to the movie}''.
Then, $H_{1,2}^{\{(T_\emph{del}, 1)\}} =\{\lstm(\emph{``the''},h_0), \lstm(\emph{``to''},h_0)\}$. 
These states result from deleting the first and second words of the prefix ``\emph{to the}'',
respectively.
We also have
$H_{2,2}^\varnothing = \{\lstm(\emph{``to the''}, h_0)\}$.
\end{example}

% The set of final states of strings in 
%  $\tightperturb{(\bfx)}$ are
% \begin{align}
%   \bigcup_{0 \le i \le \maxlen{\bfx}} H_{i,\len{\bfx}}^S \label{eq: finalstateoftight}
% \end{align}
% where $\maxlen{\bfx}$ is the upper bound of the length of the perturbed strings. $\maxlen{\bfx}$ can be overapproximated by
% \[\maxlen{\bfx} = \len{\bfx} + \sum_{(T_k, \delta_k) \in S} \max(t_k {-} s_k, 0)\delta_k\]
% where $f_k: \alphabet^{s_k} \to 2^{\alphabet^{t_k}} $.
% Because $t_k,s_k,\delta_k$ are small constants, we can regard $\maxlen{\bfx}$ as a term that is linear in the length of the original string $\len{\bfx}$, i.e., $\maxlen{\bfx} = O(\len{\bfx})$.

The set of final states of strings in 
 $\tightperturb{(\bfx)}$ is
\begin{align}
\bigcup_{i \ge 0} H_{i,\len{\bfx}}^S.
   \label{eq: finalstateoftight}
\end{align}

\paragraph{Memoizing equation}
We now demonstrate how to rewrite \Eqref{eq: complexstate} by explicitly applying the transformations defining the perturbation space $S$.
Notice that each $H_{i,j}^S$ comes from two sets of strings: (1) strings whose suffix (the last character) is not perturbed by any transformations (the first line of \Eqref{eq:contransition1}), and (2) strings whose suffix is perturbed by $T_k = (\varphi_k,f_k)$ (the second line of \Eqref{eq:contransition1}), as illustrated in \Figref{fig:illu_state_new}. 
Thus, we derive the final equation and then immediately show an example:
\vskip -0.1in
\begin{small}
\begin{align}
%   H_{i,j}^S = & \bigcup_{\substack{1\leq k \leq |S|\\ \varphi_k(\substring{\bfx}{a}{b})=1}} \{\lstm(\bfz, h) \mid  \bfz \in f_k(\substring{\bfx}{a}{b}), h \in H_{i-t_k,j-s_k}^{S_{k\downarrow{}}}\}\nonumber \\
%   &~~~~~~ \cup\ \{\lstm(x_{j}, h) \mid h \in H_{i-1,j-1}^S\} \label{eq:contransition1}
 &H_{i,j}^S = \{\lstm(x_{j}, h) \mid h \in H_{i{-}1,j{-}1}^S\} \cup \nonumber\\
 &\bigcup_{\substack{1\leq k \leq |S|\\ \varphi_k(\substring{\bfx}{a}{b})=1}} \{\lstm(\bfz, h) \mid  \bfz \in f_k(\substring{\bfx}{a}{b}), h \in H_{i{-}t_k,j{-}s_k}^{S_{k\downarrow{}}}\}\label{eq:contransition1}
\end{align}
\end{small}%
where 
$a {=} j {-} s_k + 1$ and
$b {=} j$.

We compute \Eqref{eq:contransition1} in a bottom-up fashion, starting from $H_{0,0}^\varnothing=\{0^d\}$ and increasing $i,j$ and considering every possible perturbation space in the decomposition of $S$, $\tightperturbset{S}$.

\begin{lemma}
\label{lemma:4.2}
 \Eqref{eq:contransition1} and \Eqref{eq: complexstate} are equivalent.
\end{lemma}

\begin{example}
% \yh{todo: example to show Eq 10.}
Consider computing $H_{1,2}^{\{(T_\emph{del}, 1)\}}$. 
We demonstrate how to derive states from \Eqref{eq:contransition1}:
\vskip -0.1in
\begin{small}
\begin{align}
%   H_{1,2}^{\{(T_\emph{del}, 1)\}} = & \{\lstm(\bfz, h) \mid  \bfz \in f_\emph{del}(\text{``the''}), h \in H_{1,1}^\varnothing\} \cup \nonumber \\
%   & \{\lstm(\text{``the''}, h) \mid h \in H_{0,1}^{\{(T_\emph{del}, 1)\}}\} \label{eq:concreteex}
H_{1,2}^{\{(T_\emph{del}, 1)\}} =&  \{\lstm(\text{``the''}, h) \mid h \in H_{0,1}^{\{(T_\emph{del}, 1)\}}\} \cup \nonumber \\
  & \{\lstm(\bfz, h) \mid  \bfz \in f_\emph{del}(\text{``the''}), h \in H_{1,1}^\varnothing\} \label{eq:concreteex}
\end{align}
\end{small}%
Assume $H_{1,1}^\varnothing=\{\lstm(\text{``to''}, h_0)\}$ and 
$H_{0,1}^{\{(T_\emph{del}, 1)\}}=\{h_0\}$ are computed in advance. 
The first line of \Eqref{eq:concreteex} evaluates to $\{\lstm(\text{``the''}, h_0)\}$, which corresponds to deleting the first word of the prefix ``to the''.
Because $\bfz$ can only be an empty string, the second line of \Eqref{eq:concreteex} evaluates to $\{\lstm(\text{``to''}, h_0)\}$, which corresponds to deleting the second word of ``to the''. 
The dashed green line in \cref{fig:approachfig}(b) shows the computation of \Eqref{eq:concreteex}.
\end{example}



\paragraph{Defining Final States using Prefixes}
Finally, we compute the set of final states, $F$, by considering all perturbation spaces in the decomposition of $S$.
%
%
\begin{equation}
F = \bigcup_{S' \in \tightperturbset{S}} \bigcup_{i \ge 0} H_{i,\len{\bfx}}^{S'} \label{eq:hfinal}
\end{equation}
% \yh{please check}
% Intuitively, assuming $S$ has a single transformation, $F$ is the union of final states of strings with $0$ transformations, exactly $1$ transformation, exactly $2$ transformations, etc. 

% \aws{note that in the equation above we shouldn't use $S^=$,
% because the "tightness" is implicit in the definition of $H_i^S$. I.e., you give it an $S$ and it treats it tightly.}

\begin{theorem}
\label{theorem: theorem4.1}
\Eqref{eq:hfinal} is equivalent to \Eqref{eq: theF}.
\end{theorem}


\begin{example}
Let $\spec=\{(T_\emph{del},1),(T_\emph{sub},1)\}$ and $\bfx=$``to the movie''.
$F$ is the union of four final states, $H_{3,3}^\varnothing$ (no transformations), $H_{2,3}^{\{(T_\emph{del}, 1)\}}$ (exactly 1 deletion), $H_{3,3}^{\{(T_\emph{sub}, 1)\}}$ (exactly 1 substitution), and $H_{2,3}^{\{(T_\emph{del}, 1), (T_\emph{sub}, 1)\}} $ (exactly 1 deletion and 1 substitution).
% Other $H_{i,j}^{S'}$ are either non-final or empty.
\end{example}

\subsection{Abstract Memoizing Equations}
\label{sec:abstract}
% We have characterized
% the set of final states $F$ as a memoizing system of equations.
Memoization avoids recomputing hidden states, but it still incurs a combinatorial explosion.
We employ abstract interpretation~\cite{DBLP:conf/popl/CousotC77} to solve the equations efficiently by overapproximating the set $F$.
See \citet{nnvbook} for details on abstractly interpreting neural networks.

\paragraph{Abstract Interpretation}
\label{sec: ibp_def}
The \emph{interval domain}, or \emph{interval bound propagation},
allows us to evaluate a function %
on an infinite set of inputs
represented as a hyperrectangle in $\mathbb{R}^n$.

\textit{Interval domain.}
We define the interval domain over scalars---the extension to vectors is standard.
We will use an interval $[l,u] \subset \mathbb{R}$, where $l,u\in\mathbb{R}$ and $l \leq u$,
to denote the set of all real numbers between $l$ and $u$, inclusive.
% We call  $l$ the lower bound and $u$ the upper bound.


For a finite set $X \subset \mathbb{R}$,
the \emph{abstraction} operator 
gives the tightest interval containing $X$,
as follows: $\alpha(X) = [\min(X),\max(X)]$.
Abstraction allows us to compactly represent a large set of strings.

\begin{example}
Suppose the words $x_1 = \emph{``movie''}$ and $x_2 = \emph{``film''}$
have the 1D embedding $0.1$
and $0.15$, respectively.
Then, $\alpha(\{x_1,x_2\}) = [0.1,0.15]$.
For $n$-dimensional embeddings,
we simply compute an abstraction of every dimension,
producing a vector of intervals.
\end{example}

The \emph{join} operation, $\sqcup$,
 produces the smallest interval containing two intervals:
 $[l,u] \sqcup [l',u'] = [\min(l,l'), \max(u,u')]$.
% Unlike in program analysis, join is rarely  used in network certification, due to lack of branching control-flow.
We will use joins to merge hidden states 
resulting from different strings in the perturbation space (recall \cref{fig:approachfig}(b)).

\begin{example}
Say we have two sets of 1D LSTM states
represented as intervals,
$[1,2]$ and $[10,12]$.
Then $[1,2] \sqcup [10,12] = [1,12]$.
Note that $\sqcup$ is an overapproximation of $\cup$,
introducing elements in neither interval.
\end{example}

\textit{Interval transformers.} 
To evaluate a neural network on  intervals,
we lift neural-network operations to interval arithmetic---%
\emph{abstract transformers}.
%
For a function $g$, we use $\ibp{g}$ to denote
its abstract transformer.
We use the transformers proposed by \citet{ai2,DBLP:conf/emnlp/JiaRGL19}.
We illustrate transformers for addition and any monotonically increasing function $g:\mathbb{R}\to\mathbb{R}$ (e.g., ReLU, tanh).
\vskip -0.1in
\begin{small}
\begin{align*}
    [l,u] \ibp{+}[l',u'] = [l+l', u+u'],\quad
    \quad \ibp{g}([l,u]) = [g(l),g(u)] 
\end{align*}
\end{small}%
Note how, for monotonic functions $g$, the
abstract transformer $\ibp{g}$ simply applies $g$
to the lower and upper bounds.


\begin{example}
When applying to the ReLU function,
 $\widehat{\mathrm{relu}}([-1,2]) = [\mathrm{relu}(-1),\mathrm{relu}(2)] = [0,2]$.
\end{example}

An abstract transformer
$\ibp{g}$
must be \emph{sound}: for any interval $[l,u]$
and $x \in [l,u]$, we have $g(x) \in \ibp{g}([l,u])$.
%
We use $\ibp{\lstm}$ 
to denote an abstract transformer of an LSTM cell.
It takes an interval of symbol embeddings and an interval of  states.
We use the definition of $\ibp{\lstm}$ given by \citet{DBLP:conf/emnlp/JiaRGL19}.

% \aws{i removed soundness}

% \paragraph{Soundness}
% An abstract transformer $\ibp{g}$ of a function $g$
% is said to be sound iff it overapproximates the results of
% $g$.
%
%  $\ibp{g}$
% is \emph{sound} iff for any interval $[l,u]$
% and any $x \in [l,u]$, we have $g(x) \in \ibp{g}([l,u])$.
% %
% Soundness is critical for certification,
% as we need  capture all final states $F$.


\paragraph{Abstract Memoizing Equations}
We now show how to solve
\Eqref{eq:contransition1}
and \Eqref{eq:hfinal} 
using abstract interpretation.
We do this by rewriting the equations 
using operations over intervals.
Let $\ibp{H}_{0,0}^\varnothing = \alpha(\{0^d\})$, then
\begin{align*}
%   \ibp{H}_{i,j}^S = & \bigsqcup_{\substack{1\leq k \leq |S|\\ \varphi_k(\substring{\bfx}{a}{b})=1}} \widehat{\lstm}(\alpha(f_k(\substring{\bfx}{a}{b})), \widehat{H}_{i-t_k,j-s_k}^{S_{-k}}) \\
%   &~~~~~~\sqcup \ \widehat{\lstm}(\alpha(\{x_{j}\}), \widehat{H}_{i-1,j-1}^S)\\
  \ibp{H}_{i,j}^S =&\ \widehat{\lstm}(\alpha(\{x_{j}\}), \widehat{H}_{i{-}1,j{-}1}^S) \ \sqcup \\ 
  &\bigsqcup_{\substack{1\leq k \leq |S|\\ \varphi_k(\substring{\bfx}{a}{b})=1}} \widehat{\lstm}(\alpha(f_k(\substring{\bfx}{a}{b})), \widehat{H}_{i{-}t_k,j{-}s_k}^{S_{k\downarrow{}}}) \\
%   \label{eq:abstract}~\\
 \ibp{F} = & \bigsqcup_{S' \in \tightperturbset{S}} \bigsqcup_{i \ge 0}  \ibp{H}_{i, \len{\bfx}}^{S'} \nonumber
\end{align*}
where $a$ and $b$ are the same in \Eqref{eq:contransition1}.


The two key ideas are (1) representing sets of possible LSTM inputs abstractly as intervals, using $\alpha$;
and (2) joining intervals of 
 states, using $\sqcup$.
%
These two ideas ensure that we 
efficiently solve the system of equations, producing an overapproximation $\ibp{F}$.


The above abstract equations give us a compact overapproximation of $F$ that can be computed with a number of steps that is linear in the length of the input. Even though we can have $O(\len{\bfx}^2)$ number of $H_{i,j}^S$ for a given $S$, only $O(\len{\bfx})$ number of $H_{i,j}^S$ are non-empty. This property is used in \Theref{theorem: theorem4.2} and will be proved in the appendix.
% \yh{I remove $\maxlen{\bfx}$, does the above still make sense?}

% \begin{example}
% Consider $\bfx=$``to the movie''.
% If $S=\{(T_\emph{del},1)\}$, states $H_{0,1}^S, H_{1,2}^S, H_{2,3}^S$ are non-empty. If $S =\{(T_\emph{sub},1)\}$, $H_{3,3}^S$ are non-empty.
% \end{example}


% \yh{merged the following theorems}
\begin{theorem}(Soundness \& Complexity)
\label{theorem: theorem4.2}
$F \subseteq \widehat{F}$ and the
number of LSTM cell evaluations needed to compute $\ibp{F}$ is $O(\len{\bfx}\cdot n\cdot\prod_{i=1}^n \delta_i)$.
\end{theorem}

For practical perturbations spaces (see \Secref{sec:evaluation}), the quantity $n\prod_{i=1}^n \delta_i$ is typically small and can be considered constant.

% We also make the assumption that
% the range of \emph{replace} functions $f_j$ can be abstracted offline.
% For example, if $f_j(x)$ defines the set of synonyms of a word $x$, we can compute $\alpha(f_j(x))$ offline for every word in the dictionary.
% %

% \aws{I think redrawing the running at this point with $H_i$ etc. would be very instructive} 

% \subsection{Ablation of Tight Perturbation Spaces}

\paragraph{Extension to Bi-LSTMs and Tree-LSTMs}\label{ssec:ext}
A \emph{Bi-LSTM} performs a forward and a backward pass on the input.  
The forward pass is the same as the forward pass in the original LSTM. 
For the backward pass, we reverse the input string $\bfx$, the input of the match function $\varphi_i$ and 
the input/output of the replace function $f_i$ of each transformation.

A \emph{Tree-LSTM} takes trees as input. We can define the programmable perturbation space over trees in the same form of \Eqref{eq:progspec}, where $T_i$ is a tree transformation.
We show some examples of tree transformations in \Figref{fig: treetrans}.
$\Tdelword{}$ (\Figref{fig:transdelstop}) removes a leaf node with a stop word in the tree. After removing, the sibling of the removed node becomes the new parent node.
$\Tinsword{}$ (\Figref{fig:transdup}) duplicates a word in a leaf node by first removing the word and expanding the leaf node with two children, each of which contains the previous word.
$\Tsubword{}$ (\Figref{fig:transsubsyn}) substitutes a word in the leaf node with one of its synonyms. 
\begin{figure}[!t]
    \centering\small
    \subfigure[$\Tdelword{}$: remove \textit{the}.]{\input{imgs/delstop}\label{fig:transdelstop}}
    \subfigure[$\Tinsword{}$: duplicate \textit{to}.]{\input{imgs/dup}\label{fig:transdup}}
    \subfigure[$\Tsubword{}$: substitute \textit{movie} with \textit{film}]{\input{imgs/subsyn}\label{fig:transsubsyn}}
    \caption{Examples of tree transformations.}
    \label{fig: treetrans}
\end{figure}

We provide the formalization of \toolname{} on Bi-LSTMs and Tree-LSTMs in the appendix.


==> LSTM%20robust%20training%20(EMNLP)/sections/approach_old.tex <==
\section{\toolname{}: Abstract Recursive Certification}
\label{sec:approach}
In this section, we present our technique for proving $S$-robustness of an LSTM
on $(\bfx,y)$.
Formally, we do this by computing the adversarial loss,
$\max_{\bfz \in S(\bfx)} L_\theta(\bfz,y)$.
Recall that
if the solution is $< 0$, then we have proven $S$-robustness.
%
To solve adversarial loss optimally, we effectively need to evaluate the LSTM on all of $S(\bfx)$ and collect all final states:
\begin{align}
F = \{\lstm(\bfz,h_0) \mid \bfz \in S(\bfx)\} \label{eq: theF}
\end{align}
Computing $F$  precisely is challenging,
as $S(\bfx)$ may be prohibitively large.
Therefore, we propose to compute a superset
of $F$, which we will call $\ibp{F}$.
%
This superset will therefore yield an upper bound on the adversarial loss. 
%
We prove $S$-robustness if the upper bound is $<0$.


To compute $\ibp{F}$, we present two key ideas
that go hand-in-hand:
 In \Secref{sec:concrete}, we observe that strings in the perturbation space share common prefixes,
and therefore we can \emph{memoize} hidden states to reduce the number of evaluations of LSTM cells---a form of dynamic programming.
We carefully derive the set of final states $F$
as a system of memoizing equations.
The challenge of this derivation is characterizing which strings share common prefixes without explicitly exploring the perturbation space.
In \Secref{sec:abstract},
we apply abstract interpretation
to efficiently and soundly solve the system of memoizing equations,
thus computing an overapproximation 
$\ibp{F} \supseteq F$.

% These  ideas result in an efficient approach 
% for computing $\ibp{F}$.
% that is linear\yh{polynomial?} in the length of the input string
% and the radius of the perturbation space (defined by $\delta_i$s).


\begin{figure*}[t]
    \centering
    \includegraphics[width=1.8\columnwidth]{imgs/illu_state_new.png}
    \caption{Illustration of two causes of \Eqref{eq:contransition1}}
    \label{fig:illu_state_new}
\end{figure*}


\subsection{Memoizing Equations of Final States}
\label{sec:concrete}
We now derive a set of
memoizing equations defining $F$.
We begin by showing how to characterize sets of
intermediate states of an LSTM with respect to a perturbation space.

\subsubsection{Defining prefix states}
\paragraph{Tight Perturbation Space} 
Given a perturbation space $S$, we shall use $\tightperturb{}$ 
to denote the \emph{tight} perturbation space where each transformation $T_j$ in $S$ is applied \textbf{exactly} $\delta_j$ times. 

% \aws{i rewrote this}
Think of the set of all strings
in a perturbation space as a tree, like in \cref{fig:approachfig}(b),
where strings that share prefixes
share LSTM states.
We want to characterize the set of LSTM
states at the $i$th layer of the tree
for prefixes that have had \emph{all} transformations in a space $S$ applied.
%
% We want to characterize 
% the set of possible $i$th LSTM states (i.e., the states resulting from reading the first $i$ words of each perturbed input) that the attacker can produce by applying \emph{all} transformations in $S$. 
We formally define  $H_i^S$ as follows:
\begin{align}
    H_i^S = \bigcup_{j=0}^{L_{\bfx}}  \{\lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{j}) \wedge L_{\bfz}=i\} \label{eq: complexstate}
\end{align}
%
By definition, the base case $H_0^\varnothing = \{0^d\}$.
% Informally,  $H_i^S$ looks at every prefix
% of $\bfx$ and considers perturbed strings of length $i$
% that can be produced by  $S^=$.



% \yh{only the following example uses the $T_\emph{del}$ by deleting `the` and `to`.}
\begin{example}
\label{ex: state}
Let $\bfx =$ ``\emph{to the movie}'',
and  $S = \{(T_\emph{del},1)\}$.
Then, $H_1^S =\{\lstm(\emph{``the''},h_0), \lstm(\emph{``to''},h_0)\}$. 
These states result from deleting the first and second words of the prefix ``\emph{to the}'',
respectively.
We also have
$H_2^\varnothing = \{\lstm(\emph{``to the''}, h_0)\}$.
\end{example}

% \yh{There are two intuitions for the offset. Here is the first one.}

% We need to enumerate the prefixes of input $\bfx$ because we do not know which prefix could result in the perturbed prefix $\bfz$ of length $i$. 
% However, the offset between the prefix length of $\bfx$ and the perturbed prefix length of $\bfz$ is a constant value because $\tightperturb{}$ is tight and each transformation $T_j^{s_j, t_j}$ restricts the input and output substring length.
% Thus, we simplify \Eqref{eq: complexstate} by tracking the offset between the perturbed input indexes and the original input indexes.

% \yh{Here is the second one.}
% In \Expref{ex: state}, $\concreteset{\hstate}_{1,\{(T_\emph{del},1)\}}$ comes from the initial state taking token $x_2$ and the initial state taking token $x_1$.
% As one can see, the index of token $x_2$ have been shifted when computing state $\concreteset{\hstate}_{1,\{(T_\emph{del},1)\}}$ because the transformation $T_\emph{del}$ alters the length of the perturbed string.
% Thus, we need to track the offset between the perturbed input indexes and the original input indexes.

\paragraph{Perturbation offset}
We will now  simplify the definition of $H_i^S$ using the 
notion of an \emph{offset}: a mapping between symbols of the original string and of a perturbed string.
Specifically, we compute the difference between the index $i$ of the perturbed string and the corresponding index of the original  string. 
We define $\offset_S$ as follows:
\[\offset_S = \sum_{(T_j, \delta_j) \in S} (t_j - s_j)\delta_j, \quad \text{ where } f_j: \alphabet^{s_j} \to 2^{\alphabet^{t_j}} \]
% where $s_j$ and $t_j$ are the size of the 
% domain and range of transformation $T_j = (\varphi_j,f_j)$,
% where $f_j: \alphabet^{s_j} \to 2^{\alphabet^{t_j}}$.
% \loris{maybe inline this last part in the formula}

% \begin{figure}[t]
%     \centering
%     \input{imgs/figure2}
%     \caption{Illustration of the offset $\offset_S$.}
%     \label{fig:mappingfig}
% \end{figure}




\begin{example}
Let $S=\{(T_\emph{del},1)\}$, the original string $\bfx$ = ``to the movie'', and the perturbed string $\bfz$ = ``to movie''. 
Then,
$\offset_S = (0 - 1)\times 1 = -1$.
Intuitively, $T_\emph{del}$ reduces the length of the string by 1.
The index 2 of the perturbed string $\bfz$ ($z_2=$``\emph{movie}'') corresponds to index $2 - \offset_S = 3$ in the original input string $\bfx$, where $x_3=$``\emph{movie}''.

\end{example}

We can simplify the definition in \Eqref{eq: complexstate} with the help of the offset $\offset_S$, as follows:
\begin{align}
    H_{i}^S = \{\lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S})\} \label{eq: simplestate}
\end{align}
The intuition is that strings of length $i$
in $H_i^S$ can only be produced by perturbing 
the prefix $\substring{\bfx}{1}{i-\offset_S}$,  because applying all transformations in $S$ will change the length of the string by $\offset_S$.

\begin{lemma}
\label{lemma:4.1}
\Eqref{eq: simplestate} is equivalent to \Eqref{eq: complexstate}.
\end{lemma}

By definition of offset,
we have the set of final states of strings in 
 $\tightperturb{(\bfx)}$ as $H_{L_{\bfx} + \offset_S}^S$.
\begin{align}
    H_{L_{\bfx} + \offset_S}^S = \{\lstm(\bfz, \hstate_0) \mid \bfz \in \tightperturb{}(\bfx)\} \label{eq: finalstateoftight}
\end{align}

\paragraph{Memoizing equation}
We now demonstrate how to rewrite \Eqref{eq: simplestate}
by explicitly applying the transformations defining the perturbation space $S$, thus deriving our final equation:
\begin{align}
   H_i^S = & \bigcup_{\substack{1\leq j \leq |S|\\ \varphi_j(\substring{\bfx}{a}{b})=1}} \{\lstm(\bfz, h) \mid  \bfz \in f_j(\substring{\bfx}{a}{b}), h \in H_{i-t_j}^{S_{-j}}\}\nonumber \\
  &~~~~~~ \cup\ \{\lstm(x_{i - \offset_S}, h) \mid h \in H_{i-1}^S\} \label{eq:contransition1}
\end{align}
where
$a {=} i {-} \offset_S {-} s_j {+} 1$ and
$b {=} i {-} \offset_S$.
Notation $S_{-j}$ denotes $S$
after reducing $\delta_j$ by 1;
therefore $S_{-j} \in \tightperturbset{S}$.

% \aws{discuss this paragraph...we should be very clear about these equations...and why they are memoizing}
% \yh{have rewritten the following. how about showing how to compute the example 4.1?}
% \aws{that'd be fantastic --- and perhaps an abstraction example too}

$H_i^S$ contains strings whose suffix is perturbed by $T_j = (\varphi_j,f_j)$ (the first line of \Eqref{eq:contransition1}), and strings whose  suffixes are not perturbed by any transformations (the second line of \Eqref{eq:contransition1}). 
We compute \Eqref{eq:contransition1} in a bottom-up fashion, starting from $H_0^\varnothing=\{0^d\}$ and increasing $i$ and considering every possible perturbation space in the decomposition of $S$, $\tightperturbset{S}$ (see Ex.~\ref{ex:decs}).
% \aws{check above}

\begin{example}
% \yh{todo: example to show Eq 10.}
Consider computing $H_1^{\{(T_\emph{del}, 1)\}}$, which is the set of two states 
$\lstm(\emph{``the''},h_0)$ and $\lstm(\emph{``to''},h_0)$. 
We demonstrate how to derive these two states from \Eqref{eq:contransition1}:
\begin{align}
   H_1^{\{(T_\emph{del}, 1)\}} = & \{\lstm(\bfz, h) \mid  \bfz \in f_\emph{del}(\text{``the''}), h \in H_{1}^\varnothing\} \cup \nonumber \\
  & \{\lstm(\text{``the''}, h) \mid h \in H_0^{\{(T_\emph{del}, 1)\}}\} \label{eq:concreteex}
\end{align}
We compute \Eqref{eq:contransition1} in a bottom-up fashion, so let us assume that we have computed $H_{1}^\varnothing=\{\lstm(\text{``to''}, h_0)\}$ and 
$H_{0}^{\{(T_\emph{del}, 1)\}}=\{h_0\}$ in advance. 
Because $\bfz$ can only be an empty string, the first line of \Eqref{eq:concreteex} evaluates to $\{\lstm(\text{``to''}, h_0)\}$, which corresponds to deleting the second words of the prefix ``to the'' and is memoized in $H_{1}^\varnothing$.
The second line of \Eqref{eq:concreteex} evaluates to $\{\lstm(\text{``the''}, h_0)\}$, which corresponds to deleting the first words of ``to the''. 
\end{example}

% The first line contains the set of states for 
% which the last symbol \loris{why just the last symbol?} is not perturbed by any transformation.
% The second line contains states of strings whose suffix is perturbed by $T_j = (\varphi_j,f_j)$.

% Informally, \Eqref{eq:contransition1} denotes that no transformation matches the input index $i - \offset_\tightperturb{}$, so we feed the original token $x_{i - \offset_\tightperturb{}}$ into the LSTM cell. \Eqref{eq:contransition2} denotes that a transformation $T_j=(f_j, \varphi_j)$ matches the substring $\substring{\bfx}{a}{b}$, so we feed all possible transformed substrings to the LSTM cell.

\begin{lemma}
\label{lemma:4.2}
 \Eqref{eq:contransition1} and \Eqref{eq: simplestate} are equivalent.
\end{lemma}

% Informally, \Eqref{eq:contransition1} denotes that no transformation matches the input index $i - \offset_S$, so we feed the original token $x_{i - \offset_S}$ into the LSTM cell.  denotes that a transformation $T_j=(f_j, \varphi_j)$ matches the substring $\substring{\bfx}{a}{b}$, so we feed all possible transformed substrings to the LSTM cell.



\subsubsection{Defining Final States using Prefixes}


% \yh{Better intuition than the following benefits?}The tight perturbation space can be seen as a rewritten history of the prefix input string, which has the following two benefits.
% First, the rewritten history helps us to group the perturbed strings with same length and to compute the mapping between the original input indexes and the perturbed input indexes.
% Second, the rewritten history helps us explore the perturbation space because it reflects which string transformations have been applied to the prefix and which string transformations can be applied to the remaining input string. 

Finally, we compute the set of final states, $F$, by considering all perturbation spaces in the decomposition of $S$.
%
%
\begin{equation}
F = \bigcup_{S' \in \tightperturbset{S}} H_{L_{\bfx} + \offset_{S'}}^{S'} \label{eq:hfinal}
\end{equation}
% \yh{please check}
Intuitively, assuming $S$ has a single transformation, $F$ is the union of final states of strings with $0$ transformations, exactly $1$ transformation, exactly $2$ transformations, etc. 

% \aws{note that in the equation above we shouldn't use $S^=$,
% because the "tightness" is implicit in the definition of $H_i^S$. I.e., you give it an $S$ and it treats it tightly.}

\begin{theorem}
\label{theorem: theorem4.1}
\Eqref{eq:hfinal} is equivalent to \Eqref{eq: theF}.
\end{theorem}

% \Theref{theorem: feasiblefstate} can be proved by using \Theref{theorem: theorem1} and \Eqref{eq: finalstateoftight}. 

\begin{example}
Let $\spec=\{(T_\emph{del},1),(T_\emph{sub},1)\}$.
$F$ is the union of four final states, $H_{3}^\varnothing$ (no transformations), $H_{2}^{\{(T_\emph{del}, 1)\}}$ (exactly 1 deletion), $H_{3}^{\{(T_\emph{sub}, 1)\}}$ (exactly 1 substitution), and $H_2^{\{(T_\emph{del}, 1), (T_\emph{sub}, 1)\}} $ (exactly 1 deletion and 1 substitution).
\end{example}

\subsection{Abstract Memoizing Equations}
\label{sec:abstract}
% We have characterized
% the set of final states $F$ as a memoizing system of equations.
Memoization avoids recomputing hidden states, but it still incurs in a combinatorial explosion.
We employ abstract interpretation~\cite{DBLP:conf/popl/CousotC77} to solve the equations efficiently by overapproximating the set $F$.

\subsubsection{Abstract Interpretation}
\label{sec: ibp_def}
The \emph{interval domain}~\cite{DBLP:conf/popl/CousotC77}, or \emph{interval bound propagation},
allows us to evaluate a function %
on an infinite set of inputs
represented as a hyperrectangle in $\R^n$.

\paragraph{Interval domain}
We define the interval domain over scalars---the extension to vectors is standard.
We will use an interval $[l,u] \subset \R$, where $l,u\in\R$ and $l \leq u$,
to denote the set of all real numbers between $l$ and $u$, inclusive.
% We call  $l$ the lower bound and $u$ the upper bound.


For a finite set $X \subset \R$,
the \emph{abstraction} operator 
gives the tightest interval containing $X$,
as follows: $\alpha(X) = [\min(X),\max(X)]$.
Abstraction allows us to compactly represent a large set of strings.

\begin{example}
Suppose the words $x_1 = \emph{``movie''}$ and $x_2 = \emph{``film''}$
have the 1D embedding $0.1$
and $0.15$, respectively.
Then, $\alpha(\{x_1,x_2\}) = [0.1,0.15]$.
For $n$-dimensional embeddings,
we simply compute an abstraction of every dimension,
producing a vector of intervals.
\end{example}

The \emph{join} operation, $\sqcup$,
 produces the smallest interval containing two intervals:
 $[l,u] \sqcup [l',u'] = [\min(l,l'), \max(u,u')]$.
% Unlike in program analysis, join is rarely  used in network certification, due to lack of branching control-flow.
We will use joins to merge hidden states 
resulting from different strings in the perturbation space (recall \cref{fig:approachfig}).

\begin{example}
Say we have two sets of 1D LSTM states
represented as intervals:
$[1,2]$ and $[10,12]$.
Then $[1,2] \sqcup [10,12] = [1,12]$.
Note that $\sqcup$ is an overapproximation of $\cup$,
introducing elements in neither interval.
\end{example}

\paragraph{Interval transformers} 
To evaluate a neural network on  intervals,
we lift neural-network operations to interval arithmetic---%
\emph{abstract transformers}.
%
For a function $g$, we use $\ibp{g}$ to denote
its abstract transformer.
We use the transformers proposed by \citet{ai2,DBLP:conf/emnlp/JiaRGL19}.
We illustrate transformers for addition and any monotonically increasing function $g:\mathbb{R}\to\mathbb{R}$ (e.g., ReLU, sigmoid, tanh).
%
\begin{align*}
    [l,u] \ibp{+}[l',u'] = [l+l', u+u'],\quad
    \quad \ibp{g}([l,u]) = [g(l),g(u)] 
\end{align*}
Note how, for monotonic functions $g$, the
abstract transformer $\ibp{g}$ simply applies $g$
to the lower and upper bounds.

% \begin{example}
% $[0,10] \ \ibp{+}\ [5,20] = [5,25]$.
% \end{example}
\begin{example}
For ReLU function $\mathrm{relu}(x) = \max(0,x)$,
applying $\widehat{\mathrm{relu}}([-1,2]) = [\mathrm{relu}(-1),\mathrm{relu}(2)] = [0,2]$.
\end{example}

An abstract transformer
$\ibp{g}$
must be \emph{sound}: for any interval $[l,u]$
and $x \in [l,u]$, we have $g(x) \in \ibp{g}([l,u])$.
%
We use $\ibp{\lstm}$ 
to denote an abstract transformer of an LSTM cell.
It takes an interval of symbol embeddings and an interval of  states.
We use the definition of $\ibp{\lstm}$ given by \citet{DBLP:conf/emnlp/JiaRGL19}.

% \aws{i removed soundness}

% \paragraph{Soundness}
% An abstract transformer $\ibp{g}$ of a function $g$
% is said to be sound iff it overapproximates the results of
% $g$.
%
%  $\ibp{g}$
% is \emph{sound} iff for any interval $[l,u]$
% and any $x \in [l,u]$, we have $g(x) \in \ibp{g}([l,u])$.
% %
% Soundness is critical for certification,
% as we need  capture all final states $F$.



\subsubsection{Abstract Memoizing Equations}
We now show how to solve
\Eqref{eq:contransition1}
and \Eqref{eq:hfinal} 
using abstract interpretation.
We do this by rewriting the equations 
using operations over intervals.
Let $\ibp{H}_0^\varnothing = \alpha(\{0^d\})$, then
%
%
\begin{align*}
  \ibp{H}_i^S = & \bigsqcup_{\substack{1\leq j \leq |S|\\ \varphi_j(\substring{\bfx}{a}{b})=1}} \widehat{\lstm}(\alpha(f_j(\substring{\bfx}{a}{b})), \widehat{H}_{i-t_j}^{S_{-j}}) \\
  &~~~~~~\sqcup \ \widehat{\lstm}(\alpha(\{x_{i - \offset_S}\}), \widehat{H}_{i-1}^S)\\
%   \label{eq:abstract}~\\
\ \\
 \ibp{F} = & \bigsqcup_{S' \in \tightperturbset{S}} \ibp{H}_{L_{\bfx} + \offset_{S'}}^{S'} \nonumber
\end{align*}
where $a$ and $b$ are the same in \Eqref{eq:contransition1}.

% All operations of LSTM cells have corresponding sound abstract transformers over intervals.

The two key ideas are (1) representing sets of possible LSTM inputs abstractly as intervals, using $\alpha$;
and (2) joining intervals of 
 states, using $\sqcup$.
%
These two ideas ensure that we 
efficiently solve the system of equations, producing an overapproximation $\ibp{F}$.

% \aws{possibly connect back to figure 1 here. Also maybe more intuition?}

% \aws{give an example of abstraction}

% \loris{above assumes we always abstract. I thought we abstract somtimes only (like greedily).}

% \aws{we should discuss how we algorithmically solve the equations }
% \paragraph{Complexity}
% Computing the abstract set of final states $\ibp{F}$ has a memory complexity of $O(L\prod_{i=1}^n \delta_i (\dhidden + \chidden))$, where $L$ is the maximum length of the output string. We have $O(L\prod_{i=1}^n \delta_i)$ numbers of $\ibp{\hstate}_{i,\spec'}$ because we need to iterate through all possible indexes of the output string and all the tight perturbation spaces in $\tightperturbset{S}$. Each $\ibp{\hstate}_{i,\spec'}$ is an interval bound, which has a size of $O(\dhidden + \chidden)$.

% The abstract equations achieve two goals:
% (1) an compact overapproximation of $F$,
% and (2)




The abstract equations give us a compact overapproximation of $F$
that can be efficiently computed with a number of
steps that is linear in the length of the input.
% The following theorem establishes \emph{soundness} of our 
% technique, enabling certification.
% The proof follows immediately from 
% the fact that $\alpha$, $\sqcup$, and $\ibp{\lstm}$
% overapproximate their inputs,
% resulting in an overapproximation $F$.


% \yh{merged the following theorems}
\begin{theorem}(Soundness \& Complexity)
\label{theorem: theorem4.2}
$F \subseteq \widehat{F}$ and the
number of LSTM cell evaluations needed is $O(L_{\bfx} n\prod_{i=1}^n \delta_i)$.
\end{theorem}

For practical perturbations spaces (see \Secref{sec:evaluation}), the quantity $n\prod_{i=1}^n \delta_i$ is small and can be considered constant.
% We also make the assumption that
% the range of \emph{replace} functions $f_j$ can be abstracted offline.
% For example, if $f_j(x)$ defines the set of synonyms of a word $x$, we can compute $\alpha(f_j(x))$ offline for every word in the dictionary.
% %

% \aws{I think redrawing the running at this point with $H_i$ etc. would be very instructive} 

\subsection{Extension to Bi-LSTMs and Tree-LSTMs}\label{ssec:ext}
% \yh{todo: make the merge smooth}
A \emph{Bi-LSTM} performs a forward and a backward pass on the input.  
The forward pass is the same as the forward pass in the original LSTM. 
For the backward pass, we reverse the input string $\bfx$, the input of the match function $\varphi_i$ and 
the input/output of the replace function $f_i$ of each transformation.
% \loris{A little more detail?}

A \emph{Tree-LSTM} takes trees as input. We can define the programmable perturbation space over trees in the same form of \Eqref{eq:progspec}, where $T_i$ is a tree transformation.
We show some examples of tree transformations in \Figref{fig: treetrans}.
$\Tdelword{}$ (\Figref{fig:transdelstop}) removes a leaf node with a stop word in the tree. After removing, the sibling of the removed node becomes the new parent node.
$\Tinsword{}$ (\Figref{fig:transdup}) duplicates a word in a leaf node by first removing the word and expanding the leaf node with two children, each of which contains the previous word.
$\Tsubword{}$ (\Figref{fig:transsubsyn}) substitutes a word in the leaf node with one of its synonyms. 
\begin{figure}[!t]
    \centering\small
    \subfigure[$\Tdelword{}$: remove ``the''.]{\input{imgs/delstop}\label{fig:transdelstop}}
    \subfigure[$\Tinsword{}$: duplicate ``to''.]{\input{imgs/dup}\label{fig:transdup}}
    \subfigure[$\Tsubword{}$: substitute ``movie'' with ``film'']{\input{imgs/subsyn}\label{fig:transsubsyn}}
    \caption{Examples of tree transformations.}
    \label{fig: treetrans}
\end{figure}

We provide the formalization of \toolname{} on Bi-LSTMs and Tree-LSTMs in the supplementary material.


==> LSTM%20robust%20training%20(EMNLP)/sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
%\footnote{anonymous link}
% \aws{add machine details to supp}
% We conduct all experiments on a server running Ubuntu 18.04.5 LTS with V100 32GB GPUs and Intel Xeon Gold 5115 CPUs running at 2.40GHz.
% In this section, we evaluate \toolname{} by answering the following research questions:
% \begin{description}
%     \item[RQ1:] Does \toolname{} improve robustness in rich perturbation spaces for LSTM, Tree-LSTM, and Bi-LSTM?
%     % \item[RQ2:] How does \toolname{} compare to baselines\loris{how is this question different than the previous one?} \yh{baselines that cannot handle general transformations or certify the robustness.}?
%     \item[RQ2:] How does the size of the perturbation space affect the effectiveness of \toolname{}?
% \end{description}

% \subsection{Experimental Setup}
We implemented \toolname{} in PyTorch.
The source code is available online\footnote{\url{https://github.com/ForeverZyh/certified_lstms}} and provided in the supplementary materials.

\paragraph{Datasets}
We use three datasets:  \emph{IMDB}~\cite{imdbdataset}, \emph{Stanford Sentiment Treebank} (SST)~\cite{sst2}, and SST2, a two-way class split of SST.
% All datasets consist of movie reviews and human annotations of their sentiment. 
IMDB and SST2 have reviews in sentence form and binary labels. 
SST has reviews in the \emph{constituency parse tree} form and five labels.

% \aws{say something that Trees and Bi are in Appendix early on}
\paragraph{Perturbation Spaces}
\input{tables/string_trans}
Following~\citet{ZhangAD20}, we create perturbation spaces by combining the transformations in \Tblref{tab:perturbation}, e.g., $\SDS$ removes up to two stop words and replaces up to two words with synonyms.
We also design a domain-specific perturbation space $\reviewperturb{}$ for movie reviews; e.g., one transformation in $\reviewperturb{}$ can duplicate question or exclamation marks because they usually appear repeatedly in movie reviews.
We provide the detailed definition and evaluation of $\reviewperturb{}$ in the appendix.

For Tree-LSTMs, we consider the tree transformations exemplified in~\Figref{fig: treetrans} and described in \Secref{ssec:ext}.

\paragraph{Evaluation metrics} 
(1)
\emph{Accuracy} (Acc.) is the vanilla test accuracy.
(2)
\emph{HotFlip accuracy} (HF Acc.) is the adversarial accuracy with respect to the HotFlip attack~\cite{ebrahimi2018hotflip}: for each point in the test set, we use HotFlip to generate the top-5 perturbed examples and test if the classifications are correct on all the 5 examples and the original example.
%
% \aws{certification accuracy? for consistent terminology} 
(3)
\emph{Certified accuracy} (\Verifiedshort{}) 
is the percentage of points in the test set
certified as $S$-robust (\Eqref{eq:robustness}) using \toolname{}.
% \loris{explain what this means}
(4)
\emph{Exhaustive accuracy} (\Exhaustiveshort{}) is the 
percentage of points in the test set that is $S$-robust (\Eqref{eq:robustness}).
HotFlip accuracy is an upper bound of exhaustive accuracy; certified accuracy is a lower bound of exhaustive accuracy.

% In RQ2, we also use random smoothing~\cite{DBLP:conf/acl/YeGL20} to certify the accuracy of the model. 

% \aws{We might want to present this one later}

% \textbf{RS accuracy} 
%  is the accuracy certified by random smoothing~\cite{DBLP:conf/acl/YeGL20}: a prediction on $(\bfx, y)$ is considered correct if and only if more than half of perturbed samples in $S(\bfx)$ are correctly classified with $1\%$ significance level.


\paragraph{Baselines}
%
For training certifiable models against arbitrary string transformations, we compare \toolname{} to (1) \emph{Normal training} that minimizes the cross entropy. (2) \emph{Data augmentation} that augments the dataset with random samples from the perturbation space. (3) \emph{HotFlip~\cite{ebrahimi2018hotflip}} adversarial training.
And (4) \emph{A3T~\cite{ZhangAD20}} that trains robust CNNs.

For training certifiable models against word substitution, we compare \toolname{} to (1) \emph{\citet{DBLP:conf/emnlp/JiaRGL19}} that trains \emph{certifiably} robust (Bi)LSTMs. We call this \jiaapproach{} in the rest of this section. (2) \emph{ASCC~\cite{dong2021towards}} that trains \emph{empirically} robust (Bi)LSTMs. And (3) \emph{\citet{DBLP:conf/emnlp/HuangSWDYGDK19}} that trains \emph{certifiably} robust CNNs (comparison results are in the appendix).

For certification, we compare \toolname{} to (1) \emph{POPQORN~\cite{POPQORN}}, the state-of-the-art approach for certifying LSTMs. (2) \emph{SAFER~\cite{DBLP:conf/acl/YeGL20}} that provides probabilistic certificates to word substitution.

\emph{\citet{DBLP:conf/nips/XuS0WCHKLH20}} is a special case of \toolname{} where the perturbation space only contains substitution. We provide theoretical comparison in the appendix.

\input{tables/qexample}

\subsection{Arbitrary Perturbation Spaces}

% We first compare \toolname{} to approaches that can handle arbitrary spaces: data augmentation, HotFlip, and A3T.
\input{tables/lstm_whole}

\textbf{Comparison to Data Augmentation \& HotFlip.}
% We compare to these two baselines on four perturbation spaces
% shown in \twoTblrefs{tab:lstm}{tab:compare_DSreview}.
%$\{(\Tdelword{}, 2), (\Tsubword{}, 2)\}$, $\{(\Tinsword{},2), (\Tsubword{},2)\}$, $\{(\Tdelword{},2), (\Tinsword{},2)\}$, and $\reviewperturb{}$.
We use the three perturbation spaces in \Tblref{tab:lstm_whole} and the domain-specific perturbation space $\reviewperturb{}$ in \Tblref{tab:compare_DSreview}.

\textbf{\textit{\toolname{} 
 outperforms 
data augmentation and HotFlip in terms of \Exhaustiveshort{} and \Verifiedshort{}
}}
\Tblref{tab:lstm_whole} shows the results of LSTM, Tree-LSTM, and Bi-LSTM models on the tree perturbation spaces.
\Tblref{tab:compare_DSreview} shows the results of LSTM models on the domain-specific perturbation space $\reviewperturb{}$.
\toolname{} has significantly higher \Exhaustiveshort{}
than normal training ($+8.1, +14.0, +8.7$ on average), data augmentation ($+4.2, +10.4, +5.0$), and HotFlip ($+3.6, +6.7, +10.4$) for LSTM, Tree-LSTM, and Bi-LSTM respectively. 

Models trained with \toolname{} have a relatively high \Verifiedshort{} ($53.6$ on average). 
Data augmentation and HotFlip 
result in models not amenable to certification---in some cases, almost nothing in the test set can be certified.

\toolname{} produces more robust models at the expense of accuracy. 
Other robust training approaches like \jiaapproach{} and A3T also exhibit this trade-off.
However, as we will show next, \toolname{} retains higher accuracy than these approaches.
% Moreover, \toolname{} retains higher accuracy than data augmentation and HotFlip for $\reviewperturb{}$.

\input{tables/comparea3t_whole} 
\paragraph{Comparison to A3T}
% We compare \toolname{} against A3T using $\SDS$ and $\SIS$. 
% We do not use $\SDI$ because A3T degenerates to HotFlip training for this perturbation space.
A3T degenerates to HotFlip training on $\SDI$, so we do not use this perturbation space.
%We download two models from the A3T website for comparison.\footnote{\url{github.com/ForeverZyh/A3T}}

\textbf{\textit{
The LSTMs trained using \toolname{} are more robust than the CNNs trained by A3T for both perturbation spaces; \toolname{} can certify the robustness of models while A3T cannot.}}
\Tblref{tab:compare_a3twhole} shows that
\toolname{} results in models with higher accuracy ($+2.3$ and $+0.3$), HF Acc. ($+5.9$ and $+1.7$), and \Exhaustiveshort{} ($+6.8$ and $+6.3$) than those produced by A3T. 
\toolname{} can certify the trained models while A3T cannot.
% \Tblref{tab:compare_a3t} shows the results of the perturbation space $\SDS$ (results of $\SIS$ are in the appendix).

% \yh{move it here.} We can apply the idea of A3T to \toolname{}, extending \toolname{} to abstract any subset of the given perturbation space and to augment the remaining perturbation space. We show the effectiveness of this extension in the appendix.

\subsection{Experiments on Word Substitution}
We compare to
works \emph{limited} to word substitution.

% \loris{following para can still be cleaned}
\input{tables/comparejia}

\paragraph{Comparison to \jiaapproach{} and ASCC} We choose two perturbation spaces, $\{(\Tsubword{}, 1)\}$ and $\{(\Tsubword{}, 2)\}$.
% \loris{following sentence is so confusing. Is it 2 models, 2 models per perturbations?}
We train one model per perturbation space using \toolname{} under the same experimental setup of \jiaapproach{}, BiLSTM on the IMDB dataset.
%provided in their paper, i.e., the same dataset (IMDB), synonym sets, and the Bi-LSTM architecture.
By definition, \jiaapproach{} and ASCC
train for an arbitrary number of substitutions.
\Verifiedshort{} is computed using \toolname{}. 
Note that \jiaapproach{} can only certify for $\{(\Tsubword{}, \infty)\}$ and ASCC cannot certify.
%We download the trained model from their website and evaluate it on $\{(\Tsubword{}, 1)\}$ and $\{(\Tsubword{}, 2)\}$.\footnote{\url{github.com/robinjia/certified-word-sub}}


\textbf{\textit{\toolname{} trains more robust models than \jiaapproach{} for two perturbation spaces with word substitution.}}
\Tblref{tab:compare_jia} shows that \toolname{} achieves higher accuracy, 
% ($+10.9$ and $+9.5$, respectively)
\Verifiedshort{}, 
% ($+10.8$ and $+6.2$, respectively)
and \Exhaustiveshort{} 
% ($+11.6$ and $+9.9$, respectively) 
than \jiaapproach{} on the two perturbation spaces.

% \paragraph{Comparison to ASCC.} We use the same perturbation spaces and the same model structure as in the comparison to \jiaapproach{}. 
%We train the model using their code.\footnote{\url{https://github.com/dongxinshuai/ASCC}}. 

\textbf{\textit{\toolname{} trains a more robust model than ASCC for $\{(\Tsubword{}, 1)\}$, but ASCC's model is more robust for $\{(\Tsubword{}, 2)\}$.}}
% \yh{results are not ready.}
% \toolname{} trains a more robust model ($+1.1$ \Exhaustiveshort{}) than \toolname{} for $\{(\Tsubword{}, 1)\}$, but ASCC's model is more robust (\yh{$+X.X$} \Exhaustiveshort{}) for $\{(\Tsubword{}, 2)\}$.
\Tblref{tab:compare_jia} shows that the \toolname{}-trained models have higher accuracy
%($+4.9$ and $+3.5$, respectively) 
and \Verifiedshort{}
%($+77.8$ and $+71.0$, respectively).


\paragraph{Comparison to POPQORN} We compare the certification of an \toolname{}-trained model and a normal model against $\{(\Tsubword{}, 3)\}$ on the first 100 examples in SST2 dataset. Because POPQORN can only certify the $l_p$ norm ball, we overapproximate the radius of the ball as the maximum $l_1$ distance between the original word and its synonyms. 

\textbf{\emph{\toolname{} runs much faster than POPQORN. \toolname{} is more accurate than POPQORN on the \toolname{}-trained model, while POPQORN is more accurate on the normal model.}} \toolname{} certification takes 0.17sec/example on average for both models, while POPQORN certification takes 12.7min/example. \toolname{} achieves 67\% and 5\% \Verifiedshort{} on \toolname{}-trained model and normal model, respectively, while POPQORN achieves 22\% and 28\% \Verifiedshort{}, but crashes on 45\% and 1\% of examples for two models.



\paragraph{Comparison to SAFER~\cite{DBLP:conf/acl/YeGL20}} 
SAFER is a post-processing technique for
certifying robustness via \emph{randomized smoothing}.
% Therefore, we can apply it to \toolname{} models.
% We compute the randomized smoothing accuracy using the perturbation spaces $\{(\Tsubword{}, 1)\}$ and $\{(\Tsubword{}, 2)\}$---randomized smoothing has not been studied for perturbation spaces involving deletions and insertions.
%
%
We train a Bi-LSTM model using \toolname{}
following SAFER's experimental setup on the IMDB dataset
and SAFER's synonym set, which is different from \jiaapproach{}'s.
We consider the perturbation spaces $\{(\Tsubword{}, 1)\}$ and $\{(\Tsubword{}, 2)\}$.
We use both \toolname{} and SAFER to certify the robustness.
The significance level of SAFER is set to $1\%$.

\textbf{\emph{SAFER has a higher certified accuracy than \toolname{}. However, 
its certificates are statistical, tied to word substitution only,
and are slower to compute.}}
Considering $\{(\Tsubword{}, 2)\}$, \toolname{} results in a certified accuracy of 79.6 and SAFER results in a certified accuracy of 86.7 (see appendix). 
Note that certified accuracies are incomparable because SAFER computes certificates
that only provide statistical guarantees.
% However, we observe higher randomized smoothing accuracy
% by applying SAFER to models trained using data augmentation instead of ARC (e.g., 89.7 vs. 86.7).
Also, note that ARC uses $O(n\prod_{i=1}^n \delta_i)$ forward passes for each sample, while SAFER needs to randomly sample thousands of times.  
In the future, it would be interesting to explore 
extensions of SAFER to \toolname{}'s rich perturbation spaces.

\subsection{ Effects of Perturbation Space Size} 
\begin{figure}[t]
    \centering
    % \vspace{-4mm}
    % \aws{y axis: "size of perturbation space"}
     \includegraphics[width=0.75\columnwidth]{imgs/RQ3.pdf}
    \caption{Accuracy metrics and the maximum perturbation space size as $\delta$ varies from 1 to 5 for $\{(\Tinsword{},\delta), (\Tsubword{},\delta)\}$.}
    \label{fig:RQ3}
\end{figure}


We fix the LSTM model (\Tblref{tab:lstm_whole}) trained using \toolname{} on $\SIS$ and SST2.
Then, we test this model’s \Verifiedshort{} and HotFlip accuracy on $\{(\Tinsword{},\delta), (\Tsubword{},\delta)\}$ by varying $\delta$ from 1 to 5.
We evaluate the \Exhaustiveshort{} only for $\delta=1,2,3$, due to the combinatorial  explosion. 

\textbf{\textit{\toolname{} maintains a reasonable \Verifiedshort{} for increasingly larger spaces}.} \Figref{fig:RQ3} shows the results, along with the maximum perturbation space size in the test set.
\toolname{} can certify $41.7\%$ of the test set even when the perturbation space size grows to about $10^{10}$.
For $\delta=1,2,3$, the \Verifiedshort{} is lower than the \Exhaustiveshort{} ($8.2$ on average), while the HF Acc. is higher than the \Exhaustiveshort{} ($5.6$ on average).
Note that \toolname{} uses a small
amount of time to certify the entire test set, $3.6$min on average,
using a single V100 GPU,
making it incredibly efficient compared
to brute-force enumeration.
% \aws{check}
% than HotFlip attack ($14.4$ minutes on average) to compute the bound. 
% \aws{give the amount of time it takes ARC to do verification}

==> LSTM%20robust%20training%20(EMNLP)/sections/intro.tex <==
\section{Introduction}
Adversarial examples are small perturbations of an input that fool a neural network into changing its prediction~\cite{DBLP:conf/ccs/Carlini017, DBLP:journals/corr/SzegedyZSBEGF13}.
%
In NLP, 
adversarial examples involve modifying an input string
by, for example, replacing words with synonyms, deleting stop words, inserting words, etc.~\cite{ebrahimi2018hotflip, DBLP:conf/ndss/LiJDLW19, DBLP:conf/acl/ZhangZML19}.
% Adversarial examples rise security concerns for all real-world applications that run on DNN.

% Over the past few years, researchers have developed a promising arsenal of \emph{defense} techniques against adversarial examples in NLP tasks, resulting in models that are increasingly \emph{robust} to adversarial inputs. 
Ideally, a \emph{defense}  against adversarial examples in NLP tasks
should fulfill the following desiderata: (1) Handle \textbf{recursive models}, like LSTMs and extensions thereof, which are prevalent in NLP. (2) Construct \textbf{certificates} (proofs) of robustness. (3) Defend against \textbf{arbitrary string transformations}, like combinations of word deletion, insertion, etc.

\begin{figure}[t]
    \centering
    \input{imgs/figure1}
    \caption{An illustration of our approach.}
    \label{fig:approachfig}
\end{figure}

It is quite challenging to fulfill all three desiderata;
indeed, existing techniques are forced to make tradeoffs.
For instance,
the theoretical insights underlying a number of certification approaches are intimately tied to symbol substitution~\cite{DBLP:conf/emnlp/JiaRGL19,DBLP:conf/emnlp/HuangSWDYGDK19,DBLP:conf/acl/YeGL20, DBLP:conf/nips/XuS0WCHKLH20, dong2021towards},
and some techniques cannot handle recursive models~\cite{DBLP:conf/emnlp/HuangSWDYGDK19, ZhangAD20}.
%
On the other hand, techniques that strive to be robust
to arbitrary string transformations achieve this  at the expense of  certification~\cite{ZhangAD20,ebrahimi2018hotflip}.

In this paper, we ask:
Can we develop a \emph{certified} defense to \emph{arbitrary string transformations} that applies to \emph{recursive neural networks}?

\paragraph{Our approach}
Certifying robustness involves proving that
a network's prediction is the same no matter how a given input string is perturbed. 
%
We assume that the \emph{perturbation space} is defined as a program
describing a set of possible  string transformations~\cite{ZhangAD20}---e.g., \emph{if you see the word ``movie'', replace it with ``film'' or ``movies''}.
Such transformations can succinctly define a  perturbation space that is exponentially large in the length of the input;
so, certification by enumerating the perturbation space is generally impractical. 

We present  \toolname{} (Abstract Recursive Certification),
an approach for \textit{certifying} robustness to programmatically defined perturbation spaces. \toolname{} can be used within an adversarial training loop
to \textit{train robust models}.
We illustrate the key ideas behind \toolname{} through a simple example.
Consider the (partial) input sentence \emph{to the movie...},
and say we are using an LSTM for prediction.
Say we have two string transformations:
(\textbf{T1}) If you see the word \emph{movie}, you can replace it with \emph{film} or \emph{movies}.
(\textbf{T2}) If you see the word \emph{the} or \emph{to}, you can delete it.
ARC avoids enumerating the large perturbation space (\cref{fig:approachfig}(a))
using two key insights.

\emph{Memoization}:
 \toolname{} exploits the recursive structure of LSTM networks, and their extensions (BiLSTMs, TreeLSTMs),
to avoid recomputing intermediate hidden states.
\toolname{}  \emph{memoizes} hidden states of prefixes shared across
multiple sequences in the perturbation space.
For example, the two sentences 
\emph{to the movie...} and \emph{to the film...}.
share the prefix \emph{to the},
and therefore we memoize the hidden state
after the word \emph{the}, as illustrated in \cref{fig:approachfig}(b) with dashed blue lines.
% We carefully derive a memoizing set of equations
% that captures the structure of programmatically
% defined string transformations.
The critical challenge is characterizing 
which strings share prefixes without having to explicitly explore the perturbation space.

% \loris{sentences below can go IMHO}
% So, instead of evaluating the LSTM from scratch on the second sentence, we can start the evaluation from the hidden state after \emph{the}, and just evaluate the LSTM on \emph{film...}.
% This form of \emph{dynamic programming} \yh{not sure if we still call this DP} is illustrated in \cref{fig:approachfig}(b).

\emph{Abstraction}:
 \toolname{} uses \emph{abstract interpretation}~\cite{DBLP:conf/popl/CousotC77} to symbolically 
represent sets of perturbed strings,
avoiding a combinatorial explosion.
Specifically, \toolname{} represents a set of strings as a hyperrectangle
in a $\mathbb{R}^n$
and propagates the hyperrectangle through the network
using interval arithmetic~\cite{ai2, DBLP:conf/iccv/GowalDSBQUAMK19}.%---each dimension of a hyperrectangle is an interval of possible values.
This idea is illustrated in \cref{fig:approachfig}(b),
where the words \emph{film} and \emph{movies} are represented as a hyperrectangle.
% Note how the words \emph{film} and \emph{movies} are represented as a single hyperrectangle, using the abstraction function $\alpha$.
% \yh{not greedily though. we merge branches that are in the same tight perturbation space.}
By \emph{joining} hidden states of different sentences (a common idea in program analysis), 
\toolname{} can perform certification efficiently.


Memoization and abstraction enable
ARC to efficiently certify robustness to
very large perturbation spaces.
% \aws{move Xu et comparison here, saying we subsume it}
Note that \toolname{} subsumes \citet{DBLP:conf/nips/XuS0WCHKLH20} because \toolname{} can certify arbitrary string transformations, while \citet{DBLP:conf/nips/XuS0WCHKLH20} only works on word substitutions.

% \aws{cite more ibp papers, in addition to ai2}

% \loris{add sec numbers to contrib}
\paragraph{Contributions}
We make the following contributions:
(1) We present \toolname{},
an approach   for training certifiably robust recursive neural networks.
    We demonstrate our approach on LSTMs, BiLSTMs, and TreeLSTMs.
(2) We present a novel application of abstract interpretation to 
    symbolically capture a large space of strings, defined programmatically,
    and propagate it through a recursive network (\Secref{sec:approach}).
(3) Our evaluation shows that \toolname{} can train models that are more robust to arbitrary perturbation spaces than those produced by existing techniques; \toolname{} can show high certification accuracy of the resulting models; and \toolname{} can certify robustness to attacks (transformations) that are out-of-scope for existing techniques (\Secref{sec:evaluation}). 


==> LSTM%20robust%20training%20(EMNLP)/sections/old_proof.tex <==
\subsection{Proof of Lemmas and Theorems}

\textbf{\Lemmaref{lemma:4.1}}
\begin{proof}
Taking the difference of \Eqref{eq: complexstate} and \Eqref{eq: simplestate}, we need to prove
\begin{small}
\begin{align}
 &\bigcup_{j=0, j\neq i - \offset_S}^{L_{\bfx}}  \{ \bfz \mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{j}) \wedge L_{\bfz}=i\} = \varnothing \label{eq: lemma4.1_1}\\
&\left\{ 
\begin{aligned}
   \bfz \mid &\bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S}) \\
   &\wedge L_{\bfz}=i
\end{aligned}
\right\} = \{ \bfz \mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S})\} \label{eq: lemma4.1_2}
\end{align}
\end{small}

\Eqref{eq: lemma4.1_1} denotes that all other sets are empty except for $j=i - \offset_S$ in \Eqref{eq: complexstate}. \Eqref{eq: lemma4.1_2} denotes the set at $j=i - \offset_S$ in \Eqref{eq: complexstate} is the same as the set in \Eqref{eq: simplestate}.

By the definition of the offset, \Eqref{eq: lemma4.1_1} is true because $\tightperturb{}(\substring{\bfx}{1}{j})$ contains strings $\bfz$ where $\len{\bfz} = j + \offset_S$, i.e., $\len{\bfz} \neq i$.
Similarly, \Eqref{eq: lemma4.1_2} is true because $\tightperturb{}(\substring{\bfx}{1}{i - \offset_S})$ only contains strings $\bfz$ such that $\len{\bfz}=i$.
\end{proof}

\textbf{\Lemmaref{lemma:4.2}}
\begin{proof}
We prove \Lemmaref{lemma:4.2} by induction on $i$ and $S$. 

\textbf{Base case:} $H_0^\varnothing = {h_0}$ is defined by both \Eqref{eq: simplestate} and \Eqref{eq:contransition1}.

\textbf{Inductive step:} Suppose the lemma holds for $H_j^{S'}$, where $(0\le j \le i \wedge S' \subset S) \vee (0\le j < i \wedge S' \subseteq S)$. 
$S' \subseteq S$ denotes that for all $(T_k, \delta_k') \in S'$, we have $(T_k, \delta_k) \in S$ and $\delta_k' \le \delta_k$. And $S' \subset S$ denotes that $S' \subseteq S$ and there exists a transformation $T_k$ such that $(T_k, \delta_k') \in S' \wedge (T_k, \delta_k) \in S$ and $\delta_k' < \delta_k$.

The computation of $H_i^S$ contains strings whose suffix is perturbed by $T_j = (\varphi_j,f_j)$ (the first line of \Eqref{eq:contransition1}), and strings whose  suffixes are not perturbed by any transformations (the second line of \Eqref{eq:contransition1}). 

Indeed, we can decompose \Eqref{eq: simplestate} to
\begin{small}
\begin{align}
     H_{i}^S = \bigcup_{\substack{1\leq j \leq |S|\\ \varphi_j(\substring{\bfx}{a}{b})=1}} 
     \left\{\!
     \begin{aligned}
        \lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S}) \wedge \\ 
        \substring{\bfz}{i-t_j+1}{i} \in f_j(\substring{\bfx}{a}{b})
     \end{aligned}
     \right\} \cup \nonumber\\
     \left\{\!
     \begin{aligned}
        \lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S}) \wedge \\ 
        \forall 1\le j \le n.\ \substring{\bfz}{i-t_j+1}{i} \notin f_j(\substring{\bfx}{a}{b}) \vee \varphi_j(\substring{\bfx}{a}{b}) = 0
     \end{aligned}
     \right\} \label{eq: lemma4.2_1}
\end{align}
\end{small}

To prove \Lemmaref{lemma:4.2}, we will compare the first line of \Eqref{eq:contransition1} with the first line of \Eqref{eq: lemma4.2_1} and the second line of \Eqref{eq:contransition1} with the second line of \Eqref{eq: lemma4.2_1}.

% \aws{the superscript should be $S_{-j}$}

\textit{The first line. }
Because of the inductive hypothesis on $H_{i-t_j} ^{S_{-j}}$ (we have $i-t_j \le i$ and $S_{-j} \subset S$), the first line of \Eqref{eq:contransition1} is equivalent to 
\begin{align}
    \bigcup_{\substack{1\leq j \leq |S|\\ \varphi_j(\substring{\bfx}{a}{b})=1}} \left\{\!
    \begin{aligned}
       \lstm(\bfz, h_0) \mid  &
    \substring{\bfz}{i-t_j+1}{i} \in f_j(\substring{\bfx}{a}{b}) \wedge\\
    &\substring{\bfz}{1}{i-t_j} \in S_{-j}^{=}(\bfx_{1:a})
    \end{aligned}
    \right\}
    \label{eq: lemma4.2_2}
\end{align}

Let 
\begin{align*}
    A &\triangleq \substring{\bfz}{i-t_j+1}{i} \in f_j(\substring{\bfx}{a}{b})  \\
    B &\triangleq \substring{\bfz}{1}{i-t_j} \in S_{-j}^{=}(\bfx_{1:a}) \\
    C &\triangleq \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S})
\end{align*}
Next, we show $A \wedge B$ is equivalent to $A \wedge C$, which proves that the first line of \Eqref{eq:contransition1} is equivalent to the first line of \Eqref{eq: lemma4.2_1}.
Note that (1) $A \wedge C \implies B$, because if $\bfz$ is in the tight perturbation space $S^=$ and the suffix of $\bfz$ is perturbed by $T_j$, then the rest of $\bfz$ (excluding the suffix) is in the tight perturbation space $S^=_{-j}$; and (2) $A \wedge B \implies C$, because if the suffix of $\bfz$ is perturbed by $T_j$ and the rest of $\bfz$ (excluding the suffix) is in the tight perturbation space $S^=_{-j}$, then $\bfz$ is in the perturbation space $S^=$.
Putting (1) and (2) together gives us $A \wedge B \Longleftrightarrow A \wedge C$.

\textit{The second line.} 
Because of the inductive hypothesis on $H_{i-1} ^S$ (we have $i-1 < i$ and $S \subseteq S$), the second line of \Eqref{eq:contransition1} is equivalent to 
\begin{align}
    \{\lstm(\bfz, h_0) \mid \substring{\bfz}{1}{i-1} \in S^=(\substring{\bfx}{1}{i -1- \offset_S}) \wedge z_{i} = x_{i-1 - \offset}\} \label{eq: lemma4.2_3}
\end{align}

We can show the condition
\begin{align*}
& \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S}) \wedge  \\
        &~~~~ \forall 1\le j \le n.\ \substring{\bfz}{i-t_j+1}{i} \notin f_j(\substring{\bfx}{a}{b}) \vee \varphi_j(\substring{\bfx}{a}{b}) = 0
\end{align*}
implies that 
\[\substring{\bfz}{1}{i-1} \in S^=(\substring{\bfx}{1}{i -1- \offset_S}) \wedge z_{i} = x_{i -1- \offset},\]
because if none of the suffix of $\bfz$ is perturbed by any $T_j$, then the last symbol of $\bfz$ must be the same as $\substring{\bfx}{1}{i - \offset_S}$.
This implication means that the second line of \Eqref{eq: lemma4.2_1} is the subset of \Eqref{eq: lemma4.2_3}.

Unfortunately, \Eqref{eq: lemma4.2_3} may not be the subset of the second line of \Eqref{eq: lemma4.2_1} because there might exist $\bfz$ such that 
\begin{align*}
    &\substring{\bfz}{1}{i-1} \in S^=(\substring{\bfx}{1}{i -1- \offset_S}) \wedge z_{i} = x_{i -1- \offset} \wedge \\
    % &~~~~ \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S + 1}) \wedge  \\
    &~~~~ \exists 1\le j \le n.\ \substring{\bfz}{i-t_j+1}{i} \in f_j(\substring{\bfx}{a}{b}) \wedge \varphi_j(\substring{\bfx}{a}{b}) = 1 
\end{align*}
However, if such $\bfz$ exists, $\lstm(\bfz, \hstate_0)$ will be included in the first line of \Eqref{eq: lemma4.2_1}.
In other words, \Eqref{eq: lemma4.2_3} is the subset of the set defined in \Eqref{eq: lemma4.2_1}.

Combining the comparison of \textit{the first line} and \textit{the second line} completes the proof.
\end{proof}


\textbf{\Theref{theorem: theorem4.1}}
\begin{proof}
We can expand \Eqref{eq: theF} using the decomposition of the perturbation space as
\begin{align}
    \bigcup_{S'\in \tightperturbset{S}} \{\lstm(\bfz, \hstate_0) \mid \bfz \in S'^{=}(\bfx)\}
    \label{eq: theorem4.1_1}
\end{align}

% \aws{"Plug X into Y"}
We can plug into \Eqref{eq: simplestate} and \Eqref{eq: finalstateoftight} into \Eqref{eq:hfinal}, getting
\begin{align}
    &\bigcup_{S'\in \tightperturbset{S}}  \{\lstm(\bfz, \hstate_0)\mid \bfz \in S'^{=}(\substring{\bfx}{1}{\len{\bfx} + \offset_S - \offset_S})\}\nonumber\\
&\bigcup_{S'\in \tightperturbset{S}} \{\lstm(\bfz, \hstate_0) \mid \bfz \in S'^{=}(\bfx)\}
    \label{eq: theorem4.1_2}
\end{align}
Because \Eqref{eq: theorem4.1_1} and \Eqref{eq: theorem4.1_2} are equivalent, we can show the equivalence of \Eqref{eq: theF} and \Eqref{eq:hfinal}.
\end{proof}

\textbf{\Theref{theorem: theorem4.2}}
\begin{proof}
The proof of soundness follows immediately from 
the fact that $\alpha$, $\sqcup$, and $\ibp{\lstm}$
overapproximate their inputs,
resulting in an overapproximation $F$.

% \aws{what does the "number of intervals" mean?
% $H_i^S$ is a single hyperrect as defined in the abstract equations}\yh{using hyperrectangle now}

The proof of complexity follows that the number of hyperrectangles $\ibp{H}_i^S$ is $O(\len{\bfx} \prod_{i=1}^n \delta_i)$. For each $\ibp{H}_i^S$, we need to enumerate through all transformations, so the complexity is $O(\len{\bfx}n\prod_{i=1}^n \delta_i)$ in terms of the number of LSTM cell evaluations. The interval bound propagation needs only two forward passes for computing the lower bound and upper bound of the hyperrectangles, so it only contributes constant time in complexity. 
In all, the total number of LSTM cell evaluation needed is $O(\len{\bfx}n\prod_{i=1}^n \delta_i)$.
\end{proof}


==> LSTM%20robust%20training%20(EMNLP)/sections/overview.tex <==
\section{Overview}
\label{sec: overview}
% In this section, we compare our approach with a previous work \citep{DBLP:conf/emnlp/JiaRGL19} for LSTM interval bound propagation (IBP) against a particular perturbation space, word substitutions.
\subsection{Our approach}
In this section, we illustrate our approach using a concrete example and a particular perturbation space, word substitutions. Word substitutions allow an adversary to substitute words in the target sentence with synonyms within a specific budget $\delta$, i.e., at most $\delta$ words can be substituted. \yh{why it is reasonable to consider a budget?} Let us consider a target sentence:
\begin{center}
\emph{I love this movie}
\end{center}
and the following possible word substitutions: $\emph{I} \rightarrow \emph{We}$, $\emph{love} \rightarrow \emph{like}$, $\emph{this} \rightarrow \emph{that}$, and $\emph{movie} \rightarrow \emph{film}$.
If we allow at most $\delta=1$ word substitutions in the target sentence, we have $5 = {4\choose 0} + {4\choose 1}$ possible perturbed sentences. However, the perturbed sentence \emph{We like that movie} is infeasible in this perturbation space because the sentence contains 3 word substitutions.

\loris{at this point I think you need a paragraph that summarizes the approach.
We do 1) this, 2) that, 3) this. In the following we describe each step (maybe use paragraph headers).}

We build our approach on top of interval bound propagation (IBP), an efficient method for training verifiable neural networks. \yh{We can that say our approach can generalize to any abstract domain, as long as the join operation is defined.} IBP abstracts a set of inputs as intervals (lower bounds and upper bounds) and propagates the intervals through the neural network to compute the over-approximation of worst-cast loss. The neural network is further trained on the over-approximated loss.
To use IBP, we convert the word embeddings $\embed{w}$ of each word and synonym \loris{first time using synonym}  $w$ to intervals. 
In the previous example, the embedding of the sentence 
\[[\embed(\emph{I}), \embed(\emph{love}), \embed(\emph{this}), \embed(\emph{movie})] \in \mathbb{R}^{4 \times \dinput}\]
is converted to the interval $l^\emph{input} \in \mathbb{R}^{4 \times \dinput}, u^\emph{input} \in \mathbb{R}^{4 \times \dinput}$, where
\loris{inconsistent notation in superscript, some have parens. Also can you give some intutition before you throw this formula}
\begin{align*}
\begin{array}{lll}
    l^{(\emph{input})}_{1,j} = \min(\embed(\emph{I})_j, \embed(\emph{We})_j), &u^{(\emph{input})}_{1,j} = \max(\embed(\emph{I})_j, \embed(\emph{We})_j),&\\
    l^{(\emph{input})}_{2,j} = \min(\embed(\emph{love})_j, \embed(\emph{like})_j), &u^{(\emph{input})}_{2,j} = \max(\embed(\emph{love})_j, \embed(\emph{like})_j),&\\
    l^{(\emph{input})}_{3,j} = \min(\embed(\emph{this})_j, \embed(\emph{that})_j), &u^{(\emph{input})}_{3,j} = \max(\embed(\emph{this})_j, \embed(\emph{that})_j),&\\
    l^{(\emph{input})}_{4,j} = \min(\embed(\emph{movie})_j, \embed(\emph{film})_j), &u^{(\emph{input})}_{4,j} = \max(\embed(\emph{movie})_j, \embed(\emph{film})_j), & \forall j \in\{1,2,\ldots, \dinput\},
\end{array}
\end{align*}
where $\embed(\bfx)\in \mathbb{R}^\dinput$ is the word embedding for word $\bfx$.
\loris{this def should come earlier. I added it before, but you might want to add  the type}

%Figure~\ref{fig:overview0} shows the LSTM IBP by \citet{DBLP:conf/emnlp/JiaRGL19} where the interval bounds of hidden state $\hstate_4$ and cell state $c_4$ contain $32 = 2^4$ possible perturbed sentences because it allows all possible word substitutions.
%As we will show in experiments, allowing all possible word substitutions leads to severe over-approximation, reducing both normal test accuracy and robustness. 

An RNN cell is a function that takes as input a word embedding $\embed(\bfx_i)$ and the previous hidden state $\hstate_{i-1}$, and outputs the hidden state $\hstate_i$ at the current time step
\begin{align}
    \hstate_i = \emph{RNN}(\embed(x_i), \hstate_{i-1}) \quad \hstate_i, \hstate_{i-1}\in \mathbb{R}^\dhidden. \label{eq:pointform}
\end{align}
In IBP, an RNN cell $\emph{RNN}^\sharp$ can take as input intervals and output intervals as well
\begin{align}
    \interval{\hstate_i}{} = \emph{RNN}^\sharp((\interval{\emph{input}}{i}),(\interval{\hstate_{i-1}}{}))  \label{eq:intervalform}
\end{align}
where $\interval{input}{i}$ are the intervals for the $i$th input token and $(\interval{\hstate_i}{}), (\interval{\hstate_{i-1}}{})$ are the intervals for $\hstate_i$ and $\hstate_{i-1}$, respectively. 
\Eqref{eq:pointform} is subsumed by the interval form \Eqref{eq:intervalform} because a concrete value $x\in R$ can be written as an interval with lower bound $x$ and upper bound $x$.
%We will use the interval form like \eqref{eq:intervalform} in the rest of our paper. \yh{check.} 
To simplify notations, we write an interval $\interval{x}{}$ as $\simitvl{x}{}$.

\loris{some version of this should come early in the section, see comment about summary}
The key idea of our approach is to instrument \loris{first time you talk about instrumentation, what does it mean?} each hidden state not only with the time step but also with a rewritten history. In the word substitution case, the rewritten history counts how many word substitutions have been applied \loris{substituted?} to previous time steps.
By considering the rewritten history, we can control the budget $\delta$ and eliminate \loris{succinctly represent the space?} infeasible perturbed sentences. 

\loris{I'm having a hard time following this. You are introducing new variables and all of them should be defined. The index $\hstate_{i,j}$. I think this section should be rewritten. We can have a short meeting to discuss how.}
We use $\hstate_{i,j}$ to denote the hidden state at time step $i$ with at most $j$ substitutions applied to the prefix ending at $i$, while $\hstate_{i}$ is the hidden state at time step $i$ without rewritten history.\footnote{$\hstate_i$ can be seen as the concatenation of the hidden state and cell state at time step $i$ in LSTM.}
We use dynamic programming 
\loris{dynamic programming is a technique not the main point here. You should just give the defs first, and then
end with. These quantities can be computed in linear time using dynamic programming}
to compute $\hstate_{i,j}$, which can be transitioned from state $\hstate_{i-1,j}$ with the $i$th input token untouched, and state $\hstate_{i-1,j-1}$ with the $i$th input token substituted to its synonyms. 
\begin{align*}
    \simitvl{\hstate_{i,j}}{} = &\emph{RNN}^\sharp(\embed(x_i),\simitvl{\hstate_{i-1,j}}{})  \\
     \sqcup & \emph{RNN}^\sharp(\simitvl{\emph{input}}{i},\simitvl{\hstate_{i-1,j-1}}{}),
\end{align*}
where $\sqcup$ denotes the join of two intervals $\interval{a}{}$ and $\interval{b}{}$, defined as 
\begin{align*}
    \interval{a}{} \sqcup \interval{b}{} = \interval{c}{},
\end{align*}
where $l^{(c)}_j = \min(l^{(a)}_j, l^{(b)}_j), u^{(c)}_j = \max(u^{(a)}_j, u^{(b)}_j), \forall j\in \{1,2,\dots, d\}$. The join operation helps us merge two intervals into one interval that contains all possible concrete values of the previous two intervals.

% \begin{figure*}[!t]
%     \centering
%     \subfigure[LSTM IBP by our approach]{\includegraphics[width=\textwidth]{imgs/overview1.png}\label{fig:overview1}}
%     \subfigure[LSTM IBP by \citet{DBLP:conf/emnlp/JiaRGL19}]{\includegraphics[width=0.95\textwidth]{imgs/overview0.png}\label{fig:overview2}}
%     \caption{LSTM IBP Comparison.}
%     \label{fig: overview}
% \end{figure*}

The computation overview of our approach is shown in \Figref{fig:overview1}, which is divided into two parts.
The top part contains the perturbed sentences with no substitution, i.e., the original target sentence, while the bottom part contains the perturbed sentences with at most one substitution. \yh{need to fix the figure}

\subsection{A Previous Work}
In this section, we compare our approach with a previous work \citep{DBLP:conf/emnlp/JiaRGL19}, which also uses IBP to train robust RNNs against word substitutions.
We show two key differences between our approach and \citet{DBLP:conf/emnlp/JiaRGL19}.
First, \citet{DBLP:conf/emnlp/JiaRGL19} assumes that every word substitution can happen in the target sentence.
In other words, \citet{DBLP:conf/emnlp/JiaRGL19} does not consider the budget $\delta$ for word substitutions.
We show how \citet{DBLP:conf/emnlp/JiaRGL19} computes the hidden states in \Eqref{eq:intervalform} and in \Figref{fig:overview2}.
Second, our approach can generalize to any programmable perturbation space while the previous work cannot, as we will show in the next section.

==> LSTM%20robust%20training%20(EMNLP)/sections/problemdef.tex <==
\section{Robustness Problem and Preliminaries}
% In this section,
% we formalize the robustness-certification problem
% and provide necessary background.

% \subsection{The Robustness Problem}
We consider a classification setting with a neural network $F_\theta$ with parameters $\theta$, trained on samples from domain $\gX$ and labels from $\gY$.
%
The 
 domain $\gX$ is a set of  strings over a finite set of \emph{symbols} $\alphabet$ (e.g., English words or characters), i.e., $\gX = \alphabet^*$.
We use $\bfx \in \alphabet^*$ to denote a string; $x_i \in \alphabet$ to denote the $i$th element of the string; $\substring{\bfx}{i}{j}$ to denote the substring $x_i, \ldots, x_{j}$; $\epsilon$ to denote the empty string; and $\len{\bfx}$ to denote the length of the string.


% \loris{I find it awkward that we use $x_i$ instead of $\bfx_i$}
% \aws{that's what we did last time,
% so we can subscript vectors}
%We will also use $\substring{\bfx}{}{j}$ to denote the prefix ending at $x_{j-1}$ and $\substring{\bfx}{i}{}$ to denote the suffix starting at $x_i$.


\paragraph{Robustness to string transformations} A \emph{perturbation space} $S$ is a function in $\alphabet^* \to 2^{\alphabet^*}$, i.e., $S$ takes a string $\bfx$ and returns a set of possible perturbed strings obtained by modifying $\bfx$.
Intuitively, $S(\bfx)$ denotes a set of strings
that are semantically \emph{similar} to $\bfx$ and therefore
should receive the same prediction.
We assume $\bfx \in S(\bfx)$.

Given string $\bfx$ with label $y$
and a perturbation space $S$,
We say that a neural network $F_\theta$ is \textit{$S$-robust} on $(\bfx,y)$ iff
\begin{align}
    \forall \bfz \in S(\bfx) \ldotp F_\theta(\bfz) = y \label{eq:robustness}
\end{align}



Our primary goal in this paper is  to \emph{certify}, or prove, $S$-robustness (\Eqref{eq:robustness}) of the neural network for a pair $(\bfx,y)$.
Given a certification approach, we can then use it within an adversarial training loop to yield certifiably robust networks.


\paragraph{Robustness certification}
We will  certify $S$-robustness by solving
an \emph{adversarial loss} objective: 
\begin{align} 
\max_{\bfz \in S(\bfx)} L_\theta(\bfz,y)\label{eq:advloss}
\end{align} 
where we assume that the loss function $L_\theta$ is $< 0$ when $F_\theta(\bfz) = y$
and $\geq 0$ when $F_\theta(\bfz) \neq y$.
Therefore, if we can show that the solution to the above problem is $< 0$, then we have a certificate of $S$-robustness.



% The key challenge is solving the above optimization objective.
% In order to construct an $S$-robustness certificate,
% we need to compute an upper bound on the adversarial loss.

\paragraph{Certified training}
If we have a procedure to compute adversarial loss,
we can use it for \emph{adversarial training} by solving the following
\emph{robust optimization} objective~\cite{madry2017towards},
where $\mathcal{D}$ is the data distribution:
\begin{align} 
\argmin_\theta \mathop{\mathbb{E}}_{(\bfx,y) \sim \mathcal{D}} \left[\max_{\bfz \in S(\bfx)} L_\theta(\bfz,y)\right]\label{eq:advlosstrain}
\end{align} 

% \aws{I removed the challenges part}
% \paragraph{Certification challenges}
% To solve adversarial loss optimally,
% we can enumerate all strings $\bfz$ in the set $S(\bfx)$ and compute the network prediction of $\bfz$. 
% In general, it is infeasible to consider the entire perturbation space, as it can be exponentially large in the size of the input.
% Further, even if the space is practically enumerable, e.g., millions of strings, performing enumeration during training makes training impractically slow. 

% Recent works have been proposed to certify the robustness of neural networks by abstract interpretation~\yh{cite}. These works either target at the continuous $L_p$ norm region in the word embedding space or target at a specific transformation, word substitutions. 
% However, we are interested in a discrete perturbation space where there are general string transformations specified by users.

\subsection{Programmable Perturbation Spaces}
\label{sec:pps}
In our problem definition, we assumed an arbitrary perturbation 
space $S$.
%
We adopt the recently 
proposed specification language~\citep{ZhangAD20}
to define $S$ \emph{programmatically}
as a set of string transformations.
The language is very flexible, allowing 
the definition of a rich class of transformations
as \emph{match} and \emph{replace} functions.

\paragraph{Single transformations}
% \loris{I added the parameters $s$ and $t$ to $T$. It's ugly but maybe more precise.}
A string transformation $T$ is a pair $(\varphi, f)$, where 
$\varphi: \alphabet^s \to \{0,1\}$ is the \emph{match} function, a Boolean function that specifies the substrings (of length $s$)  to which the transformation can be applied; and
$f: \alphabet^s \to 2^{\alphabet^t}$ is the \emph{replace} function, which specifies
how the substrings matched by $\varphi$ can be replaced (with strings of length $t$).
We will call $s$ and $t$ the size of the \emph{domain}
and \emph{range} of transformation $T$, respectively.

\begin{example}
\label{exp:transformation}
In all examples, the set of symbols $\Sigma$ is English words.
So, strings are English sentences.
%
Let $T_\emph{del}$ be a string transformation that deletes the stop words ``\emph{to}'' and ``\emph{the}''. 
%
Formally, $T_\emph{del}=(\varphi_\emph{del},f_\emph{del})$, where $\varphi_\emph{del}: \alphabet^1 \mapsto \{0,1\}$ and $f_\emph{del}: \alphabet^1 \to 2^{\alphabet^0}$ are:
\vskip -0.1in
\begin{small}
\begin{align*}
    \varphi_\emph{del}(x) = \begin{cases}
    1,& x\in \{\text{``to'', ``the''}\} \\
    0,& \text{otherwise}
\end{cases}, \quad f_\emph{del}(x) = \{\epsilon\},
\end{align*}
\end{small}%

Let $T_\emph{sub}$ be a  transformation substituting the word ``\emph{movie}'' with ``\emph{movies}'' or ``\emph{film}''. Formally,
$T_\emph{sub}=(\varphi_\emph{sub},f_\emph{sub})$, where $\varphi_\emph{sub}: \alphabet^1 \mapsto \{0,1\}$ and $f_\emph{sub}: \alphabet^1 \to 2^{\alphabet^1}$ are:
\vskip -0.1in
\begin{small}
\begin{align*}
    \varphi_\emph{sub}(x) = \begin{cases}
    1,& x = \emph{``movie''}\\
    0,& \text{otherwise}
\end{cases}, f_\emph{sub}(x) = \left\{\!\begin{aligned}
&~~\emph{``film''},\\
&\emph{``movies''}
\end{aligned}\right\}
\end{align*}
\end{small}%
\end{example}
% \aws{eq outside line}

\paragraph{Defining perturbation spaces}
We can compose different string transformation to construct perturbation space $S$:
\begin{align}
    \spec=\{(T_1, \delta_1), \dots ,(T_n, \delta_n)\}, \label{eq:progspec}
\end{align}
where each $T_i$ denotes a string transformation that can be applied \emph{up to} $\delta_i \in \mathbb{N}$ times. 
% \yh{added this sentence, please check}
Note that the transformations can be applied whenever they match a \emph{non-overlapping} set of substrings and are then transformed in parallel.
We illustrate with an example
and refer to \citet{ZhangAD20} for formal semantics.

\begin{example}
\label{exp: perturbspace}
Let $\spec =\{(T_\emph{del},1),(T_\emph{sub},1)\}$ be a perturbation space that applies $T_\emph{del}$ and $T_\emph{sub}$ to the given input sequence up to once each.
%
If $\bfx=$``\emph{to the movie}'', a subset of the perturbation space $\spec(\bfx)$ is shown in \cref{fig:approachfig}(a). 
% \yh{In intro, we only allow to delete ``the'', need we unify this later?}
\end{example}

\paragraph{Decomposition}
$S=\{(T_i, \delta_i)\}_i$ can be decomposed into $\prod (\delta_i + 1)$ subset perturbation spaces by considering all smaller combinations of $\delta_i$.
We denote the decomposition of perturbation space $S$ as $\tightperturbset{S}$, and exemplify below:

\begin{example}
\label{ex:decs}
$S_1=\{(T_\emph{del},2)\}$ can be decomposed to a set of three perturbation spaces $\tightperturbset{S_1} = 
\{\varnothing,  \{(T_\emph{del},1)\}, \{(T_\emph{del},2)\}\}$,
while 
 $S_2=\{(T_\emph{del},1),(T_\emph{sub},1)\}$ can be decomposed to a set of four perturbation spaces
 \vskip -0.1in
 \begin{small}
 \[
     \tightperturbset{S_2}=\{\varnothing, \{(T_\emph{del},1)\}, \{(T_\emph{sub},1)\}, \{(T_\emph{del},1),(T_\emph{sub},1)\}\}\]
 \end{small}%
where $\varnothing$ is the perturbation space  with no transformations, i.e.,
if $S = \varnothing$, then $S(\bfx) = \{\bfx\}$
for any string $\bfx$.
\end{example}

% \yh{move to here}
We use notation $S_{k\downarrow{}}$ to denote $S$
after reducing $\delta_k$ by 1;
therefore, $S_{k\downarrow{}} \in \tightperturbset{S}$.

% \begin{example}
% The definition of $\sqcup$ is consistent when $a,b$ are two tensors of intervals. Suppose $\lb{a}=(0,0)^\top, \ub{a}=(0,1)^\top, \lb{b}=(-1,2)^\top, \ub{b}=(0,3)^\top$, the lower bound and upper bound of $a \sqcup b$ are $(-1, 0)^\top$ and $(0,3)^\top$.
% \end{example}


\subsection{The LSTM Cell}
We  focus our exposition on LSTMs.
%
% An LSTM takes as input a string $\bfx$ and returns a prediction;
% this is done by recursively applying an LSTM \emph{cell} to each symbol $x_i$ of $\bfx$.
%
% We assume that our alphabet is that of \emph{words} (i.e., word-level modeling, see Example~\ref{exp:transformation}).
% and that each word is given a real-valued vector
% generated, for example, using word embeddings.
% Thus, we use the $i$th word of string $x_i$ as a vector.
% \aws{maybe early on in prob def we just say our alphabet is a dictionary $\Sigma$}
%
An LSTM cell is a function, denoted $\lstm$, that takes as input a symbol $x_i$ and the previous \emph{hidden state} and \emph{cell state}, and outputs the hidden state and the cell state at the current time step.
For simplicity, we use $\hstate_i$ to denote the concatenation of the hidden and cell states at the $i$th time step,
and simply refer to it as the \emph{state}.
Given string $\bfx$, we define $\hstate_i$ as follows:
\begin{align*}
    \hstate_i &= \lstm(x_i, \hstate_{i-1}) \quad \hstate_i, \hstate_{i-1}\in \mathbb{R}^{d}, %\label{eq:pointformlstm2}
\end{align*}
where     $\hstate_0 = 0^{d}$
and $d$ is the dimensionality of the state.
For a string $\bfx$ of length $n$,
we say that $h_n$ is the \emph{final state}.

% It will be useful for us to apply LSTMs to substrings
% of a string $\bfx$.
For a string $\bfx$ and state $h$,
We use $\lstm(\bfx,h)$ to denote 
\[\lstm(x_{\len{\bfx}}, \lstm(\ldots, \lstm(x_1 ,\hstate)\ldots))\]
E.g., $\lstm(\bfx, \hstate_0)$ is the final state of the LSTM applied to  $\bfx$.


==> LSTM%20robust%20training%20(EMNLP)/sections/relatedwork.tex <==
\section{Related Work}
\input{tables/approaches}

\cref{tab:approaches}
compares \toolname{} to most related approaches.

% \paragraph{Adversarial attacks in NLP} \citet{SurveyZhangSAL20} and \citet{SurveyHugTP20} conduct surveys of adversarial attacks in NLP.
% %
% There are different kinds of test-time attacks: word/character-level attacks~\cite{DBLP:conf/coling/EbrahimiLD18, DBLP:conf/milcom/PapernotMSH16, DBLP:conf/emnlp/GargR20}, 
% paraphrasing attacks~\cite{DBLP:conf/naacl/IyyerWGZ18},
% and sentence-level attacks~\cite{DBLP:conf/naacl/WangB18}.
% Some works combine different attacks~\cite{DBLP:conf/conll/BlohmJSYV18}.
% Other test-time attacks \cite{DBLP:conf/emnlp/WallaceFKGS19} look for \emph{backdoors} (universal triggers) in NLP models.

% \toolname{} is very flexible, allowing specification of attack models as sets of string transformations using \emph{match} and \emph{replace} functions
% over symbols in the strings.
% We additionally demonstrate how to extend our approach to tree transformations for TreeLSTMs~\cite{DBLP:conf/acl/TaiSM15}.

% \aws{characters and words are the same from a mathematical perspective, so not interesting to separate them. Also our approach can go beyond words, e.g., matching phrases}


\paragraph{Certification of robustness in NLP}
See \citet{SurveyLiQXL20} for a survey of robust training.
Some works focus on certifying the $l_p$ norm ball of each word embedding for LSTMs~\cite{DBLP:conf/icml/KoLWDWL19, DBLP:conf/atva/JacobyBK20} and transformers~\cite{DBLP:conf/iclr/ShiZCHH20}. 
Others focus on certifying word substitutions for CNNs~\cite{DBLP:conf/emnlp/HuangSWDYGDK19} and LSTMs~\cite{DBLP:conf/emnlp/JiaRGL19, DBLP:conf/nips/XuS0WCHKLH20}, and word deletions for the decomposable attention model~\cite{DBLP:conf/iclr/WelblHSGDSK20}. 
Existing techniques rely on abstract interpretation, such as IBP~\cite{DBLP:conf/iccv/GowalDSBQUAMK19} and CROWN~\cite{DBLP:conf/nips/ZhangWCHD18}.
We focus on certifying the robustness of LSTM models (including TreeLSTMs) to a programmable perturbation space, which is out-of-scope for existing techniques.
Note that \citet{DBLP:conf/nips/XuS0WCHKLH20} also uses memoization and abstraction to certify, but \toolname{} subsumes \citet{DBLP:conf/nips/XuS0WCHKLH20} because \toolname{} can certify arbitrary string transformations. %\yh{add comparison Xu et al. here.}
We use IBP, but our approach can use other abstract domains, such as zonotopes~\cite{ai2}.

% Randomized smoothing~\cite{RSDBLP:conf/icml/CohenRK19, RSDBLP:conf/nips/SalmanLRZZBY19} gives a probabilistic certificate of robustness.
SAFER~\cite{DBLP:conf/acl/YeGL20} is a model-agnostic approach 
that uses \emph{randomized smoothing}~\cite{RSDBLP:conf/icml/CohenRK19} to give probabilistic certificates of robustness to word substitution.
Our approach gives a non-probabilistic certificate and can handle arbitrary perturbation spaces beyond substitution.

\paragraph{Robustness techniques in NLP}
Adversarial training is an empirical defense method that can improve the robustness of models by solving a \emph{robust-optimization} problem~\cite{madry2017towards},
which minimizes worst-case (adversarial) loss.
%
Some techniques in NLP
use adversarial attacks to compute a lower bound on the worst-case loss~\cite{ebrahimi2018hotflip, DBLP:conf/naacl/MichelLNP19}.
ASCC~\cite{dong2021towards} overapproximates the word substitution attack space by a convex hull where a lower bound on the worst-case loss is computed using gradients.
Other techniques 
compute upper bounds on adversarial loss using abstract interpretation~\cite{DBLP:conf/iccv/GowalDSBQUAMK19, DBLP:conf/icml/MirmanGV18}. 
\citet{DBLP:conf/emnlp/HuangSWDYGDK19}
and \citet{DBLP:conf/emnlp/JiaRGL19, DBLP:conf/nips/XuS0WCHKLH20} used abstract interpretation to train CNN and LSTM models against word substitutions.
A3T~\cite{ZhangAD20} trains robust CNN models against a programmable perturbation space by combining 
adversarial training and abstraction.
Our approach uses abstract interpretation to train robust LSTMs against programmable perturbation spaces
as defined in \citet{ZhangAD20}.

% Preprocessing-based techniques improve robustness by using spelling-mistake detectors~\cite{DBLP:conf/acl/PruthiDL19, DBLP:conf/aaai/SakaguchiDPD17}.


==> LSTM%20robust%20training%20(EMNLP)/sections/tails.tex <==
\section{Conclusion}
We present \toolname{}, which uses memoization and abstract interpretation
to certify robustness to programmable perturbations for LSTMs. 
\toolname{} can be used to  train models that are more robust 
than those trained  using existing techniques and handle more complex perturbation spaces.
Last, the models trained with \toolname{} have high certification accuracy,
which can be certified using \toolname{} itself.
% and (3) \toolname{} can certify robustness to combinations of string transformations that are out-of-scope for existing techniques.


==> LSTM%20robust%20training%20(EMNLP)/tables/a3t-arc.tex <==
\begin{table}[t]
    \centering
    \caption{Results of different instantiations of \toolname{}-A3T on SST2 dataset. }
    \setlength{\tabcolsep}{3pt}

    \begin{small}
    \begin{tabular}{l *2{ccc}}
        \toprule
         & \multicolumn{3}{c}{\scriptsize $\{(\Tdelword{}, 2),(\Tsubword{},2)\}$} & \multicolumn{3}{c}{\scriptsize $\{(\Tinsword{}, 2),(\Tsubword{},2)\}$} \\ 
         
         \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
        Train & {\small Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\small Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}}  \\
        \midrule
        Abs-fir & \textbf{83.2}  & 15.1 & 68.6 & 82.6 & 15.9 & \textbf{66.7} \\
        Abs-sec & 81.4  & 71.1 & 75.8 & \textbf{83.0} & 48.8 & 65.4 \\
        \toolname{} & 82.5 & \textbf{72.5} & \textbf{77.0} & 80.2 & \textbf{55.4} & 64.0\\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:arc_a3t}

\end{table}

==> LSTM%20robust%20training%20(EMNLP)/tables/approaches.tex <==
\begin{table}[t]
    \centering
    \caption{ \toolname{} compared to other approaches. \citet{DBLP:conf/acl/YeGL20} provide probabilistic certificates. 
    }
    % \setlength{\tabcolsep}{1pt}
 \renewcommand{\arraystretch}{1}
    \begin{small}
    \begin{tabular}{lccl}
        \toprule
         Approach & LSTM & Cert & Transf.   \\ 
        \midrule
        \small{\citet{ebrahimi2018hotflip}} & \cmark & \xmark & \emph{arbitrary}\\
        \small{\citet{POPQORN}} & \cmark & \cmark & $l_p$ norm\\
        \small{\citet{DBLP:conf/emnlp/HuangSWDYGDK19}} & \xmark & \cmark & substitution \\
        \small{\citet{DBLP:conf/emnlp/JiaRGL19}} & \cmark & \cmark & substitution \\
        \small{\citet{ZhangAD20}} & \xmark & \xmark & \emph{arbitrary}  \\
        \small{\citet{DBLP:conf/acl/YeGL20}} & \cmark & $\mathbb{P}$ & substitution \\
        \small{\citet{DBLP:conf/nips/XuS0WCHKLH20}} & \cmark & \cmark & substitution \\
        \citet{dong2021towards} & \cmark & \xmark & substitution \\
        \small{\toolname{} (\emph{this paper})} & \cmark & \cmark & \emph{arbitrary} \\
        \bottomrule
    \end{tabular}
    \end{small}

    \label{tab:approaches}
\end{table}


==> LSTM%20robust%20training%20(EMNLP)/tables/compare_huang.tex <==
\begin{table}[t]
    \centering
    \caption{\toolname{} vs \citet{DBLP:conf/emnlp/HuangSWDYGDK19} (CNN) on SST2 dataset. }
    % \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{5pt}

    \begin{small}
    \begin{tabular}{ll *1{cccc}}
        \toprule
         && \multicolumn{4}{c}{$\{(\Tsubword{},3)\}$}\\ 
         
         \cmidrule(lr){3-6}
        Train & Model & {\small Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}}  \\
        \midrule
        Huang et al. & CNN & 81.7 & 77.2 & 44.5 & 76.5 \\
        \toolname{} & LSTM & \textbf{83.3} & \textbf{78.3} & \textbf{73.3} & \textbf{77.9}\\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:compare_huang}

\end{table}

==> LSTM%20robust%20training%20(EMNLP)/tables/comparea3t.tex <==
\begin{table}[t]
    \centering
    \caption{\toolname{} vs A3T (CNN) on SST2 dataset. }
    \renewcommand{\arraystretch}{0.8}
    % \setlength{\tabcolsep}{1pt}

    \begin{small}
    \begin{tabular}{ll *1{p{\lengthcellshorter{}}p{\lengthcell{}}p{\lengthcell{}}p{\lengthcelllonger{}}}}
        \toprule
         && \multicolumn{4}{>{\centering\arraybackslash}p{\lengththreecell{}}}{$\SDS$}\\ 
         
         \cmidrule(lr){3-6}
        Train & Model & {\small Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}}  \\
        \midrule
        A3T & CNN & 80.2 & 71.9 & N/A & 70.2 \\
        \textbf{\toolname{}} & LSTM & \textbf{82.5} & \textbf{77.8} & \textbf{72.5} & \textbf{77.0}\\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:compare_a3t}

\end{table}

==> LSTM%20robust%20training%20(EMNLP)/tables/comparea3t_whole.tex <==
% \begin{table}[t]
%     \centering
%     \caption{\toolname{} vs A3T (CNN) on SST2 dataset. }
%     % \setlength{\tabcolsep}{1pt}
%     \vskip 0.1in
%     \small
%     \begin{tabular}{ll *1{p{\lengthcellshorter{}}p{\lengthcell{}}p{\lengthcell{}}p{\lengthcelllonger{}}}}
%         \toprule
%          && \multicolumn{4}{>{\centering\arraybackslash}p{\lengththreecell{}}}{$\{(\Tinsword{}, 2),(\Tsubword{},2)\}$} \\ 
         
%          \cmidrule(lr){3-6} 
%         Training & Model & {\small Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} \\
%         \midrule
%         A3T & CNN & 79.9 & 68.3 & N/A & 57.7 \\
%         \toolname{} & LSTM & \textbf{80.2} & \textbf{70.0} & \textbf{55.4} & \textbf{64.0}\\
%         \bottomrule
%     \end{tabular}
%     \label{tab:compare_a3twhole}
% \end{table}
\begin{table*}[t]
    \centering
    \caption{\toolname{} vs A3T (CNN) on SST2 dataset. }
    % \setlength{\tabcolsep}{1pt}

    \begin{small}
    \begin{tabular}{ll *2{p{\lengthcellshorter{}}p{\lengthcell{}}p{\lengthcell{}}p{\lengthcelllonger{}}}}
        \toprule
         && \multicolumn{4}{>{\centering\arraybackslash}p{\lengththreecell{}}}{$\{(\Tdelword{}, 2),(\Tsubword{},2)\}$} & \multicolumn{4}{>{\centering\arraybackslash}p{\lengththreecell{}}}{$\{(\Tinsword{}, 2),(\Tsubword{},2)\}$} \\ 
         
         \cmidrule(lr){3-6} \cmidrule(lr){7-10} 
        Train & Model & {\small Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\small Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}}  \\
        \midrule
        A3T (HotFlip) & CNN & 80.2 & 71.9 & N/A & 70.2 & 79.9 & 68.3 & N/A & 57.7 \\
        \toolname{} & LSTM & \textbf{82.5} & \textbf{77.8} & \textbf{72.5} & \textbf{77.0} & \textbf{80.2} & \textbf{70.0} & \textbf{55.4} & \textbf{64.0}\\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:compare_a3twhole}

\end{table*}

==> LSTM%20robust%20training%20(EMNLP)/tables/comparejia.tex <==
\begin{table}[t]
    \centering
    \caption{ \toolname{} vs \jiaapproach{} and ASCC on IMDB dataset.}
    \renewcommand{\arraystretch}{0.8}
    \setlength{\tabcolsep}{5pt}

    \begin{small}
    \begin{tabular}{lllllll}
        \toprule
         & \multicolumn{3}{c}{$\{(\Tsubword{},1)\}$} & \multicolumn{3}{c}{$\{(\Tsubword{},2)\}$} \\ 
         
         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
        {\scriptsize Train} & {\scriptsize Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}}  \\
        \midrule
        {\scriptsize \jiaapproach{}} & 76.8 & 67.0 & 71.0 & 76.8 & 64.8 &  68.3\\
        {\scriptsize ACSS} & 82.8 & ~~0.0 & 81.5 & 82.8 & ~~0.0 & \textbf{80.8}\\
        {\scriptsize \textbf{\toolname{}}} & \textbf{87.7} & \textbf{77.8} & \textbf{82.6} & \textbf{86.3} & \textbf{71.0} & 78.2\\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:compare_jia}

\end{table}


==> LSTM%20robust%20training%20(EMNLP)/tables/comparers.tex <==
\begin{table}[t]
    \centering\small
    \caption{SAFER post-processing on IMDB dataset.
    % $^*$Exhaustive accuracy for SAFER
    % is very expensive to compute; we give an \emph{upper bound} on exhaustive accuracy, by restricting the perturbation space
    }
    % It takes more than one week to compute the exhaustive accuracy of the smoothed model. We show an upper bound of exhaustive accuracy by enumerating a subset of the perturbation space of each sample. We are able to compute the exhaustive accuracy of the model trained by \toolname{} owing to the high certified accuracy because we do not have to enumerate an example if it is certified. \yh{please check the above. should we call it data augmentation rather than smoothing?}}
    % \setlength{\tabcolsep}{1pt}

    \begin{small}
    \begin{tabular}{lllll}
        \toprule
         & \multicolumn{2}{c}{$\{(\Tsubword{},1)\}$} & \multicolumn{2}{c}{$\{(\Tsubword{},2)\}$} \\ 
         
         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        Train & \Verifiedshort{} & RS Acc. & \Verifiedshort{} & RS Acc. \\
        \midrule
        % Smoothing & \textbf{89.8} & ~~0.2 & 82.9 & \textbf{90.0} & \textbf{89.9} & ~~0.1 & 79.9$^*$ & \textbf{89.7}\\
        % \toolname{} & 86.8 & \textbf{82.0} & \textbf{84.8} & 87.2 & 86.4 & 
        % \textbf{79.6} & \textbf{83.0} & 86.7\\
        Data Aug. & ~~0.2 & \textbf{90.0} & ~~0.1 & \textbf{89.7}\\
        \toolname{} & \textbf{82.0} & 87.2 & 
        \textbf{79.6} & 86.7\\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:compare_rs}

\end{table}


==> LSTM%20robust%20training%20(EMNLP)/tables/comparers_whole.tex <==
\begin{table}[t]
    \centering
    \caption{\toolname{} vs SAFER  on IMDB dataset.}
    % \setlength{\tabcolsep}{1pt}

    \begin{small}
    \begin{tabular}{lllll}
        \toprule
         & \multicolumn{2}{c}{$\{(\Tsubword{},1)\}$} & \multicolumn{2}{c}{$\{(\Tsubword{},2)\}$} \\ 
         
         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        Train & \Verifiedshort{} & RS Acc. & \Verifiedshort{} & RS Acc. \\
        \midrule
        % Smoothing & \textbf{89.8} & ~~0.2 & 82.9 & \textbf{90.0} & \textbf{89.9} & ~~0.1 & 79.9$^*$ & \textbf{89.7}\\
        % \toolname{} & 86.8 & \textbf{82.0} & \textbf{84.8} & 87.2 & 86.4 & 
        % \textbf{79.6} & \textbf{83.0} & 86.7\\
        Data Aug. & ~~0.2 & \textbf{90.0} & ~~0.1 & \textbf{89.7}\\
        \toolname{} & \textbf{82.0} & 87.2 & 
        \textbf{79.6} & 86.7\\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:compare_rswhole}

\end{table}


==> LSTM%20robust%20training%20(EMNLP)/tables/lstm.tex <==
% \begin{table*}[t!]
%     \centering

%     % \aws{should we also highlight the \Verifiedshort{} Acc column, because that's our contribution? / also bold points for winners in all columns}
%     % \aws{we can potentially combine the three tables into one mega table, as they all have the same structure} \yh{todo: distinguish LSTM, Tree-LSTM, and Bi-LSTM}
%     \caption{Results of LSTM (on SST2 dataset) and Tree-LSTM (on SST) for three perturbation spaces. %We show the clean accuracy (Acc.), HotFlip accuracy (HF Acc.), certified accuracy (\Verifiedshort{}), and exhaustive accuracy (\Exhaustiveshort{}) of four different training methods. 
%     }
%     \setlength{\tabcolsep}{5pt}
%     \renewcommand{\arraystretch}{0.8}
%     \begin{small}
%     \begin{tabular}{cl *3{cccc}}
%         \toprule
%          && \multicolumn{4}{c}{$\{(\Tdelword{}, 2),(\Tsubword{},2)\}$} & \multicolumn{4}{c}{$\{(\Tinsword{}, 2),(\Tsubword{},2)\}$} & \multicolumn{4}{c}{$\{(\Tdelword{}, 2),(\Tinsword{},2)\}$} \\ 
         
%          \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
%         &Train & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} \\
%         \midrule
%         \multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{\tiny{LSTM}}}} & Normal & \textbf{84.6} & 71.9 & \cellcolor{Gray!10}~~4.6 & \cellcolor{Gray!10}68.9 & 84.6 & 64.0 & \cellcolor{Gray!10}~~0.5 & \cellcolor{Gray!10}55.1 & \textbf{84.6} & 73.7 & \cellcolor{Gray!10}~~1.2 & \cellcolor{Gray!10}65.2 \\
        
%         & Data Aug. & 84.0 & 77.0 & \cellcolor{Gray!10}~~5.5 & \cellcolor{Gray!10}74.4 & \textbf{84.7} & 70.2 & \cellcolor{Gray!10}~~0.3 & \cellcolor{Gray!10}61.5 & 84.5 & 75.4 & \cellcolor{Gray!10}~~0.4 & \cellcolor{Gray!10}68.3 \\
        
%         & HotFlip  & 84.0 & \textbf{78.7} & \cellcolor{Gray!10}~~4.3 & \cellcolor{Gray!10}74.6 & 82.5 & \textbf{75.9} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}62.0 & 84.4 & \textbf{80.6} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}68.7 \\ 
        
%         & \toolname{} & 82.5 & 77.8 & \cellcolor{Gray!10}\textbf{72.5} &  \cellcolor{Gray!10}\textbf{77.0} & 80.2 & 70.0 & \cellcolor{Gray!10}\textbf{55.4} & \cellcolor{Gray!10}\textbf{64.0} & 82.6 & 78.6 & \cellcolor{Gray!10}\textbf{69.4} &  \cellcolor{Gray!10}\textbf{74.6} \\ 
        
        
%                 \midrule
%         \multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{\tiny{Tree-LSTM}}}} & Normal & \textbf{50.3} & 39.9 & \cellcolor{Gray!10}~~4.1 & \cellcolor{Gray!10}33.8 & \textbf{50.3} & 33.4 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}17.9 & \textbf{50.3} & 40.1 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}25.7\\
        
%         & Data Aug. & 47.5 & 40.8 & \cellcolor{Gray!10}~~1.4 & \cellcolor{Gray!10}36.4 & 48.1 & 37.1 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}23.0 & 47.6 & 40.6 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}29.0\\
        
%         & HotFlip  & 49.5 & 43.4 & \cellcolor{Gray!10}~~1.6 & \cellcolor{Gray!10}38.4 & 48.7 & \textbf{39.5} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}29.0 & 49.5 & 42.7 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}32.1 \\ 
        
%         & \toolname{} & 46.4 & \textbf{43.4} & \cellcolor{Gray!10}\textbf{30.9} & \cellcolor{Gray!10}\textbf{41.9} & 46.1 & 39.0 & \cellcolor{Gray!10}\textbf{17.1} & \cellcolor{Gray!10}\textbf{37.6} & 46.5 & \textbf{43.8} & \cellcolor{Gray!10}\textbf{19.2} & \cellcolor{Gray!10}\textbf{40.0}\\ 
%         \bottomrule
%     \end{tabular}
%     \end{small}
%     \label{tab:lstm}
% \end{table*}


\begin{table*}[t!]
    \centering

    % \aws{should we also highlight the \Verifiedshort{} Acc column, because that's our contribution? / also bold points for winners in all columns}
    % \aws{we can potentially combine the three tables into one mega table, as they all have the same structure} \yh{todo: distinguish LSTM, Tree-LSTM, and Bi-LSTM}
    \caption{Results of LSTM on SST2 dataset for three perturbation spaces. %We show the clean accuracy (Acc.), HotFlip accuracy (HF Acc.), certified accuracy (\Verifiedshort{}), and exhaustive accuracy (\Exhaustiveshort{}) of four different training methods. 
    }
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{0.8}
    \begin{small}
    \begin{tabular}{l *3{cccc}}
        \toprule
         & \multicolumn{4}{c}{$\SDS$} & \multicolumn{4}{c}{$\SIS$} & \multicolumn{4}{c}{$\SDI$} \\ 
         
         \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
        Train & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} \\
        \midrule
         Normal & \textbf{84.6} & 71.9 & \cellcolor{Gray!10}~~4.6 & \cellcolor{Gray!10}68.9 & 84.6 & 64.0 & \cellcolor{Gray!10}~~0.5 & \cellcolor{Gray!10}55.1 & \textbf{84.6} & 73.7 & \cellcolor{Gray!10}~~1.2 & \cellcolor{Gray!10}65.2 \\
        
         Data Aug. & 84.0 & 77.0 & \cellcolor{Gray!10}~~5.5 & \cellcolor{Gray!10}74.4 & \textbf{84.7} & 70.2 & \cellcolor{Gray!10}~~0.3 & \cellcolor{Gray!10}61.5 & 84.5 & 75.4 & \cellcolor{Gray!10}~~0.4 & \cellcolor{Gray!10}68.3 \\
        
         HotFlip  & 84.0 & \textbf{78.7} & \cellcolor{Gray!10}~~4.3 & \cellcolor{Gray!10}74.6 & 82.5 & \textbf{75.9} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}62.0 & 84.4 & \textbf{80.6} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}68.7 \\ 
        
         \textbf{\toolname{}} & 82.5 & 77.8 & \cellcolor{Gray!10}\textbf{72.5} &  \cellcolor{Gray!10}\textbf{77.0} & 80.2 & 70.0 & \cellcolor{Gray!10}\textbf{55.4} & \cellcolor{Gray!10}\textbf{64.0} & 82.6 & 78.6 & \cellcolor{Gray!10}\textbf{69.4} &  \cellcolor{Gray!10}\textbf{74.6} \\ 
        
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:lstm}
\end{table*}


==> LSTM%20robust%20training%20(EMNLP)/tables/lstm_whole.tex <==
\begin{table*}[t]
    \centering

    % \aws{should we also highlight the \Verifiedshort{} Acc column, because that's our contribution? / also bold points for winners in all columns}
    % \aws{we can potentially combine the three tables into one mega table, as they all have the same structure} \yh{todo: distinguish LSTM, Tree-LSTM, and Bi-LSTM}
    \caption{Results of LSTM (on SST2), Tree-LSTM (on SST), and Bi-LSTM (on SST2) for three perturbation spaces. %We show the clean accuracy (Acc.), HotFlip accuracy (HF Acc.), certified accuracy (\Verifiedshort{}), and exhaustive accuracy (\Exhaustiveshort{}) of four different training methods. 
    }

    \setlength{\tabcolsep}{4.5pt}
    \renewcommand{\arraystretch}{0.8}
    \begin{small}
    \begin{tabular}{cl *3{cccc}}
        \toprule
         && \multicolumn{4}{>{\centering\arraybackslash}p{\lengththreecell{}}}{$\{(\Tdelword{}, 2),(\Tsubword{},2)\}$} & \multicolumn{4}{>{\centering\arraybackslash}p{\lengththreecell{}}}{$\{(\Tinsword{}, 2),(\Tsubword{},2)\}$} & \multicolumn{4}{>{\centering\arraybackslash}p{\lengththreecell{}}}{$\{(\Tdelword{}, 2),(\Tinsword{},2)\}$} \\ 
         
         \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
        &Train & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} \\
        \midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{\tiny{LSTM}}}} & Normal & \textbf{84.6} & 71.9 & \cellcolor{Gray!10}~~4.6 & \cellcolor{Gray!10}68.9 & 84.6 & 64.0 & \cellcolor{Gray!10}~~0.5 & \cellcolor{Gray!10}55.1 & \textbf{84.6} & 73.7 & \cellcolor{Gray!10}~~1.2 & \cellcolor{Gray!10}65.2 \\
        
        & Data Aug. & 84.0 & 77.0 & \cellcolor{Gray!10}~~5.5 & \cellcolor{Gray!10}74.4 & \textbf{84.7} & 70.2 & \cellcolor{Gray!10}~~0.3 & \cellcolor{Gray!10}61.5 & 84.5 & 75.4 & \cellcolor{Gray!10}~~0.4 & \cellcolor{Gray!10}68.3 \\
        
        & HotFlip & 84.0 & \textbf{78.7} & \cellcolor{Gray!10}~~4.3 & \cellcolor{Gray!10}74.6 & 82.5 & \textbf{75.9} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}62.0 & 84.4 & \textbf{80.6} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}68.7 \\ 
        
        & \toolname{} & 82.5 & 77.8 & \cellcolor{Gray!10}\textbf{72.5} &  \cellcolor{Gray!10}\textbf{77.0} & 80.2 & 70.0 & \cellcolor{Gray!10}\textbf{55.4} & \cellcolor{Gray!10}\textbf{64.0} & 82.6 & 78.6 & \cellcolor{Gray!10}\textbf{69.4} &  \cellcolor{Gray!10}\textbf{74.6} \\ 
        
        
                \midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{\tiny{Tree-LSTM}}}} & Normal & \textbf{50.3} & 39.9 & \cellcolor{Gray!10}~~4.1 & \cellcolor{Gray!10}33.8 & \textbf{50.3} & 33.4 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}17.9 & \textbf{50.3} & 40.1 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}25.7\\
        
        & Data Aug. & 47.5 & 40.8 & \cellcolor{Gray!10}~~1.4 & \cellcolor{Gray!10}36.4 & 48.1 & 37.1 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}23.0 & 47.6 & 40.6 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}29.0\\
        
        & HotFlip & 49.5 & 43.4 & \cellcolor{Gray!10}~~1.6 & \cellcolor{Gray!10}38.4 & 48.7 & \textbf{39.5} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}29.0 & 49.5 & 42.7 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}32.1 \\ 
        
        & \toolname{} & 46.4 & \textbf{43.4} & \cellcolor{Gray!10}\textbf{30.9} & \cellcolor{Gray!10}\textbf{41.9} & 46.1 & 39.0 & \cellcolor{Gray!10}\textbf{17.1} & \cellcolor{Gray!10}\textbf{37.6} & 46.5 & \textbf{43.8} & \cellcolor{Gray!10}\textbf{19.2} & \cellcolor{Gray!10}\textbf{40.0}\\ 
        
        
                \midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{\tiny{Bi-LSTM}}}} & Normal & 83.0 & 71.1 & \cellcolor{Gray!10}~~8.2 & \cellcolor{Gray!10}68.0 & 83.0 & 63.4 & \cellcolor{Gray!10}~~2.1 &  \cellcolor{Gray!10}56.1 & 83.0 & 72.5 & \cellcolor{Gray!10}~~6.4 & \cellcolor{Gray!10}65.5 \\
        
        & Data Aug. & 83.2 & 75.1 & \cellcolor{Gray!10}~~8.7 & \cellcolor{Gray!10}72.9 & \textbf{83.5} & 66.8 & \cellcolor{Gray!10}~~1.3 & \cellcolor{Gray!10}59.1 & \textbf{84.6} & 75.0 & \cellcolor{Gray!10}~~4.6 & \cellcolor{Gray!10}68.6 \\
        
        & HotFlip & \textbf{83.6} & \textbf{79.2} & \cellcolor{Gray!10}~~9.2 & \cellcolor{Gray!10}73.4 & 82.8 & \textbf{76.6} & \cellcolor{Gray!10}~~0.1 & \cellcolor{Gray!10}55.5 & 83.5 & \textbf{79.1} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}55.7\\ 
        
        & \toolname{} & 83.5 & 78.7 & \cellcolor{Gray!10}\textbf{70.9} & \cellcolor{Gray!10}\textbf{77.5} & 80.2 & 71.4 & \cellcolor{Gray!10}\textbf{59.8} & \cellcolor{Gray!10}\textbf{66.4} & 82.6 & 76.2 & \cellcolor{Gray!10}\textbf{66.2} & \cellcolor{Gray!10}\textbf{71.8}\\ 
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:lstm_whole}

\end{table*}



\begin{table}[t]
    \centering
    \caption{Results of LSTM on SST2 dataset for $\reviewperturb{}$. }
    % \renewcommand{\arraystretch}{0.8}
    % \setlength{\tabcolsep}{1pt}
    \renewcommand{\arraystretch}{0.8}
    \begin{small}
    \begin{tabular}{l *1{p{\lengthcellshorter{}}p{\lengthcell{}}p{\lengthcell{}}p{\lengthcelllonger{}}}}
        \toprule
         & \multicolumn{4}{>{\centering\arraybackslash}p{\lengththreecell{}}}{$\reviewperturb{}$}\\ 
         
         \cmidrule(lr){2-5}
        Train  & {\small Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}}  \\
        \midrule
        Normal & \textbf{83.9} & 72.4 & 21.0 & 71.0 \\
        Data Aug. & 79.2 & 72.5 & 30.5 & 71.7\\
        HotFlip & 79.6 & 74.3 & 34.5 & 72.9\\
        \textbf{\toolname{}}  & 82.3 & \textbf{78.1} & \textbf{74.2} & \textbf{77.1}\\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:compare_DSreview}

\end{table}

==> LSTM%20robust%20training%20(EMNLP)/tables/qexample.tex <==
\begin{table}[t!]
    \centering
     \caption{Qualitative examples. The vanilla model incorrectly classifies the perturbed samples.}

    % \setlength{\tabrowsep{1pt}
    \renewcommand{\arraystretch}{1}
    \begin{small} 
    \begin{tabular}{p{6.2cm}c}
        \toprule
        \textit{Original sample in SST2 dataset}   \\
        i was perplexed to watch it unfold with an astonishing lack of passion or uniqueness {$\bm .$} & \textbf{-ve}\\
        \midrule
        \textit{Perturbed sample in $\SDS$}  \\
        i was perplexed \perturbed{\sout{to}} watch it unfold with an \perturbed{astounding}
        \perturbed{absence} of passion or uniqueness $\bm .$ & \textbf{+ve}\\
        \toprule
        \textit{Original sample in SST2 dataset} \\
        this is pretty dicey material $\bm .$ & \textbf{-ve}
        \\
        \midrule
        \textit{Perturbed sample in $\SIS$} \\
        this \perturbed{becomes} pretty \perturbed{pretty} dicey material $\bm .$ \perturbed{$\bm .$}  & \textbf{+ve}
      \\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:examples}

\end{table}

==> LSTM%20robust%20training%20(EMNLP)/tables/sreview.tex <==
\begin{table*}[t]
    \centering
     \caption{String transformations for $\reviewperturb{}$.}

    % \setlength{\tabcolsep}{1pt}
    % \rowcolors{2}{}{gray!10}
    \begin{small}
    \begin{tabular}{ll}
        \toprule
         Trans & Description\\
        \midrule
          $\TReviewFirst{}$ & substitute a phrase in the set $A$ with another phrase in $A$.\\
         $\TReviewSecond{}$ & substitute a phrase in the set $B$ with another phrase in $B$ or substitute a phrase in $C$ with another phrase in $C$.\\
        $\TReviewThird{}$ & delete a phrase ``one of'' from ``one of the most ...'' or from ``one of the ...est''.  \\
        $\TReviewFourth{}$ & duplicate a question mark ``?'' or an exclamation mark ``!''.\\
        \bottomrule
    \end{tabular}
    \label{tab:s_review}
    \end{small}

\end{table*}

==> LSTM%20robust%20training%20(EMNLP)/tables/string_trans.tex <==
\begin{table}[t!]
    \centering
     \caption{String transformations.}
\renewcommand{\arraystretch}{1}
    % \setlength{\tabcolsep}{1pt}
    % \rowcolors{2}{}{gray!10}
    \begin{small}
    \begin{tabular}{ll}
        \toprule
         Trans & Description\\
        \midrule
          $\Tdelword{}$ &   \textbf{delete} a \textbf{stop word}, e.g., \textit{and, the, a, to, of,...} \\
         $\Tinsword{}$ &  \textbf{duplicate} a word \\
        $\Tsubword{}$ & \textbf{substitute} a word with one of its synonyms  \\
        \bottomrule
    \end{tabular}
    \label{tab:perturbation}
    \end{small}

\end{table}

==> sections/ablation.tex <==
\newpage
\subsection{Discussion}

\subsubsection{Ablation Study}
Alternatively, we can change the definition of $H_i^S$ to $C_i^S$:
\begin{align*}
    C_i^S = \bigcup_{j=0}^{L_{\bfx}}  \{\lstm(\bfz, \hstate_0)\mid \bfz \in S(\substring{\bfx}{1}{j}) \wedge L_{\bfz}=i\}
\end{align*}
%
By definition, the base case $C_0^\varnothing = \{0^d\}$. Notice that we do not require a tight perturbation space in the definition.

There are several disadvantages of defining $C_i^S$ in the above way:
\begin{itemize}
    \item $C_i^S$ overlap with each other, e.g., $C_i^{S_{-j}} \subseteq C_i^S$. While $H_i^S$ are disjoint unless different transformations lead to the same prefix.
    \item We have to enumerate all possible offsets for each state in $C_i^S$ because the original prefix lengths transformed by $S$ are unknown and different among the LSTM states in $C_i^S$. While the original prefix lengths transformed by $S^=$ are determined and the same among the LSTM states in $H_i^S$.
    \item The memoization of $C_i^S$ can be imprecise, i.e., containing infeasible states. While $H_i^S$ is precise.
\end{itemize}

For example, there are two states in the set $C^{\{(T_\emph{del}, 1)\}}_1$: $\lstm(\text{``to''}, \hstate_0)$ and $\lstm(\text{``the''}, \hstate_0)$. 

\textbf{Different offsets:}
For state $\lstm(\text{``to''}, \hstate_0)$, there are two possible original prefix: ``to'' (with offset 0) and ``to the'' (with offset -1). 
In other words, we can get transformed prefix ``to'' from the original prefix ``to'' by applying no transformations or from ``to the'' by applying deletion to word ``the''.

\textbf{Imprecision:}
Notice that we cannot tell what prefix has been proceeded by LSTM for each state in $C^{\{(T_\emph{del}, 1)\}}_1$. 
Because we cannot distinguish $\lstm(\text{``to''}, \hstate_0)$ with $\lstm(\text{``the''}, \hstate_0)$, we will generate states of ``to the'' (feasible), ``the the'' (infeasible) for $C^{\{(T_\emph{del}, 1)\}}_2$, resulting in imprecision. 

As we will show in the evaluation, this ablation version runs slower and certifies less test examples. 

\subsection{\textcolor{red}{new write up for memoization}}

\paragraph{Tight Perturbation Space} 

Think of the set of all strings
in a perturbation space as a tree, like in \cref{fig:approachfig}(b),
where strings that share prefixes
share LSTM states.
We want to characterize the set of LSTM
states at the $i$th layer of the tree
for prefixes that have had \emph{all} transformations in a space $S$ applied on the original prefix $\substring{\bfx}{1}{j}$.

We formally define  $H_{i,j}^S$ as follows:
\begin{align}
    H_{i,j}^S = \{\lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{j}) \wedge L_{\bfz}=i\} \label{eq: newcomplexstate}
\end{align}
By definition, the base case $H_{0,0}^\varnothing = \{0^d\}$.

\paragraph{Memoizing equation}
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.8\columnwidth]{imgs/illu_state_new.png}
    \caption{Illustration of two causes of \Eqref{eq:newcontransition1}}
    \label{fig:illu_state_new}
\end{figure*}


We now demonstrate how to rewrite \Eqref{eq: newcomplexstate}
by explicitly applying the transformations defining the perturbation space $S$, thus deriving our final equation:
\begin{align}
   H_{i,j}^S = & \bigcup_{\substack{1\leq k \leq |S|\\ \varphi_k(\substring{\bfx}{a}{b})=1}} \{\lstm(\bfz, h) \mid  \bfz \in f_k(\substring{\bfx}{a}{b}), h \in H_{i-t_k,j-s_k}^{S_{-k}}\}\nonumber \\
  &~~~~~~ \cup\ \{\lstm(x_{j}, h) \mid h \in H_{i-1,j-1}^S\} \label{eq:newcontransition1}
\end{align}
where 
$a {=} j {-} s_k + 1$ and
$b {=} j$.
Notation $S_{-k}$ denotes $S$
after reducing $\delta_k$ by 1;
therefore $S_{-k} \in \tightperturbset{S}$.

As illustrated in \Figref{fig:illu_state_new},
$H_{i,j}^S$ contains strings whose suffix is perturbed by $T_k = (\varphi_k,f_k)$ (the first line of \Eqref{eq:newcontransition1}), and strings whose suffixes are not perturbed by any transformations (the second line of \Eqref{eq:newcontransition1}). 
We compute \Eqref{eq:newcontransition1} in a bottom-up fashion, starting from $H_{0,0}^\varnothing=\{0^d\}$ and increasing $i,j$ and considering every possible perturbation space in the decomposition of $S$, $\tightperturbset{S}$.

\paragraph{Defining final states using prefixes}
Finally, we compute the set of final states, $F$, by considering all perturbation space in $\tightperturbset{S}$.
\begin{equation}
F = \bigcup_{S' \in \tightperturbset{S}} \bigcup_{i \ge 0} H_{i, L_{\bfx}}^{S'} \label{eq:newhfinal}
\end{equation}

\paragraph{Abstract memozing equations}
\begin{align*}
  \ibp{H}_{i,j}^S = & \bigsqcup_{\substack{1\leq k \leq |S|\\ \varphi_k(\substring{\bfx}{a}{b})=1}} \widehat{\lstm}(\alpha(f_k(\substring{\bfx}{a}{b})), \widehat{H}_{i-t_k,j-s_k}^{S_{-k}}) \\
  &~~~~~~\sqcup \ \widehat{\lstm}(\alpha(\{x_{j}\}), \widehat{H}_{i-1,j-1}^S)\\
%   \label{eq:abstract}~\\
\ \\
 \ibp{F} = & \bigsqcup_{S' \in \tightperturbset{S}} \bigsqcup_{i \ge 0}  \ibp{H}_{i, L_{\bfx}}^{S'} \nonumber
\end{align*}
where $a$ and $b$ are the same in \Eqref{eq:newcontransition1}.

The above abstract equations give us a compact overapproximation of $F$ that can be computed with a number of steps that is quadratic in the length of the input because we can have $O(\len{\bfx}^2)$ number of $H_{i,j}^S$ for a given $S$. 

\paragraph{Optimize the number of $H$'s} We now show that we can compute $\ibp{F}$ with a number of steps that is linear in the length of the input.

\begin{lemma}
\label{lemma: optimize_h}
For a given $i$ and $S$, define $j$ as 
\[j = \sum_{(T_k, \delta_k) \in S} (s_k - t_k)\delta_k + i \]
where $f_k: \alphabet^{s_k} \to 2^{\alphabet^{t_k}} $.
Then $H_{i,j'}^S = \varnothing$ for all $j' \neq j$.
\end{lemma}
\Lemmaref{lemma: optimize_h} tells us there is at most one non-empty $H_{i,j}^S$ for a given $i$ and $S$, which implies that there are only $O(L_x)$ number of non-empty $H_{i,j}^S$ for a given $S$.
We can prove a similar lemma for $\ibp{H}_{i,j}^S$ as well.

\begin{theorem}(Soundness \& Complexity)
\label{theorem: theorem4.2}
$F \subseteq \widehat{F}$ and the
number of LSTM cell evaluations needed is $O(L_{\bfx} n\prod_{i=1}^n \delta_i)$.
\end{theorem}

\newpage

==> sections/approach_old.tex <==
\section{\toolname{}: Abstract Recursive Certification}
\label{sec:approach}
In this section, we present our technique for proving $S$-robustness of an LSTM
on $(\bfx,y)$.
Formally, we do this by computing the adversarial loss,
$\max_{\bfz \in S(\bfx)} L_\theta(\bfz,y)$.
Recall that
if the solution is $< 0$, then we have proven $S$-robustness.
%
To solve adversarial loss optimally, we effectively need to evaluate the LSTM on all of $S(\bfx)$ and collect all final states:
\begin{align}
F = \{\lstm(\bfz,h_0) \mid \bfz \in S(\bfx)\} \label{eq: theF}
\end{align}
Computing $F$  precisely is challenging,
as $S(\bfx)$ may be prohibitively large.
Therefore, we propose to compute a superset
of $F$, which we will call $\ibp{F}$.
%
This superset will therefore yield an upper bound on the adversarial loss. 
%
We prove $S$-robustness if the upper bound is $<0$.


To compute $\ibp{F}$, we present two key ideas
that go hand-in-hand:
 In \Secref{sec:concrete}, we observe that strings in the perturbation space share common prefixes,
and therefore we can \emph{memoize} hidden states to reduce the number of evaluations of LSTM cells---a form of dynamic programming.
We carefully derive the set of final states $F$
as a system of memoizing equations.
The challenge of this derivation is characterizing which strings share common prefixes without explicitly exploring the perturbation space.
In \Secref{sec:abstract},
we apply abstract interpretation
to efficiently and soundly solve the system of memoizing equations,
thus computing an overapproximation 
$\ibp{F} \supseteq F$.

% These  ideas result in an efficient approach 
% for computing $\ibp{F}$.
% that is linear\yh{polynomial?} in the length of the input string
% and the radius of the perturbation space (defined by $\delta_i$s).


\begin{figure*}[t]
    \centering
    \includegraphics[width=1.8\columnwidth]{imgs/illu_state_new.png}
    \caption{Illustration of two causes of \Eqref{eq:contransition1}}
    \label{fig:illu_state_new}
\end{figure*}


\subsection{Memoizing Equations of Final States}
\label{sec:concrete}
We now derive a set of
memoizing equations defining $F$.
We begin by showing how to characterize sets of
intermediate states of an LSTM with respect to a perturbation space.

\subsubsection{Defining prefix states}
\paragraph{Tight Perturbation Space} 
Given a perturbation space $S$, we shall use $\tightperturb{}$ 
to denote the \emph{tight} perturbation space where each transformation $T_j$ in $S$ is applied \textbf{exactly} $\delta_j$ times. 

% \aws{i rewrote this}
Think of the set of all strings
in a perturbation space as a tree, like in \cref{fig:approachfig}(b),
where strings that share prefixes
share LSTM states.
We want to characterize the set of LSTM
states at the $i$th layer of the tree
for prefixes that have had \emph{all} transformations in a space $S$ applied.
%
% We want to characterize 
% the set of possible $i$th LSTM states (i.e., the states resulting from reading the first $i$ words of each perturbed input) that the attacker can produce by applying \emph{all} transformations in $S$. 
We formally define  $H_i^S$ as follows:
\begin{align}
    H_i^S = \bigcup_{j=0}^{L_{\bfx}}  \{\lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{j}) \wedge L_{\bfz}=i\} \label{eq: complexstate}
\end{align}
%
By definition, the base case $H_0^\varnothing = \{0^d\}$.
% Informally,  $H_i^S$ looks at every prefix
% of $\bfx$ and considers perturbed strings of length $i$
% that can be produced by  $S^=$.



% \yh{only the following example uses the $T_\emph{del}$ by deleting `the` and `to`.}
\begin{example}
\label{ex: state}
Let $\bfx =$ ``\emph{to the movie}'',
and  $S = \{(T_\emph{del},1)\}$.
Then, $H_1^S =\{\lstm(\emph{``the''},h_0), \lstm(\emph{``to''},h_0)\}$. 
These states result from deleting the first and second words of the prefix ``\emph{to the}'',
respectively.
We also have
$H_2^\varnothing = \{\lstm(\emph{``to the''}, h_0)\}$.
\end{example}

% \yh{There are two intuitions for the offset. Here is the first one.}

% We need to enumerate the prefixes of input $\bfx$ because we do not know which prefix could result in the perturbed prefix $\bfz$ of length $i$. 
% However, the offset between the prefix length of $\bfx$ and the perturbed prefix length of $\bfz$ is a constant value because $\tightperturb{}$ is tight and each transformation $T_j^{s_j, t_j}$ restricts the input and output substring length.
% Thus, we simplify \Eqref{eq: complexstate} by tracking the offset between the perturbed input indexes and the original input indexes.

% \yh{Here is the second one.}
% In \Expref{ex: state}, $\concreteset{\hstate}_{1,\{(T_\emph{del},1)\}}$ comes from the initial state taking token $x_2$ and the initial state taking token $x_1$.
% As one can see, the index of token $x_2$ have been shifted when computing state $\concreteset{\hstate}_{1,\{(T_\emph{del},1)\}}$ because the transformation $T_\emph{del}$ alters the length of the perturbed string.
% Thus, we need to track the offset between the perturbed input indexes and the original input indexes.

\paragraph{Perturbation offset}
We will now  simplify the definition of $H_i^S$ using the 
notion of an \emph{offset}: a mapping between symbols of the original string and of a perturbed string.
Specifically, we compute the difference between the index $i$ of the perturbed string and the corresponding index of the original  string. 
We define $\offset_S$ as follows:
\[\offset_S = \sum_{(T_j, \delta_j) \in S} (t_j - s_j)\delta_j, \quad \text{ where } f_j: \alphabet^{s_j} \to 2^{\alphabet^{t_j}} \]
% where $s_j$ and $t_j$ are the size of the 
% domain and range of transformation $T_j = (\varphi_j,f_j)$,
% where $f_j: \alphabet^{s_j} \to 2^{\alphabet^{t_j}}$.
% \loris{maybe inline this last part in the formula}

% \begin{figure}[t]
%     \centering
%     \input{imgs/figure2}
%     \caption{Illustration of the offset $\offset_S$.}
%     \label{fig:mappingfig}
% \end{figure}




\begin{example}
Let $S=\{(T_\emph{del},1)\}$, the original string $\bfx$ = ``to the movie'', and the perturbed string $\bfz$ = ``to movie''. 
Then,
$\offset_S = (0 - 1)\times 1 = -1$.
Intuitively, $T_\emph{del}$ reduces the length of the string by 1.
The index 2 of the perturbed string $\bfz$ ($z_2=$``\emph{movie}'') corresponds to index $2 - \offset_S = 3$ in the original input string $\bfx$, where $x_3=$``\emph{movie}''.

\end{example}

We can simplify the definition in \Eqref{eq: complexstate} with the help of the offset $\offset_S$, as follows:
\begin{align}
    H_{i}^S = \{\lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S})\} \label{eq: simplestate}
\end{align}
The intuition is that strings of length $i$
in $H_i^S$ can only be produced by perturbing 
the prefix $\substring{\bfx}{1}{i-\offset_S}$,  because applying all transformations in $S$ will change the length of the string by $\offset_S$.

\begin{lemma}
\label{lemma:4.1}
\Eqref{eq: simplestate} is equivalent to \Eqref{eq: complexstate}.
\end{lemma}

By definition of offset,
we have the set of final states of strings in 
 $\tightperturb{(\bfx)}$ as $H_{L_{\bfx} + \offset_S}^S$.
\begin{align}
    H_{L_{\bfx} + \offset_S}^S = \{\lstm(\bfz, \hstate_0) \mid \bfz \in \tightperturb{}(\bfx)\} \label{eq: finalstateoftight}
\end{align}

\paragraph{Memoizing equation}
We now demonstrate how to rewrite \Eqref{eq: simplestate}
by explicitly applying the transformations defining the perturbation space $S$, thus deriving our final equation:
\begin{align}
   H_i^S = & \bigcup_{\substack{1\leq j \leq |S|\\ \varphi_j(\substring{\bfx}{a}{b})=1}} \{\lstm(\bfz, h) \mid  \bfz \in f_j(\substring{\bfx}{a}{b}), h \in H_{i-t_j}^{S_{-j}}\}\nonumber \\
  &~~~~~~ \cup\ \{\lstm(x_{i - \offset_S}, h) \mid h \in H_{i-1}^S\} \label{eq:contransition1}
\end{align}
where
$a {=} i {-} \offset_S {-} s_j {+} 1$ and
$b {=} i {-} \offset_S$.
Notation $S_{-j}$ denotes $S$
after reducing $\delta_j$ by 1;
therefore $S_{-j} \in \tightperturbset{S}$.

% \aws{discuss this paragraph...we should be very clear about these equations...and why they are memoizing}
% \yh{have rewritten the following. how about showing how to compute the example 4.1?}
% \aws{that'd be fantastic --- and perhaps an abstraction example too}

$H_i^S$ contains strings whose suffix is perturbed by $T_j = (\varphi_j,f_j)$ (the first line of \Eqref{eq:contransition1}), and strings whose  suffixes are not perturbed by any transformations (the second line of \Eqref{eq:contransition1}). 
We compute \Eqref{eq:contransition1} in a bottom-up fashion, starting from $H_0^\varnothing=\{0^d\}$ and increasing $i$ and considering every possible perturbation space in the decomposition of $S$, $\tightperturbset{S}$ (see Ex.~\ref{ex:decs}).
% \aws{check above}

\begin{example}
% \yh{todo: example to show Eq 10.}
Consider computing $H_1^{\{(T_\emph{del}, 1)\}}$, which is the set of two states 
$\lstm(\emph{``the''},h_0)$ and $\lstm(\emph{``to''},h_0)$. 
We demonstrate how to derive these two states from \Eqref{eq:contransition1}:
\begin{align}
   H_1^{\{(T_\emph{del}, 1)\}} = & \{\lstm(\bfz, h) \mid  \bfz \in f_\emph{del}(\text{``the''}), h \in H_{1}^\varnothing\} \cup \nonumber \\
  & \{\lstm(\text{``the''}, h) \mid h \in H_0^{\{(T_\emph{del}, 1)\}}\} \label{eq:concreteex}
\end{align}
We compute \Eqref{eq:contransition1} in a bottom-up fashion, so let us assume that we have computed $H_{1}^\varnothing=\{\lstm(\text{``to''}, h_0)\}$ and 
$H_{0}^{\{(T_\emph{del}, 1)\}}=\{h_0\}$ in advance. 
Because $\bfz$ can only be an empty string, the first line of \Eqref{eq:concreteex} evaluates to $\{\lstm(\text{``to''}, h_0)\}$, which corresponds to deleting the second words of the prefix ``to the'' and is memoized in $H_{1}^\varnothing$.
The second line of \Eqref{eq:concreteex} evaluates to $\{\lstm(\text{``the''}, h_0)\}$, which corresponds to deleting the first words of ``to the''. 
\end{example}

% The first line contains the set of states for 
% which the last symbol \loris{why just the last symbol?} is not perturbed by any transformation.
% The second line contains states of strings whose suffix is perturbed by $T_j = (\varphi_j,f_j)$.

% Informally, \Eqref{eq:contransition1} denotes that no transformation matches the input index $i - \offset_\tightperturb{}$, so we feed the original token $x_{i - \offset_\tightperturb{}}$ into the LSTM cell. \Eqref{eq:contransition2} denotes that a transformation $T_j=(f_j, \varphi_j)$ matches the substring $\substring{\bfx}{a}{b}$, so we feed all possible transformed substrings to the LSTM cell.

\begin{lemma}
\label{lemma:4.2}
 \Eqref{eq:contransition1} and \Eqref{eq: simplestate} are equivalent.
\end{lemma}

% Informally, \Eqref{eq:contransition1} denotes that no transformation matches the input index $i - \offset_S$, so we feed the original token $x_{i - \offset_S}$ into the LSTM cell.  denotes that a transformation $T_j=(f_j, \varphi_j)$ matches the substring $\substring{\bfx}{a}{b}$, so we feed all possible transformed substrings to the LSTM cell.



\subsubsection{Defining Final States using Prefixes}


% \yh{Better intuition than the following benefits?}The tight perturbation space can be seen as a rewritten history of the prefix input string, which has the following two benefits.
% First, the rewritten history helps us to group the perturbed strings with same length and to compute the mapping between the original input indexes and the perturbed input indexes.
% Second, the rewritten history helps us explore the perturbation space because it reflects which string transformations have been applied to the prefix and which string transformations can be applied to the remaining input string. 

Finally, we compute the set of final states, $F$, by considering all perturbation spaces in the decomposition of $S$.
%
%
\begin{equation}
F = \bigcup_{S' \in \tightperturbset{S}} H_{L_{\bfx} + \offset_{S'}}^{S'} \label{eq:hfinal}
\end{equation}
% \yh{please check}
Intuitively, assuming $S$ has a single transformation, $F$ is the union of final states of strings with $0$ transformations, exactly $1$ transformation, exactly $2$ transformations, etc. 

% \aws{note that in the equation above we shouldn't use $S^=$,
% because the "tightness" is implicit in the definition of $H_i^S$. I.e., you give it an $S$ and it treats it tightly.}

\begin{theorem}
\label{theorem: theorem4.1}
\Eqref{eq:hfinal} is equivalent to \Eqref{eq: theF}.
\end{theorem}

% \Theref{theorem: feasiblefstate} can be proved by using \Theref{theorem: theorem1} and \Eqref{eq: finalstateoftight}. 

\begin{example}
Let $\spec=\{(T_\emph{del},1),(T_\emph{sub},1)\}$.
$F$ is the union of four final states, $H_{3}^\varnothing$ (no transformations), $H_{2}^{\{(T_\emph{del}, 1)\}}$ (exactly 1 deletion), $H_{3}^{\{(T_\emph{sub}, 1)\}}$ (exactly 1 substitution), and $H_2^{\{(T_\emph{del}, 1), (T_\emph{sub}, 1)\}} $ (exactly 1 deletion and 1 substitution).
\end{example}

\subsection{Abstract Memoizing Equations}
\label{sec:abstract}
% We have characterized
% the set of final states $F$ as a memoizing system of equations.
Memoization avoids recomputing hidden states, but it still incurs in a combinatorial explosion.
We employ abstract interpretation~\cite{DBLP:conf/popl/CousotC77} to solve the equations efficiently by overapproximating the set $F$.

\subsubsection{Abstract Interpretation}
\label{sec: ibp_def}
The \emph{interval domain}~\cite{DBLP:conf/popl/CousotC77}, or \emph{interval bound propagation},
allows us to evaluate a function %
on an infinite set of inputs
represented as a hyperrectangle in $\R^n$.

\paragraph{Interval domain}
We define the interval domain over scalars---the extension to vectors is standard.
We will use an interval $[l,u] \subset \R$, where $l,u\in\R$ and $l \leq u$,
to denote the set of all real numbers between $l$ and $u$, inclusive.
% We call  $l$ the lower bound and $u$ the upper bound.


For a finite set $X \subset \R$,
the \emph{abstraction} operator 
gives the tightest interval containing $X$,
as follows: $\alpha(X) = [\min(X),\max(X)]$.
Abstraction allows us to compactly represent a large set of strings.

\begin{example}
Suppose the words $x_1 = \emph{``movie''}$ and $x_2 = \emph{``film''}$
have the 1D embedding $0.1$
and $0.15$, respectively.
Then, $\alpha(\{x_1,x_2\}) = [0.1,0.15]$.
For $n$-dimensional embeddings,
we simply compute an abstraction of every dimension,
producing a vector of intervals.
\end{example}

The \emph{join} operation, $\sqcup$,
 produces the smallest interval containing two intervals:
 $[l,u] \sqcup [l',u'] = [\min(l,l'), \max(u,u')]$.
% Unlike in program analysis, join is rarely  used in network certification, due to lack of branching control-flow.
We will use joins to merge hidden states 
resulting from different strings in the perturbation space (recall \cref{fig:approachfig}).

\begin{example}
Say we have two sets of 1D LSTM states
represented as intervals:
$[1,2]$ and $[10,12]$.
Then $[1,2] \sqcup [10,12] = [1,12]$.
Note that $\sqcup$ is an overapproximation of $\cup$,
introducing elements in neither interval.
\end{example}

\paragraph{Interval transformers} 
To evaluate a neural network on  intervals,
we lift neural-network operations to interval arithmetic---%
\emph{abstract transformers}.
%
For a function $g$, we use $\ibp{g}$ to denote
its abstract transformer.
We use the transformers proposed by \citet{ai2,DBLP:conf/emnlp/JiaRGL19}.
We illustrate transformers for addition and any monotonically increasing function $g:\mathbb{R}\to\mathbb{R}$ (e.g., ReLU, sigmoid, tanh).
%
\begin{align*}
    [l,u] \ibp{+}[l',u'] = [l+l', u+u'],\quad
    \quad \ibp{g}([l,u]) = [g(l),g(u)] 
\end{align*}
Note how, for monotonic functions $g$, the
abstract transformer $\ibp{g}$ simply applies $g$
to the lower and upper bounds.

% \begin{example}
% $[0,10] \ \ibp{+}\ [5,20] = [5,25]$.
% \end{example}
\begin{example}
For ReLU function $\mathrm{relu}(x) = \max(0,x)$,
applying $\widehat{\mathrm{relu}}([-1,2]) = [\mathrm{relu}(-1),\mathrm{relu}(2)] = [0,2]$.
\end{example}

An abstract transformer
$\ibp{g}$
must be \emph{sound}: for any interval $[l,u]$
and $x \in [l,u]$, we have $g(x) \in \ibp{g}([l,u])$.
%
We use $\ibp{\lstm}$ 
to denote an abstract transformer of an LSTM cell.
It takes an interval of symbol embeddings and an interval of  states.
We use the definition of $\ibp{\lstm}$ given by \citet{DBLP:conf/emnlp/JiaRGL19}.

% \aws{i removed soundness}

% \paragraph{Soundness}
% An abstract transformer $\ibp{g}$ of a function $g$
% is said to be sound iff it overapproximates the results of
% $g$.
%
%  $\ibp{g}$
% is \emph{sound} iff for any interval $[l,u]$
% and any $x \in [l,u]$, we have $g(x) \in \ibp{g}([l,u])$.
% %
% Soundness is critical for certification,
% as we need  capture all final states $F$.



\subsubsection{Abstract Memoizing Equations}
We now show how to solve
\Eqref{eq:contransition1}
and \Eqref{eq:hfinal} 
using abstract interpretation.
We do this by rewriting the equations 
using operations over intervals.
Let $\ibp{H}_0^\varnothing = \alpha(\{0^d\})$, then
%
%
\begin{align*}
  \ibp{H}_i^S = & \bigsqcup_{\substack{1\leq j \leq |S|\\ \varphi_j(\substring{\bfx}{a}{b})=1}} \widehat{\lstm}(\alpha(f_j(\substring{\bfx}{a}{b})), \widehat{H}_{i-t_j}^{S_{-j}}) \\
  &~~~~~~\sqcup \ \widehat{\lstm}(\alpha(\{x_{i - \offset_S}\}), \widehat{H}_{i-1}^S)\\
%   \label{eq:abstract}~\\
\ \\
 \ibp{F} = & \bigsqcup_{S' \in \tightperturbset{S}} \ibp{H}_{L_{\bfx} + \offset_{S'}}^{S'} \nonumber
\end{align*}
where $a$ and $b$ are the same in \Eqref{eq:contransition1}.

% All operations of LSTM cells have corresponding sound abstract transformers over intervals.

The two key ideas are (1) representing sets of possible LSTM inputs abstractly as intervals, using $\alpha$;
and (2) joining intervals of 
 states, using $\sqcup$.
%
These two ideas ensure that we 
efficiently solve the system of equations, producing an overapproximation $\ibp{F}$.

% \aws{possibly connect back to figure 1 here. Also maybe more intuition?}

% \aws{give an example of abstraction}

% \loris{above assumes we always abstract. I thought we abstract somtimes only (like greedily).}

% \aws{we should discuss how we algorithmically solve the equations }
% \paragraph{Complexity}
% Computing the abstract set of final states $\ibp{F}$ has a memory complexity of $O(L\prod_{i=1}^n \delta_i (\dhidden + \chidden))$, where $L$ is the maximum length of the output string. We have $O(L\prod_{i=1}^n \delta_i)$ numbers of $\ibp{\hstate}_{i,\spec'}$ because we need to iterate through all possible indexes of the output string and all the tight perturbation spaces in $\tightperturbset{S}$. Each $\ibp{\hstate}_{i,\spec'}$ is an interval bound, which has a size of $O(\dhidden + \chidden)$.

% The abstract equations achieve two goals:
% (1) an compact overapproximation of $F$,
% and (2)




The abstract equations give us a compact overapproximation of $F$
that can be efficiently computed with a number of
steps that is linear in the length of the input.
% The following theorem establishes \emph{soundness} of our 
% technique, enabling certification.
% The proof follows immediately from 
% the fact that $\alpha$, $\sqcup$, and $\ibp{\lstm}$
% overapproximate their inputs,
% resulting in an overapproximation $F$.


% \yh{merged the following theorems}
\begin{theorem}(Soundness \& Complexity)
\label{theorem: theorem4.2}
$F \subseteq \widehat{F}$ and the
number of LSTM cell evaluations needed is $O(L_{\bfx} n\prod_{i=1}^n \delta_i)$.
\end{theorem}

For practical perturbations spaces (see \Secref{sec:evaluation}), the quantity $n\prod_{i=1}^n \delta_i$ is small and can be considered constant.
% We also make the assumption that
% the range of \emph{replace} functions $f_j$ can be abstracted offline.
% For example, if $f_j(x)$ defines the set of synonyms of a word $x$, we can compute $\alpha(f_j(x))$ offline for every word in the dictionary.
% %

% \aws{I think redrawing the running at this point with $H_i$ etc. would be very instructive} 

\subsection{Extension to Bi-LSTMs and Tree-LSTMs}\label{ssec:ext}
% \yh{todo: make the merge smooth}
A \emph{Bi-LSTM} performs a forward and a backward pass on the input.  
The forward pass is the same as the forward pass in the original LSTM. 
For the backward pass, we reverse the input string $\bfx$, the input of the match function $\varphi_i$ and 
the input/output of the replace function $f_i$ of each transformation.
% \loris{A little more detail?}

A \emph{Tree-LSTM} takes trees as input. We can define the programmable perturbation space over trees in the same form of \Eqref{eq:progspec}, where $T_i$ is a tree transformation.
We show some examples of tree transformations in \Figref{fig: treetrans}.
$\Tdelword{}$ (\Figref{fig:transdelstop}) removes a leaf node with a stop word in the tree. After removing, the sibling of the removed node becomes the new parent node.
$\Tinsword{}$ (\Figref{fig:transdup}) duplicates a word in a leaf node by first removing the word and expanding the leaf node with two children, each of which contains the previous word.
$\Tsubword{}$ (\Figref{fig:transsubsyn}) substitutes a word in the leaf node with one of its synonyms. 
\begin{figure}[!t]
    \centering\small
    \subfigure[$\Tdelword{}$: remove ``the''.]{\input{imgs/delstop}\label{fig:transdelstop}}
    \subfigure[$\Tinsword{}$: duplicate ``to''.]{\input{imgs/dup}\label{fig:transdup}}
    \subfigure[$\Tsubword{}$: substitute ``movie'' with ``film'']{\input{imgs/subsyn}\label{fig:transsubsyn}}
    \caption{Examples of tree transformations.}
    \label{fig: treetrans}
\end{figure}

We provide the formalization of \toolname{} on Bi-LSTMs and Tree-LSTMs in the supplementary material.


==> sections/old_proof.tex <==
\subsection{Proof of Lemmas and Theorems}

\textbf{\Lemmaref{lemma:4.1}}
\begin{proof}
Taking the difference of \Eqref{eq: complexstate} and \Eqref{eq: simplestate}, we need to prove
\begin{small}
\begin{align}
 &\bigcup_{j=0, j\neq i - \offset_S}^{L_{\bfx}}  \{ \bfz \mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{j}) \wedge L_{\bfz}=i\} = \varnothing \label{eq: lemma4.1_1}\\
&\left\{ 
\begin{aligned}
   \bfz \mid &\bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S}) \\
   &\wedge L_{\bfz}=i
\end{aligned}
\right\} = \{ \bfz \mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S})\} \label{eq: lemma4.1_2}
\end{align}
\end{small}

\Eqref{eq: lemma4.1_1} denotes that all other sets are empty except for $j=i - \offset_S$ in \Eqref{eq: complexstate}. \Eqref{eq: lemma4.1_2} denotes the set at $j=i - \offset_S$ in \Eqref{eq: complexstate} is the same as the set in \Eqref{eq: simplestate}.

By the definition of the offset, \Eqref{eq: lemma4.1_1} is true because $\tightperturb{}(\substring{\bfx}{1}{j})$ contains strings $\bfz$ where $\len{\bfz} = j + \offset_S$, i.e., $\len{\bfz} \neq i$.
Similarly, \Eqref{eq: lemma4.1_2} is true because $\tightperturb{}(\substring{\bfx}{1}{i - \offset_S})$ only contains strings $\bfz$ such that $\len{\bfz}=i$.
\end{proof}

\textbf{\Lemmaref{lemma:4.2}}
\begin{proof}
We prove \Lemmaref{lemma:4.2} by induction on $i$ and $S$. 

\textbf{Base case:} $H_0^\varnothing = {h_0}$ is defined by both \Eqref{eq: simplestate} and \Eqref{eq:contransition1}.

\textbf{Inductive step:} Suppose the lemma holds for $H_j^{S'}$, where $(0\le j \le i \wedge S' \subset S) \vee (0\le j < i \wedge S' \subseteq S)$. 
$S' \subseteq S$ denotes that for all $(T_k, \delta_k') \in S'$, we have $(T_k, \delta_k) \in S$ and $\delta_k' \le \delta_k$. And $S' \subset S$ denotes that $S' \subseteq S$ and there exists a transformation $T_k$ such that $(T_k, \delta_k') \in S' \wedge (T_k, \delta_k) \in S$ and $\delta_k' < \delta_k$.

The computation of $H_i^S$ contains strings whose suffix is perturbed by $T_j = (\varphi_j,f_j)$ (the first line of \Eqref{eq:contransition1}), and strings whose  suffixes are not perturbed by any transformations (the second line of \Eqref{eq:contransition1}). 

Indeed, we can decompose \Eqref{eq: simplestate} to
\begin{small}
\begin{align}
     H_{i}^S = \bigcup_{\substack{1\leq j \leq |S|\\ \varphi_j(\substring{\bfx}{a}{b})=1}} 
     \left\{\!
     \begin{aligned}
        \lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S}) \wedge \\ 
        \substring{\bfz}{i-t_j+1}{i} \in f_j(\substring{\bfx}{a}{b})
     \end{aligned}
     \right\} \cup \nonumber\\
     \left\{\!
     \begin{aligned}
        \lstm(\bfz, \hstate_0)\mid \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S}) \wedge \\ 
        \forall 1\le j \le n.\ \substring{\bfz}{i-t_j+1}{i} \notin f_j(\substring{\bfx}{a}{b}) \vee \varphi_j(\substring{\bfx}{a}{b}) = 0
     \end{aligned}
     \right\} \label{eq: lemma4.2_1}
\end{align}
\end{small}

To prove \Lemmaref{lemma:4.2}, we will compare the first line of \Eqref{eq:contransition1} with the first line of \Eqref{eq: lemma4.2_1} and the second line of \Eqref{eq:contransition1} with the second line of \Eqref{eq: lemma4.2_1}.

% \aws{the superscript should be $S_{-j}$}

\textit{The first line. }
Because of the inductive hypothesis on $H_{i-t_j} ^{S_{-j}}$ (we have $i-t_j \le i$ and $S_{-j} \subset S$), the first line of \Eqref{eq:contransition1} is equivalent to 
\begin{align}
    \bigcup_{\substack{1\leq j \leq |S|\\ \varphi_j(\substring{\bfx}{a}{b})=1}} \left\{\!
    \begin{aligned}
       \lstm(\bfz, h_0) \mid  &
    \substring{\bfz}{i-t_j+1}{i} \in f_j(\substring{\bfx}{a}{b}) \wedge\\
    &\substring{\bfz}{1}{i-t_j} \in S_{-j}^{=}(\bfx_{1:a})
    \end{aligned}
    \right\}
    \label{eq: lemma4.2_2}
\end{align}

Let 
\begin{align*}
    A &\triangleq \substring{\bfz}{i-t_j+1}{i} \in f_j(\substring{\bfx}{a}{b})  \\
    B &\triangleq \substring{\bfz}{1}{i-t_j} \in S_{-j}^{=}(\bfx_{1:a}) \\
    C &\triangleq \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S})
\end{align*}
Next, we show $A \wedge B$ is equivalent to $A \wedge C$, which proves that the first line of \Eqref{eq:contransition1} is equivalent to the first line of \Eqref{eq: lemma4.2_1}.
Note that (1) $A \wedge C \implies B$, because if $\bfz$ is in the tight perturbation space $S^=$ and the suffix of $\bfz$ is perturbed by $T_j$, then the rest of $\bfz$ (excluding the suffix) is in the tight perturbation space $S^=_{-j}$; and (2) $A \wedge B \implies C$, because if the suffix of $\bfz$ is perturbed by $T_j$ and the rest of $\bfz$ (excluding the suffix) is in the tight perturbation space $S^=_{-j}$, then $\bfz$ is in the perturbation space $S^=$.
Putting (1) and (2) together gives us $A \wedge B \Longleftrightarrow A \wedge C$.

\textit{The second line.} 
Because of the inductive hypothesis on $H_{i-1} ^S$ (we have $i-1 < i$ and $S \subseteq S$), the second line of \Eqref{eq:contransition1} is equivalent to 
\begin{align}
    \{\lstm(\bfz, h_0) \mid \substring{\bfz}{1}{i-1} \in S^=(\substring{\bfx}{1}{i -1- \offset_S}) \wedge z_{i} = x_{i-1 - \offset}\} \label{eq: lemma4.2_3}
\end{align}

We can show the condition
\begin{align*}
& \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S}) \wedge  \\
        &~~~~ \forall 1\le j \le n.\ \substring{\bfz}{i-t_j+1}{i} \notin f_j(\substring{\bfx}{a}{b}) \vee \varphi_j(\substring{\bfx}{a}{b}) = 0
\end{align*}
implies that 
\[\substring{\bfz}{1}{i-1} \in S^=(\substring{\bfx}{1}{i -1- \offset_S}) \wedge z_{i} = x_{i -1- \offset},\]
because if none of the suffix of $\bfz$ is perturbed by any $T_j$, then the last symbol of $\bfz$ must be the same as $\substring{\bfx}{1}{i - \offset_S}$.
This implication means that the second line of \Eqref{eq: lemma4.2_1} is the subset of \Eqref{eq: lemma4.2_3}.

Unfortunately, \Eqref{eq: lemma4.2_3} may not be the subset of the second line of \Eqref{eq: lemma4.2_1} because there might exist $\bfz$ such that 
\begin{align*}
    &\substring{\bfz}{1}{i-1} \in S^=(\substring{\bfx}{1}{i -1- \offset_S}) \wedge z_{i} = x_{i -1- \offset} \wedge \\
    % &~~~~ \bfz \in \tightperturb{}(\substring{\bfx}{1}{i - \offset_S + 1}) \wedge  \\
    &~~~~ \exists 1\le j \le n.\ \substring{\bfz}{i-t_j+1}{i} \in f_j(\substring{\bfx}{a}{b}) \wedge \varphi_j(\substring{\bfx}{a}{b}) = 1 
\end{align*}
However, if such $\bfz$ exists, $\lstm(\bfz, \hstate_0)$ will be included in the first line of \Eqref{eq: lemma4.2_1}.
In other words, \Eqref{eq: lemma4.2_3} is the subset of the set defined in \Eqref{eq: lemma4.2_1}.

Combining the comparison of \textit{the first line} and \textit{the second line} completes the proof.
\end{proof}


\textbf{\Theref{theorem: theorem4.1}}
\begin{proof}
We can expand \Eqref{eq: theF} using the decomposition of the perturbation space as
\begin{align}
    \bigcup_{S'\in \tightperturbset{S}} \{\lstm(\bfz, \hstate_0) \mid \bfz \in S'^{=}(\bfx)\}
    \label{eq: theorem4.1_1}
\end{align}

% \aws{"Plug X into Y"}
We can plug into \Eqref{eq: simplestate} and \Eqref{eq: finalstateoftight} into \Eqref{eq:hfinal}, getting
\begin{align}
    &\bigcup_{S'\in \tightperturbset{S}}  \{\lstm(\bfz, \hstate_0)\mid \bfz \in S'^{=}(\substring{\bfx}{1}{\len{\bfx} + \offset_S - \offset_S})\}\nonumber\\
&\bigcup_{S'\in \tightperturbset{S}} \{\lstm(\bfz, \hstate_0) \mid \bfz \in S'^{=}(\bfx)\}
    \label{eq: theorem4.1_2}
\end{align}
Because \Eqref{eq: theorem4.1_1} and \Eqref{eq: theorem4.1_2} are equivalent, we can show the equivalence of \Eqref{eq: theF} and \Eqref{eq:hfinal}.
\end{proof}

\textbf{\Theref{theorem: theorem4.2}}
\begin{proof}
The proof of soundness follows immediately from 
the fact that $\alpha$, $\sqcup$, and $\ibp{\lstm}$
overapproximate their inputs,
resulting in an overapproximation $F$.

% \aws{what does the "number of intervals" mean?
% $H_i^S$ is a single hyperrect as defined in the abstract equations}\yh{using hyperrectangle now}

The proof of complexity follows that the number of hyperrectangles $\ibp{H}_i^S$ is $O(\len{\bfx} \prod_{i=1}^n \delta_i)$. For each $\ibp{H}_i^S$, we need to enumerate through all transformations, so the complexity is $O(\len{\bfx}n\prod_{i=1}^n \delta_i)$ in terms of the number of LSTM cell evaluations. The interval bound propagation needs only two forward passes for computing the lower bound and upper bound of the hyperrectangles, so it only contributes constant time in complexity. 
In all, the total number of LSTM cell evaluation needed is $O(\len{\bfx}n\prod_{i=1}^n \delta_i)$.
\end{proof}


==> sections/overview.tex <==
\section{Overview}
\label{sec: overview}
% In this section, we compare our approach with a previous work \citep{DBLP:conf/emnlp/JiaRGL19} for LSTM interval bound propagation (IBP) against a particular perturbation space, word substitutions.
\subsection{Our approach}
In this section, we illustrate our approach using a concrete example and a particular perturbation space, word substitutions. Word substitutions allow an adversary to substitute words in the target sentence with synonyms within a specific budget $\delta$, i.e., at most $\delta$ words can be substituted. \yh{why it is reasonable to consider a budget?} Let us consider a target sentence:
\begin{center}
\emph{I love this movie}
\end{center}
and the following possible word substitutions: $\emph{I} \rightarrow \emph{We}$, $\emph{love} \rightarrow \emph{like}$, $\emph{this} \rightarrow \emph{that}$, and $\emph{movie} \rightarrow \emph{film}$.
If we allow at most $\delta=1$ word substitutions in the target sentence, we have $5 = {4\choose 0} + {4\choose 1}$ possible perturbed sentences. However, the perturbed sentence \emph{We like that movie} is infeasible in this perturbation space because the sentence contains 3 word substitutions.

\loris{at this point I think you need a paragraph that summarizes the approach.
We do 1) this, 2) that, 3) this. In the following we describe each step (maybe use paragraph headers).}

We build our approach on top of interval bound propagation (IBP), an efficient method for training verifiable neural networks. \yh{We can that say our approach can generalize to any abstract domain, as long as the join operation is defined.} IBP abstracts a set of inputs as intervals (lower bounds and upper bounds) and propagates the intervals through the neural network to compute the over-approximation of worst-cast loss. The neural network is further trained on the over-approximated loss.
To use IBP, we convert the word embeddings $\embed{w}$ of each word and synonym \loris{first time using synonym}  $w$ to intervals. 
In the previous example, the embedding of the sentence 
\[[\embed(\emph{I}), \embed(\emph{love}), \embed(\emph{this}), \embed(\emph{movie})] \in \mathbb{R}^{4 \times \dinput}\]
is converted to the interval $l^\emph{input} \in \mathbb{R}^{4 \times \dinput}, u^\emph{input} \in \mathbb{R}^{4 \times \dinput}$, where
\loris{inconsistent notation in superscript, some have parens. Also can you give some intutition before you throw this formula}
\begin{align*}
\begin{array}{lll}
    l^{(\emph{input})}_{1,j} = \min(\embed(\emph{I})_j, \embed(\emph{We})_j), &u^{(\emph{input})}_{1,j} = \max(\embed(\emph{I})_j, \embed(\emph{We})_j),&\\
    l^{(\emph{input})}_{2,j} = \min(\embed(\emph{love})_j, \embed(\emph{like})_j), &u^{(\emph{input})}_{2,j} = \max(\embed(\emph{love})_j, \embed(\emph{like})_j),&\\
    l^{(\emph{input})}_{3,j} = \min(\embed(\emph{this})_j, \embed(\emph{that})_j), &u^{(\emph{input})}_{3,j} = \max(\embed(\emph{this})_j, \embed(\emph{that})_j),&\\
    l^{(\emph{input})}_{4,j} = \min(\embed(\emph{movie})_j, \embed(\emph{film})_j), &u^{(\emph{input})}_{4,j} = \max(\embed(\emph{movie})_j, \embed(\emph{film})_j), & \forall j \in\{1,2,\ldots, \dinput\},
\end{array}
\end{align*}
where $\embed(\bfx)\in \mathbb{R}^\dinput$ is the word embedding for word $\bfx$.
\loris{this def should come earlier. I added it before, but you might want to add  the type}

%Figure~\ref{fig:overview0} shows the LSTM IBP by \citet{DBLP:conf/emnlp/JiaRGL19} where the interval bounds of hidden state $\hstate_4$ and cell state $c_4$ contain $32 = 2^4$ possible perturbed sentences because it allows all possible word substitutions.
%As we will show in experiments, allowing all possible word substitutions leads to severe over-approximation, reducing both normal test accuracy and robustness. 

An RNN cell is a function that takes as input a word embedding $\embed(\bfx_i)$ and the previous hidden state $\hstate_{i-1}$, and outputs the hidden state $\hstate_i$ at the current time step
\begin{align}
    \hstate_i = \emph{RNN}(\embed(x_i), \hstate_{i-1}) \quad \hstate_i, \hstate_{i-1}\in \mathbb{R}^\dhidden. \label{eq:pointform}
\end{align}
In IBP, an RNN cell $\emph{RNN}^\sharp$ can take as input intervals and output intervals as well
\begin{align}
    \interval{\hstate_i}{} = \emph{RNN}^\sharp((\interval{\emph{input}}{i}),(\interval{\hstate_{i-1}}{}))  \label{eq:intervalform}
\end{align}
where $\interval{input}{i}$ are the intervals for the $i$th input token and $(\interval{\hstate_i}{}), (\interval{\hstate_{i-1}}{})$ are the intervals for $\hstate_i$ and $\hstate_{i-1}$, respectively. 
\Eqref{eq:pointform} is subsumed by the interval form \Eqref{eq:intervalform} because a concrete value $x\in R$ can be written as an interval with lower bound $x$ and upper bound $x$.
%We will use the interval form like \eqref{eq:intervalform} in the rest of our paper. \yh{check.} 
To simplify notations, we write an interval $\interval{x}{}$ as $\simitvl{x}{}$.

\loris{some version of this should come early in the section, see comment about summary}
The key idea of our approach is to instrument \loris{first time you talk about instrumentation, what does it mean?} each hidden state not only with the time step but also with a rewritten history. In the word substitution case, the rewritten history counts how many word substitutions have been applied \loris{substituted?} to previous time steps.
By considering the rewritten history, we can control the budget $\delta$ and eliminate \loris{succinctly represent the space?} infeasible perturbed sentences. 

\loris{I'm having a hard time following this. You are introducing new variables and all of them should be defined. The index $\hstate_{i,j}$. I think this section should be rewritten. We can have a short meeting to discuss how.}
We use $\hstate_{i,j}$ to denote the hidden state at time step $i$ with at most $j$ substitutions applied to the prefix ending at $i$, while $\hstate_{i}$ is the hidden state at time step $i$ without rewritten history.\footnote{$\hstate_i$ can be seen as the concatenation of the hidden state and cell state at time step $i$ in LSTM.}
We use dynamic programming 
\loris{dynamic programming is a technique not the main point here. You should just give the defs first, and then
end with. These quantities can be computed in linear time using dynamic programming}
to compute $\hstate_{i,j}$, which can be transitioned from state $\hstate_{i-1,j}$ with the $i$th input token untouched, and state $\hstate_{i-1,j-1}$ with the $i$th input token substituted to its synonyms. 
\begin{align*}
    \simitvl{\hstate_{i,j}}{} = &\emph{RNN}^\sharp(\embed(x_i),\simitvl{\hstate_{i-1,j}}{})  \\
     \sqcup & \emph{RNN}^\sharp(\simitvl{\emph{input}}{i},\simitvl{\hstate_{i-1,j-1}}{}),
\end{align*}
where $\sqcup$ denotes the join of two intervals $\interval{a}{}$ and $\interval{b}{}$, defined as 
\begin{align*}
    \interval{a}{} \sqcup \interval{b}{} = \interval{c}{},
\end{align*}
where $l^{(c)}_j = \min(l^{(a)}_j, l^{(b)}_j), u^{(c)}_j = \max(u^{(a)}_j, u^{(b)}_j), \forall j\in \{1,2,\dots, d\}$. The join operation helps us merge two intervals into one interval that contains all possible concrete values of the previous two intervals.

% \begin{figure*}[!t]
%     \centering
%     \subfigure[LSTM IBP by our approach]{\includegraphics[width=\textwidth]{imgs/overview1.png}\label{fig:overview1}}
%     \subfigure[LSTM IBP by \citet{DBLP:conf/emnlp/JiaRGL19}]{\includegraphics[width=0.95\textwidth]{imgs/overview0.png}\label{fig:overview2}}
%     \caption{LSTM IBP Comparison.}
%     \label{fig: overview}
% \end{figure*}

The computation overview of our approach is shown in \Figref{fig:overview1}, which is divided into two parts.
The top part contains the perturbed sentences with no substitution, i.e., the original target sentence, while the bottom part contains the perturbed sentences with at most one substitution. \yh{need to fix the figure}

\subsection{A Previous Work}
In this section, we compare our approach with a previous work \citep{DBLP:conf/emnlp/JiaRGL19}, which also uses IBP to train robust RNNs against word substitutions.
We show two key differences between our approach and \citet{DBLP:conf/emnlp/JiaRGL19}.
First, \citet{DBLP:conf/emnlp/JiaRGL19} assumes that every word substitution can happen in the target sentence.
In other words, \citet{DBLP:conf/emnlp/JiaRGL19} does not consider the budget $\delta$ for word substitutions.
We show how \citet{DBLP:conf/emnlp/JiaRGL19} computes the hidden states in \Eqref{eq:intervalform} and in \Figref{fig:overview2}.
Second, our approach can generalize to any programmable perturbation space while the previous work cannot, as we will show in the next section.

==> tables/comparea3t.tex <==
\begin{table}[t]
    \centering
    \caption{\toolname{} vs A3T (CNN) on SST2 dataset. }
    \renewcommand{\arraystretch}{0.8}
    % \setlength{\tabcolsep}{1pt}

    \begin{small}
    \begin{tabular}{ll *1{p{\lengthcellshorter{}}p{\lengthcell{}}p{\lengthcell{}}p{\lengthcelllonger{}}}}
        \toprule
         && \multicolumn{4}{>{\centering\arraybackslash}p{\lengththreecell{}}}{$\SDS$}\\ 
         
         \cmidrule(lr){3-6}
        Train & Model & {\small Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}}  \\
        \midrule
        A3T & CNN & 80.2 & 71.9 & N/A & 70.2 \\
        \textbf{\toolname{}} & LSTM & \textbf{82.5} & \textbf{77.8} & \textbf{72.5} & \textbf{77.0}\\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:compare_a3t}

\end{table}

==> tables/comparers.tex <==
\begin{table}[t]
    \centering\small
    \caption{SAFER post-processing on IMDB dataset.
    % $^*$Exhaustive accuracy for SAFER
    % is very expensive to compute; we give an \emph{upper bound} on exhaustive accuracy, by restricting the perturbation space
    }
    % It takes more than one week to compute the exhaustive accuracy of the smoothed model. We show an upper bound of exhaustive accuracy by enumerating a subset of the perturbation space of each sample. We are able to compute the exhaustive accuracy of the model trained by \toolname{} owing to the high certified accuracy because we do not have to enumerate an example if it is certified. \yh{please check the above. should we call it data augmentation rather than smoothing?}}
    % \setlength{\tabcolsep}{1pt}

    \begin{small}
    \begin{tabular}{lllll}
        \toprule
         & \multicolumn{2}{c}{$\{(\Tsubword{},1)\}$} & \multicolumn{2}{c}{$\{(\Tsubword{},2)\}$} \\ 
         
         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        Train & \Verifiedshort{} & RS Acc. & \Verifiedshort{} & RS Acc. \\
        \midrule
        % Smoothing & \textbf{89.8} & ~~0.2 & 82.9 & \textbf{90.0} & \textbf{89.9} & ~~0.1 & 79.9$^*$ & \textbf{89.7}\\
        % \toolname{} & 86.8 & \textbf{82.0} & \textbf{84.8} & 87.2 & 86.4 & 
        % \textbf{79.6} & \textbf{83.0} & 86.7\\
        Data Aug. & ~~0.2 & \textbf{90.0} & ~~0.1 & \textbf{89.7}\\
        \toolname{} & \textbf{82.0} & 87.2 & 
        \textbf{79.6} & 86.7\\
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:compare_rs}

\end{table}


==> tables/lstm.tex <==
% \begin{table*}[t!]
%     \centering

%     % \aws{should we also highlight the \Verifiedshort{} Acc column, because that's our contribution? / also bold points for winners in all columns}
%     % \aws{we can potentially combine the three tables into one mega table, as they all have the same structure} \yh{todo: distinguish LSTM, Tree-LSTM, and Bi-LSTM}
%     \caption{Results of LSTM (on SST2 dataset) and Tree-LSTM (on SST) for three perturbation spaces. %We show the clean accuracy (Acc.), HotFlip accuracy (HF Acc.), certified accuracy (\Verifiedshort{}), and exhaustive accuracy (\Exhaustiveshort{}) of four different training methods. 
%     }
%     \setlength{\tabcolsep}{5pt}
%     \renewcommand{\arraystretch}{0.8}
%     \begin{small}
%     \begin{tabular}{cl *3{cccc}}
%         \toprule
%          && \multicolumn{4}{c}{$\{(\Tdelword{}, 2),(\Tsubword{},2)\}$} & \multicolumn{4}{c}{$\{(\Tinsword{}, 2),(\Tsubword{},2)\}$} & \multicolumn{4}{c}{$\{(\Tdelword{}, 2),(\Tinsword{},2)\}$} \\ 
         
%          \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
%         &Train & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} \\
%         \midrule
%         \multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{\tiny{LSTM}}}} & Normal & \textbf{84.6} & 71.9 & \cellcolor{Gray!10}~~4.6 & \cellcolor{Gray!10}68.9 & 84.6 & 64.0 & \cellcolor{Gray!10}~~0.5 & \cellcolor{Gray!10}55.1 & \textbf{84.6} & 73.7 & \cellcolor{Gray!10}~~1.2 & \cellcolor{Gray!10}65.2 \\
        
%         & Data Aug. & 84.0 & 77.0 & \cellcolor{Gray!10}~~5.5 & \cellcolor{Gray!10}74.4 & \textbf{84.7} & 70.2 & \cellcolor{Gray!10}~~0.3 & \cellcolor{Gray!10}61.5 & 84.5 & 75.4 & \cellcolor{Gray!10}~~0.4 & \cellcolor{Gray!10}68.3 \\
        
%         & HotFlip  & 84.0 & \textbf{78.7} & \cellcolor{Gray!10}~~4.3 & \cellcolor{Gray!10}74.6 & 82.5 & \textbf{75.9} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}62.0 & 84.4 & \textbf{80.6} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}68.7 \\ 
        
%         & \toolname{} & 82.5 & 77.8 & \cellcolor{Gray!10}\textbf{72.5} &  \cellcolor{Gray!10}\textbf{77.0} & 80.2 & 70.0 & \cellcolor{Gray!10}\textbf{55.4} & \cellcolor{Gray!10}\textbf{64.0} & 82.6 & 78.6 & \cellcolor{Gray!10}\textbf{69.4} &  \cellcolor{Gray!10}\textbf{74.6} \\ 
        
        
%                 \midrule
%         \multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{\tiny{Tree-LSTM}}}} & Normal & \textbf{50.3} & 39.9 & \cellcolor{Gray!10}~~4.1 & \cellcolor{Gray!10}33.8 & \textbf{50.3} & 33.4 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}17.9 & \textbf{50.3} & 40.1 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}25.7\\
        
%         & Data Aug. & 47.5 & 40.8 & \cellcolor{Gray!10}~~1.4 & \cellcolor{Gray!10}36.4 & 48.1 & 37.1 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}23.0 & 47.6 & 40.6 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}29.0\\
        
%         & HotFlip  & 49.5 & 43.4 & \cellcolor{Gray!10}~~1.6 & \cellcolor{Gray!10}38.4 & 48.7 & \textbf{39.5} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}29.0 & 49.5 & 42.7 & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}32.1 \\ 
        
%         & \toolname{} & 46.4 & \textbf{43.4} & \cellcolor{Gray!10}\textbf{30.9} & \cellcolor{Gray!10}\textbf{41.9} & 46.1 & 39.0 & \cellcolor{Gray!10}\textbf{17.1} & \cellcolor{Gray!10}\textbf{37.6} & 46.5 & \textbf{43.8} & \cellcolor{Gray!10}\textbf{19.2} & \cellcolor{Gray!10}\textbf{40.0}\\ 
%         \bottomrule
%     \end{tabular}
%     \end{small}
%     \label{tab:lstm}
% \end{table*}


\begin{table*}[t!]
    \centering

    % \aws{should we also highlight the \Verifiedshort{} Acc column, because that's our contribution? / also bold points for winners in all columns}
    % \aws{we can potentially combine the three tables into one mega table, as they all have the same structure} \yh{todo: distinguish LSTM, Tree-LSTM, and Bi-LSTM}
    \caption{Results of LSTM on SST2 dataset for three perturbation spaces. %We show the clean accuracy (Acc.), HotFlip accuracy (HF Acc.), certified accuracy (\Verifiedshort{}), and exhaustive accuracy (\Exhaustiveshort{}) of four different training methods. 
    }
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{0.8}
    \begin{small}
    \begin{tabular}{l *3{cccc}}
        \toprule
         & \multicolumn{4}{c}{$\SDS$} & \multicolumn{4}{c}{$\SIS$} & \multicolumn{4}{c}{$\SDI$} \\ 
         
         \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
        Train & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} & {\scriptsize Acc.} & {\scriptsize HF Acc.} & {\scriptsize \Verifiedshort{}} & {\scriptsize \Exhaustiveshort{}} \\
        \midrule
         Normal & \textbf{84.6} & 71.9 & \cellcolor{Gray!10}~~4.6 & \cellcolor{Gray!10}68.9 & 84.6 & 64.0 & \cellcolor{Gray!10}~~0.5 & \cellcolor{Gray!10}55.1 & \textbf{84.6} & 73.7 & \cellcolor{Gray!10}~~1.2 & \cellcolor{Gray!10}65.2 \\
        
         Data Aug. & 84.0 & 77.0 & \cellcolor{Gray!10}~~5.5 & \cellcolor{Gray!10}74.4 & \textbf{84.7} & 70.2 & \cellcolor{Gray!10}~~0.3 & \cellcolor{Gray!10}61.5 & 84.5 & 75.4 & \cellcolor{Gray!10}~~0.4 & \cellcolor{Gray!10}68.3 \\
        
         HotFlip  & 84.0 & \textbf{78.7} & \cellcolor{Gray!10}~~4.3 & \cellcolor{Gray!10}74.6 & 82.5 & \textbf{75.9} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}62.0 & 84.4 & \textbf{80.6} & \cellcolor{Gray!10}~~0.0 & \cellcolor{Gray!10}68.7 \\ 
        
         \textbf{\toolname{}} & 82.5 & 77.8 & \cellcolor{Gray!10}\textbf{72.5} &  \cellcolor{Gray!10}\textbf{77.0} & 80.2 & 70.0 & \cellcolor{Gray!10}\textbf{55.4} & \cellcolor{Gray!10}\textbf{64.0} & 82.6 & 78.6 & \cellcolor{Gray!10}\textbf{69.4} &  \cellcolor{Gray!10}\textbf{74.6} \\ 
        
        \bottomrule
    \end{tabular}
    \end{small}
    \label{tab:lstm}
\end{table*}

